Understanding Fuchsia Security

Fuchsia is a new open-source operating system created at Google that is currently under active development. The core architectural principles guiding the design and development of the OS include high system modularity and a specific focus on security and privacy. This paper analyzes the architecture and the software model of Fuchsia, giving a specific focus on the core security mechanisms of this new operating system.

==> Fuchsia OS/old/conclusions.tex <==
\section{Conclusions}
\label{sec:conclusions}

This paper proposes itself as the first step in the Fuchsia world. In particular, it tries to describe the main features of this operating system. From the analysis of the features of this operating system, we highlight some points that could be analyzed deeper with dedicated researches. 

==> Fuchsia OS/old/research_directions.tex <==
\section{Research Directions}
\label{sec:research_directions}
This paper presents an overview of Fuchsia OS, focusing on security mechanisms implemented to guarantee a secure execution of processes inside the system. Briefly, Fuchsia OS secures the execution of processes through sandboxing mechanisms, such as components or virtualization. Fuchsia OS provides the capability mechanism to guarantee processes interoperability, which allows components to access only specific resources that belong to other components. The verification of capabilities is done at runtime by the component manager, which leverages the component instance tree in which live the interacting component instances, to check that all components have the capabilities to perform specific actions. At a low level, Fuchsia OS provides security mechanisms to secure the interaction between a process and the kernel through the separation of concerns carried out by kernel objects and through permissions to perform operations on those objects. Thus, although Fuchsia OS is in a beta testing phase, it implements strong security mechanisms that guarantee a high-security level inside the operating system. The security analysis carried out in this paper shows that there could be promising research points that could be developed to improve the security level of Fuchsia OS. In the following, will be declared some of the most promising ones:
\begin{itemize}
    \item all component instances have to interact with each other to carry out their main task. These interactions could lead to vulnerabilities, such as information leaks and the program’s execution flow changing.
    \item a process have to interact with the kernel to execute system calls. The specific interaction between the process and kernel objects could lead to dangerous vulnerabilities.
    \item capabilities sharing could enable a component instance to abuse its permissions and execute not wanted operations.
    \item Fuchsia OS allows the developer to run its component instances inside sessions that enable sharing api and libraries between component instances. This kind of sharing could lead to vulnerabilities due to the sharing of libraries and api to component instances that have not have them.
    \item Fidl abstracts the interaction between different processes, allowing the developer to define them through a high-level language. Thus, this language and its toolchain are critical for user processes interaction and user and kernel processes interaction. A vulnerability assessment on these protocols could lead to discovering vulnerabilities exploitable on all communication between processes.
    \item the component manager creates and manages all component instances through the Realm framework. This framework is responsible for the creation and management of realm and collections, and thus, the presence of vulnerabilities in this framework could impact the entire system’s security.
    \item the realm framework provides api that allows a component instance to dynamically create a collection and attach child component instances to it. Every capability routed to a collection is also routed to every component that belongs to the collection, providing component instances with capabilities that do not need. This capability routing would allow a malicious child component inside the collection to abuse these capabilities, gaining access to resources that it must not access.
\end{itemize}

==> Fuchsia OS/old/security_mechanisms_&_discussions_old/discussion.tex <==
\section{Discussion}
\label{sec:discussion}
This section tries to discuss security mechanisms of Fuchsia OS, described in this paper. 

\subsection{Security of Kernel Objects}

\subsubsection{Separation of Concerns}
The usage of kernel objects enables the kernel to apply separation of concerns to tasks provided by zircon. 
Each object manages a task, also specific for a process, such as vmo and vmar. So, zircon kernel is principally an object manager and a system call handler. This separation of tasks allows the kernel to isolate its critical functions on the system. For example, if an attacker gained the control of a user process and of handles that it own, it could issued commands to objects, according to the rights provided to the handle, but the attack would be limited only to the object itself, and it would not propagate to other objects. The main idea is that a process cannot access to objects of which it has not the handle, so limiting the attack surface. Another important feature of objects, is that in most critical cases, the kernel responds to a system call issue creating a specific object instance and bound it to the process. Using this approach, critical objects, such as vmar and vmo, are only linked to a specific process, and not to a set of them. This approach protects the system in case an attacker would gain the control of a process, because the attack surface will be limited only to those objects own by the process. For example, if an attacker gained the access to a vmar object through an handle own by a process, it could done only operation on the virtual address space of that process, and it cannot propagate the attack on virtual address space of other processes. 

\subsubsection{Handle rights}
The handle is a pointer to a specific kernel object, as described in the paper. To each handle are associated a set of permissions to carry out operation on the related object. Providing a set of permissions to a specific handle, improve the security level of the system, because a process that owns an handle can only perform a limited set of operations on that object. The security mechanism enables the secure sharing of handles between processes. Indeed, Fuchsia OS provide a process the possibility to share its handles with other processes, through the usage of channel or sockets objects. When a process wants to pass an handle to another process, it can duplicate it and eventually reduce the set of permissions assigned to the duplicated one, limiting the set of possible operations that the target process could do. 

\subsection{Security of Component Isolation}

\subsubsection{Components}
In Fuchsia OS, all programs execute inside their isolated environment or component. A process inside a component can only see resources that belong to the component, and only those own by other components of which it has the capabilities to access. So, the fact that all components are isolated between each other and that can see only their child components, improves the security level of the system compared to the most common os, in which processes are isolated between each other, but they can access to the same resources, such as the same file system. In Fuchsia OS, the set of shared resources is limited to hardware, zircon kernels, drivers. Each component has its own file system, so the attack surface is reduced respect to the common os, and most of the attacks that involve the access of a shared file system between processes, is not applicable on Fuchsia OS.

\subsubsection{Capabilities}
Capabilities are the main security mechanism provided by Fuchsia OS. Like other capability-based os, Fuchsia OS allows processes that live outside a specific component, to access resources, such as directories on a file system local to the component, only if they own the right capabilities. Each component can expose capabilities to access only selected resources, to enable the execution of a task shared among more components. So, all resources inside a component are isolated from processes outside the component, that cannot also see them without the right capabilities. The access model behind Fuchsia OS is based on capabilities, so if a process owns a capability for a resource, it can access that resource. This access model is opposed to those based on acl \cite{acl}, in which the process that tries to access to a specific resource, must be executed by a user can has access to the resource, and so, it must be listed inside the acl table. Capabilities can be shared, so if a process owns a capability, it can share it with other processes. This mechanism is less restrictive than the acl one, because it eliminates all checks on the user that want to access the resource, and so, every process that own the capability, also malicious ones, can access the resource. In contrast with the acl mechanism, the capability mechanism speeds up authentication phase, because it does not need an acl table to be checked, but it decreases the security level of the system. 

\subsection{Security of Capability Routing}
The capability routing is a mechanism linked to component isolation. Each component exposes capabilities to allows other components to access its resources. A component can see and interact only with its child components, and so, it can expose its capabilities only to those components. When a child component acquires the capability exposed from its parent component, it can decide to share it to its child component. This mechanism allows a capability to be shared to a specific component instance, sharing it among intermediate component instances. The capability is shared to known components, because all component instances that belong to the same component instance tree, are part of the same program, and it cannot be shared to component instances that belong to different component instance trees. If all component instances define statically its child component instances, in their manifest file, a capability will be securely routed from a component to another, because all component instance would be a priori known. The mechanism presents some problems in case of collections of components. Component instances inside a collection, are created dynamically, so all capabilities routed to the collection, are also routed to all component instances. If component instance was tricked in create a malicious component instance, the latter would gained all capabilities offered by the parent component instance, and so could performed operation to destroy the logic of the application. The capability routing mechanism is a powerful mechanism in case of statically defined realm inside a component instance tree, but it lacks in case of collections.

==> Fuchsia OS/old/security_mechanisms_&_discussions_old/security_mechanisms.tex <==
\section{Security Mechanisms}
\label{sec:securty_mechanisms}
This section describes some of the most important security mechanisms used by Fuchsia OS to guarantee the secure execution of components and of the interactions between processes and kernel objects.

\subsection{Kernel Objects Rights}
Objects are not secure by design, so every handle to kernel object is provided with a set of rights that enable specific operations on the referenced object. The rights are specific for the object, such as the permission to read or write to a channel, map vmo within the address space of the process, etc. Handles can be duplicated so that a process can take more handles to the same object. In general, a process needs to duplicate a handle to maintain handles to the same object but with a different set of rights. This mechanism is provided because a process can share its handle with another through channel or socket objects. An object can be garbage-collected only when there are no handles that reference it. So, when all handles own by processes are destroyed, also those eventually own by kernel process, the object will be garbage-collected.

\subsection{Component Isolation}
At a low level, a program is executed by a process. Fuchsia OS creates a process and gives it the minimum set of resources to start its execution. The os creates the process and provides it with the resources needed to start through the launchpad library. The launchpad library provides the process with:
\begin{itemize}
    \item a handle to a vmo that contains the executable of the program to be launched
    \item program arguments
    \item environment variables
    \item a handle to the vmo that contains the vDSO library for system call invoking
    \item handles to a local file system and a handle to the loader service
\end{itemize}
Unlike most common os, the dynamic linking of shared libraries is carried out through vmo. Each shared library to be used is pushed inside a vmo, so when a process wants to invoke a function provided by one of the shared objects, it has to invoke the function as an RPC \cite{rpc} through a dedicated channel object. To each process is assigned a set of resources that only it can see and access. The process cannot access or see the resources provided by another process unless they have capabilities to do it.

\subsection{Capability Routing}
One of the most important elements of Fuchsia OS are capabilities. The interaction between components is based on capabilities exchange. Rules of Fuchsia OS rule the exchange of capabilities. Components handle the capabilities that they provide and also those that use through their manifest file. Within the manifest file, a component can specify three kinds of keywords related to the interactions with capabilities: 
\begin{itemize}
    \item \textbf{use}: this keyword specifies which capability a component could use during its execution. In detail, with this keyword, a component is allowed to use the capability provided from some other component
    \item \textbf{offer}: this keyword specifies that the component can route a certain capability to its children component instances
    \item \textbf{expose}: this keyword specifies that the component can route a certain capability to its parent in the component instance tree 
\end{itemize}
The usage of these three keywords (particularly for keywords offer and expose) enables the routing of capabilities within a component instance tree. A component instance can only see its child components. So, to route a capability to some other component, there must be a sequence of routing of the capability between the intermediate component instances. In detail, each component instance must offer or expose the target capability to its children, that have to do the same until it is reached the target component instance. The capability routing has to be defined statically within the manifest of components by using the keywords explained before. Figure \ref{fig:capability_routing} shows an example of capability routing in a component instance tree.
\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.5\textwidth]{resources/images/capability_routing.png}
    \caption{Example of capability routing}
    \label{fig:capability_routing}
\end{figure}



==> Fuchsia OS/old/security_mechanisms_&_discussions_old/versione1.1.tex <==
\section{Security Mechanisms}
\label{sec:securty_mechanisms}
This section describes some of the most important security mechanisms used by Fuchsia OS to guarantee the secure execution of components and of the interactions between processes and kernel objects.

\subsection{Handles Rights}
Objects are not secure by design, so every handle to kernel object is provided with a set of rights that enable specific operations on the referenced object. The rights are specific for the object, such as the permission to read or write to a channel, map vmo within the address space of the process, etc. The set of all possible rights is documented inside the Fuchsia documentation page \cite{handlesRights}. Handles can be duplicated so that a process can take more handles to the same object. In general, a process needs to duplicate a handle to maintain handles to the same object but with a different set of rights. This mechanism is provided because a process can share its handle with another through channel or socket objects. An object can be garbage-collected only when there are no handles that reference it. So, when all handles own by processes are destroyed, also those eventually own by kernel process, the object will be garbage-collected.

\subsubsection{Separation of Concerns of Kernel Objects}
The usage of kernel objects enables the kernel to apply separation of concerns to tasks provided by zircon. Each object manages a task, also specific for a process, such as vmo and vmar. So, zircon kernel is principally an object manager and a system call handler. This separation of tasks allows the kernel to isolate its critical functions on the system. For example, if an attacker gained the control of a user process and of handles that it own, it could issue commands to objects, according to the rights provided to the handle, but the attack would be limited only to the object itself, and it would not propagate to other objects. The main idea is that a process cannot access to objects of which it has not the handle, so limiting the attack surface. Another important feature of objects, is that in most critical cases, the kernel responds to a system call issue creating a specific object instance and bound it to the process. Using this approach, critical objects, such as vmar and vmo, are only linked to a specific process, and not to a set of them. This approach protects the system in case an attacker would gain the control of a process, because the attack surface will be limited only to those objects own by the process. For example, if an attacker gained the access to a vmar object through an handle own by a process, it could do only operation on the virtual address space of that process, and it cannot propagate the attack on virtual address space of other processes. 

\subsubsection{Security of Handle Rights}
Providing a set of rights to a specific handle, improve the security level of the system, because a process that owns an handle can only perform a limited set of operations on that object. The security mechanism enables the secure sharing of handles between processes. Indeed, when a process wants to pass an handle to another process, it can duplicate it and eventually reduce the set of permissions assigned to the duplicated one, limiting the set of possible operations that the target process could do. A possible best practice to secure the access to kernel objects is to implement a least privilege approach on the rights of objects. Indeed, a process can change rights assigned to a handle, being able to specify only the minimum set of rights, needed to execute its task. This approach can prevent an attacker to leverage specific rights to execute non-authorized operations on objects referenced by handles own by the process. 

\subsection{Component Isolation}
At a low level, a program is executed by a process. Fuchsia OS creates a process and gives it the minimum set of resources to start its execution. The os creates processes inside a component and provides them with the resources needed to start through the launchpad library. The launchpad library provides the process with:
\begin{itemize}
    \item a handle to a vmo that contains the executable of the program to be launched
    \item program arguments
    \item environment variables
    \item a handle to the vmo that contains the vDSO library for system call invoking
    \item handles to a local file system and a handle to the loader service
\end{itemize}
Unlike most common os, the dynamic linking of shared libraries is carried out through vmo objects. Each shared library to be used is pushed inside a vmo, so when a process wants to invoke a function provided by one of the shared objects, it has to invoke the function as an RPC \cite{rpc} through a dedicated channel object. To each process is assigned a set of resources that only it can see and access. The process cannot access or see the resources provided by another process unless they have capabilities to do it. The main principle that enable the component isolation is namespace. Component manager provides each a component with a namespace. Fuchsia OS has not a single file system, but each component has its own. The absence of a shared file system simplifies the adoption of security mechanisms to protect a component file system. Indeed, in most common operating systems, the concept of user is important to manage access to specific files or directory of the common file system. The user can access only to those files that it owns or those for which it has permissions gave from owners. This mechanism is important to manage he access of files that belong to different users and that are stored on the same physical file system. The isolation of file systems for components deletes the needing for users. Indeed, a process inside a component has all privileges to access files in its namespace, because all files belong to it. 

\subsubsection{Security of Components}
In Fuchsia OS, all programs execute inside their isolated environment or component. A process inside a component can only see resources that belong to the component, and only those own by other components of which it has the capabilities to access. So, the fact that all components are isolated between each other and that can see only their child components, improves the security level of the system compared to the most common os, in which processes are isolated between each other, but they can access to the same resources, such as the same file system. In Fuchsia OS, the set of shared resources is limited to hardware, zircon kernels, drivers. Each component has its own file system, so the attack surface is reduced respect to the common os, and most of the attacks that involve the access of a shared file system between processes, is not applicable on Fuchsia OS. In Fuchsia there is not the concept of user, because a process can access only to the limited resources provided by its component, so a process has all rights to access resources within the component, included files on the local file system. The absence of users makes impossible privilege escalation attacks. The isolation provided by components protect the system in case an attacker would take the control of a process inside a component. Indeed, if an attacker took the control of a process, it would have
access and modify only to resources inside the component, in particular only to files inside the local file system of the component and those stored in other components for which it has the capabilities to access. So, exploiting a vulnerability inside a component, compromises the execution flow only of that component, and does not propagate to others.

\subsubsection{Security of Capabilities}
Capabilities are the main security mechanism provided by Fuchsia OS. Like other capability-based os, Fuchsia OS allows processes that live outside a specific component, to access resources, such as directories on a file system local to the component, only if they own the right capabilities. Each component can expose capabilities to access only selected resources, to enable the execution of a task shared among more components. So, all resources inside a component are isolated from processes outside the component, that cannot also see them without the right capabilities. The access model behind Fuchsia OS is based on capabilities, so if a process owns a capability for a resource, it can access that resource. This access model is opposed to those based on acl \cite{acl}, in which the process that tries to access to a specific resource, must be executed by a user can has access to the resource, and so, it must be listed inside the acl table. Capabilities can be shared, so if a capability is routed to a component, all processes inside the component can use it. This mechanism is less restrictive than the acl one, because it eliminates all checks on the identity of the process that want to access the resource, and so, every process inside the component, also malicious ones, can access the resource. 

\subsubsection{Packages verification}
Packages are signed through the merkle tree algorithm \cite{merkleTree}, to guarantee that its content could not be modified. Packages are uniquely identified by a url. The content of a package is separated for its typology:
\begin{itemize}
    \item \textbf{meta}: metadata information are contained within the meta.far archive. This file is the result of compressing metadata files with the far archive format \cite{far}. meta.far contains the meta directory, which contains the package file, that specifies name and version for the package, and the contents file, which support checks with for merkle tree verification of the package
    \item \textbf{non-meta files}: all files and directories outside the meta.far archive, are files needed to instance a new component instances, such as the binary of the program and eventual shared libraries
\end{itemize}
Fuchsia packages support their integrity verification thanks to the application of merkle tree algorithm. A package stores all metadata information within the meta.far archive, included the ones needed to verify the integrity of the package. To verify the integrity of the package, the package manager recomputes the merkle tree based on the content of the package. If the computed tree matches the one stored in the contents file, within the meta.far, the package is correctly verified and can be used from the component manager to instance a new component instance. Also far archives support the integrity verification through merkle tree algorithm, so the meta.far archive is previously verified before the verification of the package. The merkle root algorithm allows component manager to only verify the integrity of the package, because the package could be downloaded from external repositories through the https protocol. So, the integrity verification of the package is needed to guarantee that the package is correctly downloaded from external providers. This mechanism does not help component manager to guarantee that the package has not been maliciously modified, because an attacker could modify the package content, replacing the merkle tree stored within the contents file.

\subsection{Capability Routing}
One of the most important elements of Fuchsia OS are capabilities. The interaction between components is based on capabilities exchange. Rules of Fuchsia OS rule the exchange of capabilities. Components manage the capabilities that they provide and also those that use through their manifest file. Within the manifest file, a component can specify three kinds of keywords related to the interactions with capabilities:
\begin{itemize}
    \item \textbf{use}: this keyword specifies which capability a component could use during its execution. In detail, with this keyword, a component is allowed to use a capability provided from some other component
    \item \textbf{offer}: this keyword specifies that the component can route a certain capability to its child component instances
    \item \textbf{expose}: this keyword specifies that the component can route a certain capability to its parent in the component instance tree 
\end{itemize}
The usage of these three keywords (particularly for keywords offer and expose) enables the routing of capabilities within a component instance tree. A component instance can only see its child components. So, to route a capability to some other component, there must be a sequence of routing of the capability between the intermediate component instances. In detail, each component instance must offer or expose the target capability to its children, that have to do the same until it is reached the target component instance. The capability routing has to be defined statically within the manifest of components by using the keywords explained before. When a component needs to use a  capability provided by some other component, it has to interact with the component manager. The component manager is also responsible for managing the capability routing process. It maintains the component instance tree for all applications, to manage the routing of the exposed capabilities. So, when a component tries to access to a resource provided by another component, it forwards the request to the component manager that validate it through the component instance tree of the target component instance. After receiving the request, the component manager will navigate through the component instance tree, checking the path between the component instance that issued the request and the target one, and analysing the component manifest of all intermediate component instance between them. In particular, all intermediate component instances must access the capability and expose it to children or parent. At the end of the analysis, if the component instance that issued the request, can access the capability, it will be able to perform the request to the target component through the component manager. Figure \ref{fig:capability_routing} shows an example of capability routing in a component instance tree.
\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.5\textwidth]{resources/images/capability_routing.png}
    \caption{Example of capability routing}
    \label{fig:capability_routing}
\end{figure}

\subsubsection{Security of Capability Routing}
The capability routing is a mechanism linked to component isolation. Each component exposes capabilities to allows other components to access its resources. A component can see and interact only with its child components, and so, it can expose its capabilities only to those components. When a child component acquires the capability exposed from its parent component, it can decide to share it to its child component. This mechanism allows a capability to be shared to a specific component instance, sharing it among intermediate component instances. The capability is shared to known components, because all component instances that belong to the same component instance tree, are part of the same program, and it cannot be shared to component instances that belong to different component instance trees. If all component instances define statically its child component instances, in their manifest file, a capability will be securely routed from a component to another, because all component instance would be a priori known. The mechanism presents some problems in case of collections of components. Component instances inside a collection, are created dynamically, so all capabilities routed to the collection, are also routed to all component instances. If component instance was tricked in create a malicious component instance, the latter would gain all capabilities offered by the parent component instance, and so could perform operation to destroy the logic of the application. The capability routing mechanism is a powerful mechanism in case of statically defined realm inside a component instance tree, but it lacks in case of collections.



==> Fuchsia OS/old/version_1.0/component_description.tex <==
\section{Component Description}
\label{sec:component_description}
The following will describe some concepts and functioning of Fuchsia OS with a particular effort on the component framework and on system call invoking.

\subsection{Component}
A component is a program that executes on a Fuchsia device. Every software that executes on a Fuchsia device is a component, unless the Zircon kernel, bootloader, or device drivers. A component provides a binary program with an isolated environment not accessible from processes that belong to a different component. All components are uniquely identified by a url, ie. fuchsia-pkg://fuchsia.com/stash\#meta/$<component\_manifest>$.cm. A process inside a component can access only the resources inside that component. It could use specific resources from other ones only if it has the right capabilities. It communicates with other components through inter-process-communications (IPC) primitives, such as channels, sockets, fifo, to perform specific tasks or access resources provided by other components. Components implement the separation of concerns approach, allowing a developer to modularize its programs and dividing a more complex task into sub-tasks that can be carried out separately by different components. So, this approach allows a developer to extend its main task, adding new components without altering their main structure. A component could not contain a program to execute, and so, in this case, it can deliver \textit{capabilities} to other components. Fuchsia OS provides many runner components that can execute the code of programs inside a component. The modularization of the execution of programs inside a component would allow a developer to create custom runner components to execute programs written in a code not natively supported by Fuchsia OS. Fuchsia OS allows a component to define its configurations through the component manifest file. It describes the runner that will execute the code inside the component, the capabilities \textit{exposed} or \textit{offered} by the component, the static children of the component.

\subsubsection{Capability}
Fuchsia OS is a capability-based operating system. A capability is a token that identifies the rights to access a specific resource provided by a component. A component can expose capabilities to other components to access specific resources, enabling the interaction between different components. The available capabilities are fixed, so anyone cannot define custom capabilities to access resources other than those allowed by Fuchsia OS. Fuchsia capabilities are classified into seven types:
\begin{itemize}
    \item \textbf{Directory Capability}: this capability type allows a component to expose to other components the rights to see and use a specific directory inside the file system local to the component. The set of options associated with this capability type are declared inside the component manifest. For example, within the component manifest, a component can declare the path to the local directory and the set of rights on that directory. 
    \item \textbf{Event Capability}: this capability type allows components to receive events on information originated from the component manager. All component instances in a component instance tree can use the capability. So, see the event only if they explicitly declare it in their manifest, and it could be possible to route the capability to them. 
    \item \textbf{Protocol Capability}: in Fuchsia OS, a FIDL protocol is composed of a set of methods and events, which enable the interaction between different components. This capability type allows a component to use a specific FIDL protocol, exposed from another component or by the os itself. If the component provides a protocol, it will expose it through its outgoing directory (a directory in the local file system of the component, accessible from the other components, generally the svc directory).
    \item \textbf{Resolver Capability}: resolvers are specific elements of Fuchsia OS that allow a component to resolve the url for another component. The default url is already resolved by default, such as fuchsia-pkg, which identifies a package inside the os, fuchsia-boot, that identifies a component within the system boot image, http, that identifies a resource available through http protocol. In addition to these url schemes, a component can specify its custom url scheme through its manifest file, providing the associated resolver to other components through capability routing.
    \item \textbf{Runner Capability}: a runner component is responsible for running programs. Each runner supports the execution of a program written in a specific language. A component can specify the runner capability within the environment tag of its manifest file. So it will be available to all of its descendant components (or components inside the realm).
    \item \textbf{Service Capability}: in Fuchsia OS, a service is a set of protocols that allows components to perform more complex interactions with each other. This capability enables a component to offer or expose a specific service through its outgoing directory (usually the svc directory).  
    \item \textbf{Storage Capabilities}: the storage capability is linked to the directory capability. With this capability, a component allows another one to access an isolated directory inside its file system, visible and accessible only to the other component. This capability requires that the other component also receives the capability to access the directory in which the isolated one will be created. 
\end{itemize}

\subsubsection{Component Topology}
The component manager creates components from a package, a bundle that includes manifest, build configurations, and the program’s source that the runner process has to execute. The runner process is responsible for starting a new running component, which will be called a component instance. The component instance tree describes how component instance trees are related to each other. A moniker identifies each component instance within a component instance tree. It is an identifier built from the path to the component instance within the component instance tree. If the path used to identify the component instance is a relative path, the moniker will be a relative moniker. Else it will be an absolute moniker. Fuchsia uses a component instance tree to express composition relationships between components. Indeed, a child node is part of its parent node, forming a composition relationship between them. Each child component instance depends entirely on the parent, and so, it lives until the parent is alive.

\subsubsection{Realm \& Collection}
The component manager creates a child component instance if declared within the manifest of another one or a component calls realm framework primitives to dynamically instance new instances. In a component instance tree, a Realm is a sub-tree routed on a component instance that have only children created statically from the manifest of their parents. Each child component instance in a realm is also the root of its sub-realm. A realm manages capability routing for capabilities that belong to component instances inside the realm, deciding which capabilities can be exposed outside the realm through the root component instance of the realm. Collections are groups of dynamic component instances children that are linked to a specific parent node. A component instance can create and manage a collection through the realm framework. The capability routing for dynamic component instances inside a collection is more straightforward than that of realms. All capabilities offered to a collection are also offered to every component instance within it. 
\francesco{
    \begin{itemize}
        \item inserire immagine che spieghi cosa è un realm
        \item inserire immagine che spieghi cosa è una collection
    \end{itemize}
}

\subsubsection{Component Lifecycle}
A component has its lifecycle, which the component manager handles. Each component could listen for incoming lifecycle events, and so, they can perform tasks based on the state changed. In the following are reported the possible states for a component:
\begin{enumerate}
    \item \textbf{Create}: the component manager can create a component as the root of its component instance tree. Most of the time, starting a component is caused by the static declaration of the component inside the manifest file of another component or dynamically adding to an existing collection. Another important reason to start a component is a binding request from a component to another one. If a component wants to bind itself to another one, the component manager will check if there is a running instance of that component. If it finds a running instance, it will bind the component to the target one. Otherwise, it will create a new instance of that component and bind it to the new instance.
    
    \item \textbf{Start}: after the creation of a component, the component manager interacts with the required runner to execute the code inside that component. The runner will start the component, and so, this will pass it to the started state.
    
    \item \textbf{Stop}: a component could be stopped from the component manager because it terminated its task or when the user turns off the device. When a component passes to a stopped state, the component manager stores its state in persistent storage to restart the component further.
    
    \item \textbf{Destroy}: when a component instance is in a destroyed state, the component manager cannot restart it, and so, it completely removes it from its component instance tree. Still, it continues to exist in persistent storage.
    
    \item \textbf{Purge}: the component manager completely removes a component in this state from the system. Indeed, the OS will also delete its state from persistent storage.
\end{enumerate}

\subsection{Component Framework}
The component framework provides all tools to run components on Fuchsia and to support their execution. The main approach of Fuchsia is to divide a complex task into sub-task, each carried out by a specific component. Each component implements its sub-task through a service that it exposes to the other components. The interaction between different components through the usage of the exposed services allows the components to carry out a more complex task. Indeed, Fuchsia OS was thought to be modular and extensible during its lifetime. So, all tasks to be carried out are divided into multiple sub-task, each one executed from a different component, allowing their modularization. 

\subsection{FIDL}
Fuchsia Interface Definition Language (FIDL) is a set of tools that allows processes to communicate with each other, using high-level interfaces based on inter-process-communication (IPC) mechanisms. The usage of FIDL to abstract IPC between processes simplifies the implementation of the interaction between processes and lets avoid the more prone to bugs implementation through channels. Developers can define fidl files that specify the communication structure between processes, helping to define fuchsia protocols. These files are written in fidl language, which is similar to the most common languages and allows developers to use data types like integers, strings, arrays, structs, etc.  
The fidlc compiler compiles these files to produce client and server codes in the language used by the components that have to interoperate, and then these files can be included within the components code. These generated codes compose the fidl binding. At a low level, the communication implemented by fidl protocols is based on zircon channels, so the zircon kernel has an active part in the communication of component instances. FIDL enables the communication between processes applying standard communication models, also used in standard client-server interactions: 
\begin{itemize}
    \item \textbf{Client waits}: in this model, the client sends a request to the server and waits for the reply. The request sent can be a message or a call to a function exposed by the server
    \item \textbf{Client does not wait - no reply}: The client sends a request to the server but does not wait for the reply
    \item \textbf{Client does not wait - reply}: in this model, the client sends a request to the server but does not block itself waiting for the reply, and it will eventually check for the reply asynchronously. 
    \item \textbf{Client sends one request, Server sends multiple ones}: in this model, the client sends one request and blocks itself, waiting for the response only at the end of the computation. When the server sends the response, the client will be unlocked and can continue its execution until it needs new data from the server.
    \item \textbf{Server send data without Client request}: this model is similar to the previous one, but in this case, the server sends data without an initial request from the client
\end{itemize}

\subsection{System Call Execution}
When a process invokes a system call, the Zircon kernel starts a pipeline to handle it. In most os, a process invokes a system call passing the needed arguments to registers. Then, it invokes an interrupt to allow the os to execute the system call. In Fuchsia OS, the execution of a system call has to pass several intermediate phases to be completed:
\begin{enumerate}
    \item \textbf{vDSO}: it is a shared library that declares a function for each system call. Each declared function only has to put, in eax register, the integer that corresponds to the system call that names the function. All functions accept arguments that they have to pass to the handler procedure through the calling convention for the architecture in which the os executes. After the update of the eax register, all functions will execute a context switch to kernel mode to allow the kernel to execute the handler procedure. This shared object is hard-coded inside the Zircon kernel code, and it is loaded in a vmo object after the system boot.
    \item \textbf{Handler}: each system call takes its arguments from specific registers. The registers’ set is different for system calls (usually statically declared in the documentation). For all system calls, the eax register is responsible for storing the integer that identifies the system call within the system. The handler is composed of instructions that have to identify the invoked system call through the content of eax register and have to fill registers according to the specific system call invoked. The handler is different for system calls and for architecture in which the os executes. 
    \item \textbf{Wrapper}: the wrapper is a code that has to invoke the right system call implementation and handles every value returned from the system call. In most common cases, system call return handles to os objects.
    \item \textbf{Implementation}: this is the true code that execute the system call
\end{enumerate}
System call handlers and wrappers are automatically generated by a tool called kazoo \cite{kazoo}. Kazoo bases the generation of a specific pair of handler and wrapper on a fidl source file. The fidl source specifies input arguments to the system call and possible output values. In general, every kernel object has its fidl source \cite{vdso}, which declares all system calls related to that object. The fidl source is compiled with the fidlc compiler \cite{fidlc}, which generates a json file as an intermediate representation. This json file is given in input to the kazoo tool, which generates the handler, a c++ source that relies on the specific architecture of the device.

\subsection{Starnix Project}
Recently Google started to work on a side project called Starnix \cite{starnix}, which aims to allows Fuchsia to execute native android and linux applications. Indeed, Fuchsia provides a virtualization service to run external applications, with the overhead caused by the execution on virtual machines. Hence, the idea behind Starnix is to allow Fuchsia to emulate system call invocation and api calls, similarly to the wsl 1 \cite{wsl1}, to guarantee the complete execution of programs written for other contexts. 
 

==> Fuchsia OS/old/version_1.0/conclusions.tex <==
\section{Conclusions}
\label{sec:conclusions}

This paper proposes itself as the first step in the Fuchsia world. In particular, it tries to describe the main features of this operating system. From the analysis of the features of this operating system, we highlight some points that could be analyzed deeper with dedicated researches. 

==> Fuchsia OS/old/version_1.0/discussion.tex <==
\section{Discussion}
\label{sec:discussion}
This section tries to discuss security mechanisms of Fuchsia OS, described in this paper. 

\subsection{Security of Kernel Objects}

\subsubsection{Separation of Concerns}
The usage of kernel objects enables the kernel to apply separation of concerns to tasks provided by zircon. 
Each object manages a task, also specific for a process, such as vmo and vmar. So, zircon kernel is principally an object manager and a system call handler. This separation of tasks allows the kernel to isolate its critical functions on the system. For example, if an attacker gained the control of a user process and of handles that it own, it could issued commands to objects, according to the rights provided to the handle, but the attack would be limited only to the object itself, and it would not propagate to other objects. The main idea is that a process cannot access to objects of which it has not the handle, so limiting the attack surface. Another important feature of objects, is that in most critical cases, the kernel responds to a system call issue creating a specific object instance and bound it to the process. Using this approach, critical objects, such as vmar and vmo, are only linked to a specific process, and not to a set of them. This approach protects the system in case an attacker would gain the control of a process, because the attack surface will be limited only to those objects own by the process. For example, if an attacker gained the access to a vmar object through an handle own by a process, it could done only operation on the virtual address space of that process, and it cannot propagate the attack on virtual address space of other processes. 

\subsubsection{Handle rights}
The handle is a pointer to a specific kernel object, as described in the paper. To each handle are associated a set of permissions to carry out operation on the related object. Providing a set of permissions to a specific handle, improve the security level of the system, because a process that owns an handle can only perform a limited set of operations on that object. The security mechanism enables the secure sharing of handles between processes. Indeed, Fuchsia OS provide a process the possibility to share its handles with other processes, through the usage of channel or sockets objects. When a process wants to pass an handle to another process, it can duplicate it and eventually reduce the set of permissions assigned to the duplicated one, limiting the set of possible operations that the target process could do. 

\subsection{Security of Component Isolation}

\subsubsection{Components}
In Fuchsia OS, all programs execute inside their isolated environment or component. A process inside a component can only see resources that belong to the component, and only those own by other components of which it has the capabilities to access. So, the fact that all components are isolated between each other and that can see only their child components, improves the security level of the system compared to the most common os, in which processes are isolated between each other, but they can access to the same resources, such as the same file system. In Fuchsia OS, the set of shared resources is limited to hardware, zircon kernels, drivers. Each component has its own file system, so the attack surface is reduced respect to the common os, and most of the attacks that involve the access of a shared file system between processes, is not applicable on Fuchsia OS.

\subsubsection{Capabilities}
Capabilities are the main security mechanism provided by Fuchsia OS. Like other capability-based os, Fuchsia OS allows processes that live outside a specific component, to access resources, such as directories on a file system local to the component, only if they own the right capabilities. Each component can expose capabilities to access only selected resources, to enable the execution of a task shared among more components. So, all resources inside a component are isolated from processes outside the component, that cannot also see them without the right capabilities. The access model behind Fuchsia OS is based on capabilities, so if a process owns a capability for a resource, it can access that resource. This access model is opposed to those based on acl \cite{acl}, in which the process that tries to access to a specific resource, must be executed by a user can has access to the resource, and so, it must be listed inside the acl table. Capabilities can be shared, so if a process owns a capability, it can share it with other processes. This mechanism is less restrictive than the acl one, because it eliminates all checks on the user that want to access the resource, and so, every process that own the capability, also malicious ones, can access the resource. In contrast with the acl mechanism, the capability mechanism speeds up authentication phase, because it does not need an acl table to be checked, but it decreases the security level of the system. 

\subsection{Security of Capability Routing}
The capability routing is a mechanism linked to component isolation. Each component exposes capabilities to allows other components to access its resources. A component can see and interact only with its child components, and so, it can expose its capabilities only to those components. When a child component acquires the capability exposed from its parent component, it can decide to share it to its child component. This mechanism allows a capability to be shared to a specific component instance, sharing it among intermediate component instances. The capability is shared to known components, because all component instances that belong to the same component instance tree, are part of the same program, and it cannot be shared to component instances that belong to different component instance trees. If all component instances define statically its child component instances, in their manifest file, a capability will be securely routed from a component to another, because all component instance would be a priori known. The mechanism presents some problems in case of collections of components. Component instances inside a collection, are created dynamically, so all capabilities routed to the collection, are also routed to all component instances. If component instance was tricked in create a malicious component instance, the latter would gained all capabilities offered by the parent component instance, and so could performed operation to destroy the logic of the application. The capability routing mechanism is a powerful mechanism in case of statically defined realm inside a component instance tree, but it lacks in case of collections.

==> Fuchsia OS/old/version_1.0/fuchsia_os.tex <==
\section{Fuchsia OS}
\label{sec:fuchsia_os}
This section presents the stack of Fuchsia OS, describing the composing elements of the architecture stack

\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.5\textwidth]{resources/images/fuchsia_architecture.png}
    \caption{Fuchsia Architecture}
    \label{fig:fuchsia_architecture}
\end{figure}

\subsection{Zircon}
The core of this operating system is the Zircon kernel. Zircon is a micro-kernel based on the Little Kernel project \cite{lk} to guarantee high performances on all kinds of devices, from IoT devices to smartphones. Little Kernel is mainly thought to adapt itself to devices with limited computational resources. So, it is suitable for the Fuchsia project that aims to be supported from as many devices as possible. It provides only the basic set of functionalities needed for the OS to work correctly as a micro-kernel. It is responsible for loading userspace processes in memory, communicates with the underlying hardware to make OS and hardware communicate, handles the booting phase of the device, powers up components that will take this phase, etc. Compared to a standard kernel, Zircon has to handle fewer tasks because many elements, such as drivers and the file system, are managed by user processes. Thanks to this simplification, the number of context switches between user-mode and kernel-mode, caused by operations that the kernel code has to execute, decreases.

\subsubsection{IPC}
Zircon kernel manages inter-process communication (IPC) between different processes and allows them to communicate although isolated in memory.
\begin{itemize}
    \item \textbf{Channel}: this object implements a bidirectional communication channel. A channel has two endpoints, and each of them maintains a separate fifo queue to store incoming messages. Every channel endpoint has an owner that also marks all messages sent and received by the endpoint, and only it can access these messages. They provide user code with primitives to add messages to the queue of the recipient process and to read them, and so, to dequeue them. A channel endpoint is not duplicable, but the owner could pass its ownership to another one. When the endpoint owner passes its ownership to a new owner, the new owner cannot access all messages in the queue marked with the previous owner.
    
    \item \textbf{Socket}: this object implements a bidirectional communication channel. These objects only move data and not handles, unlike the channel object. Processes can read and write data through their socket endpoints, using socket primitives. At the creation of the socket, the process can specify the in-bytes dimension of the socket.
    
    \item \textbf{FIFO}: objects thought to support shared memory between processes. They are more efficient than socket and channel objects in terms of timing to complete io operations, but they have a more limited buffer size.
\end{itemize}

\subsubsection{Scheduling \& Synchronization}
The Zircon kernel manages scheduling tasks for processes and threads that execute on the cpu of the device. This scheduler is based on the LK scheduler \cite{lk}, but it was extended to meet the needings of the Fuchsia OS. Together with scheduling tasks, Zircon also supports signal primitives to allow synchronization between different threads.
\begin{itemize}
    \item \textbf{Profile}: this object defines a set of priorities for scheduling configurations that the zircon kernel could apply to processes and threads. A single profile object could be linked with more processes and threads, and in this case, the scheduler will put them at the same level.
    
    \item \textbf{Event}: these objects are created to signal specific events for synchronization between processes.
    
    \item \textbf{Futex}: objects that manage synchronization between processes at a low level and in user-mode. They are the basis for \textit{pthread\_mutex} and \textit{pthread\_cond}, that are higher-level primitives. Futex objects do not provide rights to access to primitives that they expose because the base operations are \textit{wait} and \textit{wake} that have to be both accessible to leverage the basic functionalities of the object. Futexes does not support priority for calling processes, but they provide some API to allow further implementations based on them that could offer priority functionalities. The basis for priority implementation is the concept of ownership of a futex. If a process owns one or more futexes, its scheduling priority will be pushed to maximum among the waiter processes on the same futex. When a process unowns all its futexes, its scheduling priority will be restored to the base one.
\end{itemize}

\subsubsection{Memory Management}
Zircon kernel manages the allocation of memory to processes. Specific objects carry out all operations on the allocation and assignment of memory.
\begin{itemize}
    \item \textbf{Virtual Memory Object (VMO)}: an object that represents a region of virtual memory that can be shared among different processes. This object allows a process to perform several operations, such as reading, writing to the mapped pages and mapping the object itself to the process that requested the object. The vmo is a high-level infrastructure that allows the process to interact with the underlying memory pages, and it can also provide on-demand pages when needed.
    
    \item \textbf{Virtual Memory Address Region}: these objects represent a continuous set of addresses taken from a virtual address space. When a program executes, it has only a single vmar that contains all addresses of the program’s virtual address space, but it could be further divided with the creation of new vmar that do not overlap themself in their address space. Each vmar has a set of rights on the underlying memory. The starting vmar has all rights (read, write, execution) on the underlying memory. When a process makes a syscall to partition an existing vmar further, it can also specify the set of permissions for the new vmar. All vmar created by a process are related to each other by a tree data structure. In detail, a parent vmar maintains a reference to its children vmar, and this does not allow the destruction of a child vmar though there are no handles to it in the processes.
    
    \item \textbf{Pager}: these objects are responsible for supporting data provider entities, such as filesystems, to cache data they have to pass to other processes that request them. Their main task is to create vmo objects and provide them the needed pages to store data from the data provider.
\end{itemize}

\subsection{Fuchsia Runtime}
Fuchsia provides different kinds of runtimes that can start components. These runner processes are components that communicate with the component manager to obtain configurations for a program to be run. Their main task is to read configurations sent from the component manager to start executing new components. They do not provide libraries, but they only start their execution, so all components must have all libraries inside their package to be run correctly. A component must specify the type of runner and the needed configurations inside its manifest file. The component manager is responsible for submitting the starting of new components to the proper runner. Before submitting the request to the runner, the component manager will build a \textit{ComponentStartInfo} bundle, which contains the url of the component to be started, the content of the component package, etc. After receiving the starting request from the component manager, the runner will start the component.
\begin{itemize}
    \item \textbf{ELF Runner}: this runner is responsible for executing elf files \cite{elf}, for example, the ones generated after the compilation phase of c or rust files. 
    \item \textbf{DART AOT Runner}: this runner provides dart program \cite{dart}, with a configured dart virtual machine, to execute all bytecode generated by the compilation of the program. Most Dart programs define the UI of graphical components.
    \item \textbf{Web Runner}: the runner renders web pages to the screen of the device through the Chromium web engine \cite{chromium}.
\end{itemize}

\subsection{File System}
The Fuchsia file system is not linked or loaded by the kernel, unlike most operating systems, but it entirely lives in user-mode space. So, the file system lives in a user process, and it interacts with the other processes to provide and take files through inter-process communication primitives. This structure allows Fuchsia to execute file systems of a different kind without relying on a specific one. In most OS, in which the file system is inside the kernel, changing the file system would require the recompilation of the kernel. Instead, with the Fuchsia modular approach, each file system process can execute every kind of file system. An essential aspect of the user process file system is that every interaction to the file system does not require system call execution. Indeed, the kernel is not aware of a file system process structure, so all operation with a file system executes only in user-mode. A client process must invoke an RPC (Remote Procedure Code) exposed by the file system server to perform every kind of operation on file systems, such as open a file or store a file. fidl protocols manage the interaction between the file system process and the other processes. All interactions between a process and the file system process are carried out through channel objects at a low level. The system calls that the process calls to perform operations on file systems are restricted to only the needed ones to communicate with channels.     
\begin{itemize}
    \item \textbf{Namespace}: a namespace is an isolated environment in which all resources inside it, such as files, directories, sockets, services, etc., are visible only to processes that live in the environment and are unknown for processes that live in different namespaces. Processes external to the namespace can access resources inside the namespace only if they have the capabilities to do it. In Fuchsia, there is no concept of a global file system because every namespace has its own.
    \item \textbf{VFS}: vfs is a library that supports different kinds of operations on file system servers inside namespaces. It provides functions that simplify the interaction between a process and a file system server. Still, the letter could not use it because the unique requirement for a file system is to rely on a fidl protocol that enables the same operations between a process and the file system.
    \item \textbf{MemFS}: this kind of file system is maintained entirely in the memory of the device. For example, the bootfs protocol uses it during the booting phase of the device.
    \item \textbf{Blobfs}: file system used to store data represented through Merkle Trees \cite{merkle_tree}, also called signed data. This kind of file system is suitable for storing data that cannot be modified because it can be written only once. Fuchsia packages are stored on this kind of file system to do not allow their further modifications.
\end{itemize}

\subsection{Component Framework}
Fuchsia supports the execution of components with a set of manager programs that guide their lifecycle.
\begin{itemize}
    \item \textbf{Component Manager}: this component is at the base for the execution of components. It manages the start of all components, and for this, it is one of the first started entities. It handles the component lifecycle, from the starting to the purge of a component. It maintains the component instance tree’s topology to check the validity of certain requests sent by components. It is the core of the capability routing mechanism because it can check the validity of a certain path on the component instance tree, allowing a component to obtain a specific capability from another component.
    \item \textbf{Realm Framework}: this framework helps components to manage the creation and the handling of Realms and Collections. It provides a set of api to manage configurations of the environment in which a Realm executes, allows components to create a collection and attach component instances to it, enables capability routing for components inside the collection, etc.
    \item \textbf{Session Framework}: the component session manager is one of the most important managers in Fuchsia OS. It is responsible for creating session components and provide them with the needed capabilities. A session is a component that supports the execution of a set of sub-components linked to it. It is usually used when a meta-component needs to share resources needed from a set of components that carry out a common task. The session can
    \begin{itemize}
        \item provides capabilities (only those previously obtained from the session manager) and libraries to the underlying components
        \item define fidl protocols to enable the communication between the session itself and its children components
        \item instantiate components that will support specific fidl protocol middleware between the session and the component
    \end{itemize}
    \item \textbf{Hub}: this component can provide the state of components instances under a specific visibility scope. For example, it can show the status of all components under a specific Realm (without considering the root of the realm). Still, it does not allow the user or other components to modify the status information it exposes.
    \item \textbf{Test Framework}: this framework is used to test components. In detail, it provides a test manager that is responsible for launching component instances to test them. The test runner inside the test framework provides api, specific for the programming language used to implement the code to be run inside the component. 
\end{itemize}


% \begin{itemize}
%     \item Cosa è un component?
%     \item Component instance tree - realms - collections
%     \item Interazione tra diversi component
%     \item Protocollo FIDL per interscambio messaggi tra diversi "oggetti" in Fuchsia (tra component diversi o tra component e kernel object per esecuzione di syscall)
%     \item Isolamento e visibilità di ciasciun component
%     \item Capability Routing
%     \item File system locale al component e tipologia ========> V
%     \item Interazione con il file system e VFS layer ========> V
%     \item Pubblicazione di un package (tramite pm tool)
%     \item Zircon kernel?  ========> V
%     \item Zircon objects? ========> V
%     \item Come vengono eseguite syscall in Fuchsia
% \end{itemize}

==> Fuchsia OS/old/version_1.0/introduction.tex <==
\section{Introduction}
\label{sec:introduction}

Fuchsia is an operating system developed by Google. Google revealed the existence of this project in august 2016, releasing the source code of an initial version of this operating system on GitHub. Fuchsia OS was officially presented, for the first time, at Google I/O 2019. This operating system has a high potential not only for performance but also for its modularity. Indeed, a user can install this operating system into every device, such as pcs, smartphones, smartwatches, and IoT devices. Google thought this operating system focused on security, so it developed all principles and concepts to guarantee proper isolation of its sub-tasks. The primary purpose of Fuchsia OS is to simplify the development of applications on different kinds of devices, installing the same operating system on them. Indeed, Google is trying to unify its operating systems, such as Chrome OS \cite{chrome_os} and Android \cite{android}. Android is one of the most used operating systems \cite{os_perc}, and anyone can install it on every kind of device, such as smartphones, infotainment, smartwatches, etc. The main problem of the Android ecosystem is that the operating system is customized specifically for the kind of device in which it is installed. These specific customizations involve that a developer has to develop an application based on the type of the device. So, it has to develop the same application many times (developing an android app for smartphones is different from doing it for smartwatches, smart homes, etc.). From this practical problem born the idea to create an ecosystem in which all devices run the same operating system version, simplifying the development of applications. These properties make Fuchsia OS interesting and innovative compared to the existing solutions, which do not care about the modern idea of an ecosystem of devices. To demonstrate the applicability of Fuchsia in a real context, Google, in May 2021, released Fuchsia OS as part of a beta testing program on its Nest Hub \cite{nest_hub}. Fuchsia OS is an interesting project because it is modular and security-oriented, but is it secure?
Fuchsia OS is a very recent operating system. So, there are not works at the state of the art that try to address security issues of this operating system, and there are not research works that describe all of its mechanisms. This paper is the first paper that analyses Fuchsia from the security point of view, providing some deeper analysis on the security of this operating system. This paper describes the functioning of Fuchsia OS, providing a stack that may help represent the most important elements of the operating system, focusing on security mechanisms adopted by Fuchsia OS. In addition, the paper tries to discuss each security mechanism, giving some ideas on possible research topics on this operating system.\\
\textit{\textbf{Structure of the paper}}. The rest of the paper is organized as follows: Section \ref{sec:fuchsia_os} describes the most relevant elements of the operating system, with the help of an architectural stack and section\ref{sec:component_description} describes components structure and their interactions within the system. Section \ref{sec:securty_mechanisms} introduces security mechanisms provided by Fuchsia OS, and \ref{sec:discussion} tries to discuss these mechanisms, focusing on their strengths and weakness. Section \ref{sec:research_directions} discusses some research directions based on the analysis of security mechanisms. Section \ref{sec:conclusions} concludes the paper.



==> Fuchsia OS/old/version_1.0/research_directions.tex <==
\section{Research Directions}
\label{sec:research_directions}

This section presents some research ideas based on the analysis of security mechanisms carried out in this paper. In Fuchsia OS, a task is divided into more sub-tasks, each carried out by a specific component instance. All component instances have to interact with each other to carry out the main task. These interactions could lead to vulnerabilities, such as information leaks and the program’s execution flow changing. This interaction analysis could also be extended on the interaction between a component and kernel objects. The primary security mechanism to share access to resources are capabilities. This mechanism is critical from the security point of view because capabilities can be shared among component instances. Capabilities sharing could enable a component instance to abuse its permissions and execute not wanted operations. Fuchsia allows the developer to run its component instances inside sessions that enable sharing api and libraries between component instances, linking isolated instances. This kind of sharing could lead to vulnerabilities due to unwanted interactions between component instances. Fidl is the primary communication protocol that enables a more structured communication between different processes. So, this communication protocol is critical both for user processes interaction both for user and kernel processes interaction. A vulnerability assessment on these protocols could lead to discovering vulnerabilities exploitable on all communication between processes. All component instances are created and managed through the Realm framework. This framework is responsible for the creation and managing of realm and collections, and so, the presence of vulnerabilities in this framework could impact the security of the entire system.

==> Fuchsia OS/old/version_1.0/security_mechanisms.tex <==
\section{Security Mechanisms}
\label{sec:securty_mechanisms}

\subsection{Kernel Objects}
Zircon is an object-based kernel, which means that all its functionalities are divided among different execution units, called objects, created only when needed. These objects are interfaces between user processes and OS resources. There is an object for every kind of task that the kernel has to manage, such as inter-process-communication, execution of user code, scheduling processes, handling synchronization between threads, managing the virtual memory assigned to a process, etc. Objects are not secure by design. A user process can interact with an object through specific handlers called Handles. 
A handle is a reference to an active object. They are created when a process issues a specific system call. When a process issues a system call, the kernel eventually creates an instance of the object needed to handle the request and also all further requests regarding the task. After the execution of the system call, the kernel returns a handle to that object to the calling process. If the process executes in user mode, the handle will be an integer that indexes a table, maintained by the kernel, which contains the set of live handles and the information on the bound objects and the set of rights to access the referenced objects. The integer index is valid only within the user process context. If another process tried to use the same index to access a handle, it would access a handle that points to another object or failed because the handle would not exist. If the process executes in kernel mode, it will obtain a c++ object that contains a reference to the kernel object, the pid of the process bound to the object, the set of rights to access the objects. A handle bound to a kernel process is said in transit. Every handle is provided with a set of rights that enable specific operations on the referenced object. The rights are specific for the object, such as the permission to read or write to a channel, map vmo within the address space of the process, etc. Handles can be duplicated so that a process can take more handles to the same object. In general, a process needs to duplicate a handle to maintain handles to the same object but with a different set of rights. This mechanism is provided because a process can share its handle with another through channel or socket objects. An object can be garbage-collected only when there are no handles that reference it. So, when all handles own by processes are destroyed, also those eventually own by kernel process, the object will be garbage-collected.

\subsection{Component Isolation}
At a low level, a program is executed by a process. Fuchsia OS creates a process and gives it the minimum set of resources to start its execution. The os creates the process and provides it with the resources needed to start through the launchpad library. The launchpad library provides the process with:
\begin{itemize}
    \item a handle to a vmo that contains the executable of the program to be launched
    \item program arguments
    \item environment variables
    \item a handle to the vmo that contains the vDSO library for system call invoking
    \item handles to a local file system (namespace) and a handle to the loader service
\end{itemize}
Unlike most common os, the dynamic linking of shared libraries is carried out through vmo. Each shared library to be used is pushed inside a vmo, so when a process wants to invoke a function provided by one of the shared objects, it has to invoke the function as an RPC \cite{rpc} through a dedicated channel object. This approach is opposed to the one provided by most operating systems, in which the dynamic linker maps the shared object in the address space of the process. So, the latter can call functions provided by the shared object, through got \cite{got}, and plt \cite{plt} tables. So, each process is assigned a set of resources that only it can see and access. The process cannot access or see the resources provided by another process unless they have capabilities to do it.

\subsection{Capability Routing}
One of the most important elements of Fuchsia OS are capabilities. The interaction between components is based on capabilities exchange. Rules of Fuchsia OS rule the exchange of capabilities. Components handle the capabilities that they provide and also those that use through their manifest file. Within the manifest file, a component can specify three kinds of keywords related to the interactions with capabilities: 
\begin{itemize}
    \item \textbf{use}: this keyword specifies which capability a component could use during its execution. In detail, with this keyword, a component is allowed to use the capability provided from some other component
    \item \textbf{offer}: this keyword specifies that the component can route a certain capability to its children component instances
    \item \textbf{expose}: this keyword specifies that the component can route a certain capability to its parent in the component instance tree 
\end{itemize}
The usage of these three keywords (particularly for keywords offer and expose) enables the routing of capabilities within a component instance tree. A component instance can only see its child components. 
So, to route a capability to some other component, there must be a sequence of routing of the capability between the intermediate component instances. In detail, each component instance must offer or expose the target capability to its children, that have to do the same until it is reached the target component instance. The capability routing has to be defined statically within the manifest of components by using the keywords explained before.
\francesco{
    \begin{itemize}
        \item inserire un immagine che mostri un esempio di capability routing
    \end{itemize}
}



==> Fuchsia OS/sections/architecture.tex <==
\section{The Fuchsia Platform Architecture}
\label{sec:fuchsia_os}

%\luca{mi chiedo se qui valga la pena porre l'accento sul fatto che la proponiamo noi questa suddivisione e che non è una cosa riconosciuta - dirlo sia qua sia nell'intro}

The Fuchsia architecture consists of a stack of layers providing the OS core functionalities, as depicted in Figure \ref{fig:fuchsia_architecture}. 
The bottom layer is the Zircon Kernel. On top of it, there live four layers that manage the hardware drivers (Drivers layer), the file system (File Systems layer), the OS runtime (Fuchsia Runtime), and the software components (Component Framework). Finally, the Application Layer comprises all the user-space apps. The rest of this section briefly describes each layer.

%This section introduces the stack architecture of Fuchsia OS, as depicted in Figure \ref{fig:fuchsia_architecture}. In the following we provide a description of the major components, namely Zircon Kernel, Drivers layer, File Systems layer, Fuchsia Runtime, the Component Framework, and the User-space components. 


\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.48\textwidth]{resources/images/fuchsia_architecture.png}
    \caption{The architecture of Fuchsia OS.}
    \label{fig:fuchsia_architecture}
\end{figure}

\subsection{Zircon Kernel}

The core of Fuchsia OS is the Zircon kernel, a micro-kernel developed in C language and based on the Little Kernel project \cite{lk}.
Zircon is an object-based kernel, which means that all its functionalities are divided among different execution units, called \emph{objects} \cite{kernelObjects}, that are instantiated as needed. These objects are interfaces between user processes and OS resources. There is an object for every kind of task that the kernel has to manage, such as inter-process-communication (IPC), scheduling, and memory management.

%The core of this operating system is the Zircon kernel, a micro-kernel based on the Little Kernel project \cite{lk}.
%Little Kernel is mainly thought to adapt itself to devices with limited computational resources. So, it is suitable for the Fuchsia project that aims to be supported from as many devices as possible. 
%Compared to a standard kernel, Zircon is designed to handle fewer tasks because many elements, such as drivers and the file system, are managed by user processes. Thanks to this simplification, the number of context switches between user-mode and kernel-mode, caused by operations that the kernel code has to execute, decreases.
%\subsubsection{Kernel Objects}
%Zircon is an object-based kernel, which means that all its functionalities are divided among different execution units, called \emph{objects}, that are instantiated as needed. These objects are interfaces between user processes and OS resources. There is an object for every kind of task that the kernel has to manage, such as the inter-process-communication (IPC), the scheduling of processes, and the memory management. %, handling synchronization between threads, managing the virtual memory assigned to a process, etc.

\subsubsection{Inter-Process-Communication}

The Zircon kernel enables the communication between different isolated processes through the following mechanisms:

\begin{itemize}
    \item \textbf{Channels} are kernel objects that implement a bidirectional communication tunnel. A channel has two endpoints and each of them maintains a separate FIFO queue to store incoming messages. Components may use channels through the \texttt{libfdio} library that provides primitives to deliver and receive messages.

    \item \textbf{Sockets} are a bidirectional stream transports that enable processes to exchange data, using specific primitives. At the creation of the socket, the process can specify the in-bytes dimension of the socket.
    
    \item \textbf{FIFOs} are first-in-first-out interprocess mechanisms that exploit shared memory between processes to maintain a queue of messages. FIFOs are the most efficient mechanism in terms of I/O operations at the cost of a severely restricted buffer size.
\end{itemize}

\subsubsection{Scheduling and Synchronization}
%\cite{scheduling}
The Zircon scheduler is priority-based and relies on the LK scheduler \cite{lk}, which supports up to 32 priority levels and a different priority queue for each available CPU. Also, Zircon manages real-time threads that are allowed to run without preemption and until they block, yield, or manually reschedule \cite{scheduling}.
The main kernel objects responsible for the scheduling activities are:
\begin{itemize}
    \item \textbf{Profile}. This object allows for the definition of a set of high-level scheduling priorities that the Zircon kernel could apply to processes and threads. A single profile object could be linked with one or more processes or threads. If this is the case, the scheduler will put them at the same level.
    \item \textbf{Event}.  Event objects are generated to signal specific events for synchronization among processes.
    \item \textbf{Futex}. Futex objects are low-level synchronization primitives that offer a building block for higher-level APIs such as \texttt{pthread\_mutex\_t} and \texttt{pthread\_cond\_t}. Futex objects do not have any \texttt{right} \cite{handlesRights} associated with them.
\end{itemize}

%The Zircon kernel manages scheduling tasks for processes and threads that execute on the CPU of the device. This scheduler is based on the LK scheduler \cite{lk}, but it was extended to meet the needings of the Fuchsia OS. 

\subsubsection{Memory Management}


%Zircon supports the memory management. In particular, it relies on the concept of virtual memory \cite{virtual_memory}. Like the most common operating systems, it handles the underlying memory dividing it in pages. 
%In detail, the memory is demanded to specific kernel objects, called Virtual Memory Address Region (VMAR), that Zircon instances for each process. 
%VMARs are responsible to manage the virtual address space assigned to a process. %This property guarantees the proper isolation for the management of processes. 
%, but this can be further divided to create non-overlapping children VMAR that manage subsets of the entire address space of the process.
%A VMAR is associated with a set of permissions on the virtual address space read, write, execution. 


The Zircon kernel empowers virtual memory \cite{virtualMemory} and paging to implement memory management. The memory management task is maintained thanks to specific kernel objects that handle the virtual address space of a process and its demand for new memory pages, i.e.: 

%Zircon does not manage the overall memory of the device, but it delegates this task to a set of dedicated manager objects, called Virtual Memory Address Regions (VMARs). 

%When the kernel creates a new process, it binds it to a unique VMAR that manages its address space. Also, each VMAR can be logically divided up into any number of non-overlapping parts, each representing a child VMARs, and associated with specific file access permissions that include read, write, and execute.

%VMAR is also responsible for creating and managing specific kernel objects called Virtual Memory Object (VMO). 
%A VMO is a kernel object that abstracts and manages a set of memory pages that belong to the process. 
\begin{itemize}
    \item \textbf{Virtual Memory Object (VMO)}. The VMO is an object that allows the process to interact with the underlying memory pages, and it can also provide on-demand pages when needed. It is usually used to store dynamic libraries, provide their procedures to the process, and share memory pages between processes.
    \item \textbf{Virtual Memory Address Region}. This type of object manages the virtual address space of a process and abstracts the set of its addresses. A program starts with a single VMAR that manages the entire process address space. The single VMAR can be further divided by creating new VMARs that manage different parts of the process address space. Each VMAR has a set of rights on the underlying memory. The starting VMAR holds all the rights (read, write, execution). All VMARs created by a process are related to each other by a tree data structure.
    \item \textbf{Pager}. Pager objects are responsible for supporting data provider entities, such as file systems, to cache data they have to pass to other processes. Their main task is to create VMO objects and provide them with the pages to store data.
\end{itemize}

%Zircon kernel manages the allocation of memory to processes. Specific objects carry out all operations on the allocation and assignment of memory.

\subsection{Drivers Layer}

Fuchsia manages the interaction with the underlying hardware using user-space drivers. Such a choice i) allows relieving the Kernel from the burden of direct management, ii) increases the portability of the OS, and iii) reduces the number of context switches between user and kernel mode.

%Fuchsia OS simplifies the interaction between processes and the underlying hardware through drivers. Drivers are specific software used to abstract more complex operations on the hardware, so they provide a more convenient interface to execute the most common operations. Unlike the most common kernels, Zircon does not directly manage drivers. Indeed, to simplify the interaction between processes and drivers, avoiding a great number of user-kernel mode context switch, drivers are executed by user processes. 

To support the development of drivers, Fuchsia OS provides the Fuchsia Driver Framework. The Fuchsia Driver Framework groups a set of tools that enable a developer to create, test and deploy drivers for Fuchsia devices. One of the most important tools inside this framework is the driver manager \cite{driverFramework}. This process is one of the first started processes at the boot of the system. It is responsible for searching for the proper drivers for each device, running them, and managing their lifecycle. It allows processes to interact with drivers through a shared file system called device file system (or \texttt{devfs}), which is mounted by each component at \texttt{/dev} path. %The development of drivers is leaved to single producers. 
Although Fuchsia OS is a recent operating system, several vendors have started to implement their drivers; the implemented drivers are listed on the official page \cite{implementedDrivers}.


%\luca{qua raccontare ad alto livello che i driver sono nello user space e che possono essere implementati tramite l'utilizzo del Device Manager (se ho capito bene - includi citazione alla documentazion) inoltre fai riferimento al fatto che nella versione attuale ci sono alcuni driver già implementati come ad esempio A, B e C}

\subsection{Component Framework}
The Component Framework (CF) \cite{component} consists of the core concepts, tools, APIs, runtime, and libraries necessary to describe and run components and to coordinate communication and access to resources between components. 
The CF contains the following core services:

\begin{itemize}
    \item \textbf{Component Manager}. This process is at the core service of Fuchsia, coordinates the entire lifecycle of all components, intermediates their interactions, and manages the communication with the system resources and the underlying kernel objects. 
    It is one of the first processes created when the system boots and it is one of the last processes destroyed when the system shuts down.
    %Also the Component Manager is responsible for ensuring the isolation among processes as will be described in Section \ref{sec:securty_mechanisms}.
    %for this, it is one of the first started entities. It maintains the component instance tree’s topology to check the validity of certain requests sent by components. It is the core of the capability routing mechanism because it can check the validity of a certain path on the component instance tree, allowing a component to obtain a specific capability from another one.
%    \item \textbf{Realm Framework}: this framework helps components to manage the creation and the handling of realms and collections. It provides a set of api to manage configurations of the environment in which a Realm executes, allows components to create a collection and attach component instances to it, enables capability routing for components inside the collection, etc.

    \item \textbf{Session Manager}. The Session Manager offers component capabilities (e.g., storage, network access, and hardware protocols) to the so-called Session components. A session is a component that encapsulates a product’s user experience. It is the first product-specific component started at boot. For example, the session for a graphical product instantiates Scenic (graphics) as a child component to render its UI.
    The Session Manager handles the management of user "apps" and their composition into a user experience and handling of user input data flow.
    
    \item \textbf{Test Manager}. This service is responsible for running tests on a Fuchsia device. The Test Manager exposes the RunBuilder protocol, which allows starting test suites, launched as a child of test manager. The Test Manager supports the definition of test suites in a plethora of programming languages, including C/C++, Rust, Dart, and Go. 
    
    %responsible for launching component instances to test them. The test runner inside the test framework provides API, specific for the programming language used to implement the code to be run inside the component. 
    
    \item \textbf{Hub}. The Hub provides access to detailed structural information about component instances at runtime, such as their names, job and process ids, and exposed capabilities. For example, the Component Manager relies on the Hub to obtain information regarding the relationships among components, in order to grant the access to specific resources or capabilities.
    
    %\item \textbf{Resolvers}: resolvers are specific elements of Fuchsia OS that allow a component to resolve urls. The default urls are already resolved by default, such as fuchsia-pkg, which identifies a package inside the os, fuchsia-boot, that identifies a component within the system boot image, http, that identifies a resource available through http protocol. In addition to these url schemes, a component can specify its custom url scheme through its manifest file.
\end{itemize}



\subsection{Fuchsia Runtime}
Fuchsia provides different kinds of runtimes that can handle components. These runner processes interact with the Component Manager to load the proper configurations for a component to be run \cite{runners}. 
%They do not provide libraries, but they only start their execution, so all components must have all libraries inside their package to be run correctly. 
A component must specify the type of runner and the required configurations inside its manifest file. The Component Manager is responsible for submitting the starting of new components to the proper runner.
Fuchsia supports the use of generic and user-defined runtimes and it currently offers the following default runners:
\begin{itemize}
    \item \textbf{ELF Runner}: this runner is responsible for executing elf files, for example, the ones generated after the compilation phase of a C or Rust program. 
    \item \textbf{DART AOT Runner}: this runner executes a fully-fledged Dart Virtual Machine, to execute Dart executable files. %Most Dart programs define the UI of graphical components.
    \item \textbf{Web Runner}: the Web runner renders web pages to the screen of the device through the Chromium web engine.
\end{itemize}

To execute the component, the runner may choose a strategy such as starting a new process for the component or isolate the component within a virtual machine.

Fuchsia also includes a set of core runtime libraries that provide essential functionalities for the new processes. The core libraries include \texttt{Libc} and \texttt{vDSO} to support the execution of components and system call invocations, and \texttt{libfdio} and \texttt{VFS} to support IPC and file systems operations, respectively. 

\begin{comment}

Furthermore, the Fuchsia RuntimeThe execution of components is supported by specific libraries:
\begin{itemize}
    \item \textbf{Libc}: the libc shared library is used to support the execution of user and os programs and also the system calls provided by the kernel.
    \item \textbf{libfdio}: this shared library can be mapped by different processes and exposes functions to simplify the execution of inter-process-communication mechanisms. Indeed, the interaction between processes is generally supervised by channel objects, so it requires processes to execute specific action invoking system calls. The library abstract these operations providing an high level interface. 
    \item \textbf{VFS}: vfs is a library that supports different kinds of operations on file system servers inside namespaces. It provides functions that simplify the interaction between a process and a file system server.
    \item \textbf{vDSO}: this shared library is mapped to every processes to allow them to invoke system call. 
    \item \textbf{launchpad}: the launchpad library, is a c implemented library that support zircon kernel for the creation of a process image. 
\end{itemize}
\end{comment}

%\luca{parlare delle core libraries https://fuchsia.dev/fuchsia-src/concepts/process/core\_libraries?hl=en}

\subsection{File Systems Layer}
The Fuchsia file system is not linked nor loaded by the kernel, unlike most operating systems, but it entirely lives in user-mode space. In detail, file systems are simply user-space processes that implement servers that can appear as file systems and responds to RPC calls \cite{filesystem}.

As a consequence, Fuchsia may support multiple file systems without the burden to recompile the kernel each time. The kernel has no knowledge about files, directories, or filesystems, thus, relieving components to invoke system calls for each file operation.
Instead, the operations on a local file system are handled through the VFS library that provides the RPC primitives needed to interact with the different file system servers.
The current version of Fuchsia supports a set of predefined file systems that include MemFS, MinFS, Blobfs, ThinFs, and FVM.


%and, thus, components do not require the excution of system calls to access file resources.
%So, the file system lives in a user process, and it interacts with the other processes to provide and take files through inter-process communication primitives and RPC calls. 

%This structure allows Fuchsia to execute file systems of a different kind without relying on a specific one. 

%In most OS, in which the file system is inside the kernel, changing the file system would require the recompilation of the kernel. Instead, with the Fuchsia modular approach, each file system process can execute every kind of file system. 

%does not require system call execution (except the ones needed for interactions between the process and the file system. A client process must invoke an RPC (Remote Procedure Code) exposed by the file system server to perform every kind of operation on file systems, such as open a file or store a file.


The file system architecture allows for the definition of collections of elements, called \texttt{namespaces} \cite{namespaces}. In detail, a namespace is a per-component composite hierarchy of files, directories, sockets, services, devices, and other named objects provided to a component by its environment. 
%The items within a namespace are called objects. 
%They come in various flavors, including: Files: objects that contain binary data Directories: objects that contain other objects Sockets: objects that establish connections when opened, like named pipes Services: objects that provide FIDL services when opened Devices: objects that provide access to hardware resources


\begin{comment}
 \begin{itemize}
    %\item \textbf{VFS}: 
    \item \textbf{MemFS}: this kind of file system is maintained entirely in the memory of the device. For example, the bootfs protocol uses it during the booting phase of the device.
    \item \textbf{Blobfs}: file system used to store data represented through Merkle Trees \cite{merkleTree}, also called signed data. This kind of file system is suitable for storing data that cannot be modified because it can be written only once. Fuchsia packages are stored on this kind of file system to do not allow their further modifications.
    \item 
\end{itemize}
   
\end{comment}

%VFS is a library that supports different kinds of operations on file system servers inside namespaces. It provides functions that simplify the interaction between a process and a file system server.

\subsection{Application Layer}

%\luca{metterlo come application layer e fare la connessione tra app e components}
%\luca{cos'è un component, la sua modularità,come viene descritto (url e manifest), come viene distribuito (packages)}

This layer comprises all the user-space software, from system services to end-user apps. 
The software model of Fuchsia allows developers to design and develop their apps as a set of components which are considered the fundamental unit of an executable software. 
Components are composable, meaning that components can be selected and assembled in various combinations to create new components. A component and its children are referred to as a \texttt{realm} \cite{realm}.
The current version of Fuchsia supports the use of several programming languages for the development of apps that include C/C++, Rust, Dart, and Go, and offers a Software Development Kit (SDK) \cite{sdk} containing all the required libraries and tools to create and compile an app.
%A Component is the fundamental unit of executable software on Fuchsia and it is the core foundation of all user-space software, from system services to end-user applications. 

At its core, a component consists of the following parts:

\begin{itemize}
    \item \textbf{Component URL.} The primary use of component URLs is to uniquely identify a component in the definition of a component instance. A component URL can, in principle, have any scheme. User-space components distributed in a Fuchsia package are usually identified using the \texttt{fuchsia-pkg} schemes that specifies the repository of the package, the package name, the build variant, and the name of the manifest file. For instance, \texttt{fuchsia-pkg://fuchsia.com/stash\#meta/sta\-sh\_secure.cm} identifies the stash package located in the official fuchsia repository.
    
    \item \textbf{Component Manifest.} The manifest describes the structure of the component, such as the type of runtime to execute the component, the list of dependencies and the rules to manage the resources owned and used by component. The manifest are then compiled in a binary form that uses the \texttt{.cm} extension.
    Listing \ref{lst:example_of_component_manifest} shows the source of the component manifest file of a hello\_world app\footnote{\url{https://cs.opensource.google/fuchsia/fuchsia/+/main:examples/components/basic/meta/hello-world.cml}}. In detail the manifest specifies the type of runner (row \ref{line:runner}), the executable file (\ref{line:binary}) and the external library to include (row \ref{line:include}).
    \begin{lstlisting}[caption={Component manifest of a hello-world app.}, label={lst:example_of_component_manifest}]
    {
        include: [ "syslog/client.shard.cml" ], |\label{line:include}|
        program: {
            runner: "elf", |\label{line:runner}|
            binary: "bin/hello_world", |\label{line:binary}|
        },
    } \end{lstlisting}
    
\end{itemize}

%Components are aggregated to create applications. Indeed, a developer can create an application, dividing its functionalities in components that have to interact with each other to carry out the task. The division of an application in components allows a developer to create a modular service, that it could easily extend to add new functionalities. 

In Fuchsia, apps and system components are distributed through packages which is a distribution unit for programs, components and services \cite{packages}. 
Packages contain the set of file, separated in a specific directory structure, that enables Fuchsia OS to provide specific programs or components.

%Indeed, the Component Manager is able to start the execution pipeline for a component, picking the right package that contains all configurations and code to support the creation of the component instance. A Fuchsia device stores also system components inside a package, to properly create new component instances of them. 
\begin{comment}
Packages are signed through the merkle tree algorithm \cite{merkleTree}, to guarantee that its content could not be modified. 
Packages are uniquely identified by a url. The content of a package is separated for its typology:
\begin{itemize}
    \item \textbf{meta}: metadata information are contained within the meta.far archive. This file is the result of compressing metadata files with the far archive format \cite{far}. meta.far contains the meta directory, which contains the package file, that specifies name and version for the package, and the contents file, which support checks with for merkle tree verification of the package
    \item \textbf{non-meta files}: all files and directories outside the meta.far archive, are files needed to instance a new component instances, such as the binary of the program and eventual shared libraries
\end{itemize}
\end{comment}
%\luca{due parole sul package e da cosa è composto}


%So, Fuchsia enables developers to develop application focusing on separation of concerns. Generally, developers think components to execute small sub-tasks of the application, to ease its modularity and its further extension. 
%Components ease the work of developers on testing, because they have to test single components opposed to the entire application. 
%They also ease the reuse of code, because the same component could be used as part of other applications. An other property of components is their reliability, because if a component crashed, the crash would not impacted on the entire application, but only on a limited part of it. 

 \begin{comment}
 
%\subsubsection{Component Structure}
The component source is composed from:
    \begin{itemize}
        \item \textbf{Component Manifest Source}: this file specifies the structure of the component, such as the type of runner that has to execute the program inside the component, API exposed to the other components and rights associated to resources own by component. Listing \ref{lst:example_of_component_manifest} shows an example of component manifest source.
        \begin{lstlisting}[caption={Example of component manifest source}, label={lst:example_of_component_manifest}]
       {
          include: [ "syslog/client.shard.cml" ],
          program: {
              runner: "elf",
              binary: "bin/echo_client",
              args: [
                  "arg0",
                  "arg1",
              ],
          },
          use: [
              { protocol: "fidl.examples.routing.echo.Echo" },
          ],
       }
        \end{lstlisting}
        \item \textbf{Source code of the program}: set of source files of the program
        \item \textbf{Build file}: file that specify build configurations for source files, to compile and build the program to be run. This file is used to generate an intermediate representation file that can given in input to the Ninja \cite{ninja} build system. Listing \ref{lst:example_of_build_file} shows an example of a build file for components.
        \begin{lstlisting}[caption={Example of build file}, label={lst:example_of_build_file}]
           import("//build/components.gni")
           import("//build/rust/rustc_binary.gni")
    
           rustc_binary("echo_client") {
             edition = "2018"
             deps = [
                 "//examples/components/routing/fidl:echo-rustc",
                 "//src/lib/fuchsia",
                 "//src/lib/fuchsia-async",
                 "//src/lib/fuchsia-component",
                 "//third_party/rust_crates:anyhow",
                 "//third_party/rust_crates:futures",
                 "//third_party/rust_crates:tracing",
             ]
    
             sources = [ "src/main.rs" ]
          }
    
          fuchsia_component("echo_client_component") {
            manifest = "meta/echo_client.cml"
            component_name = "echo_client"
            deps = [ ":echo_client" ]
          }
        \end{lstlisting}
    \end{itemize}
\end{comment}     


\begin{comment}

\begin{comment}
    The session manager is a component responsible for creating session components and provide them with the needed capabilities. A session supports the execution of a set of child components. It is usually used when a component needs to share resources needed from a set of components that carry out a common task. The session can
    \begin{itemize}
        \item provide capabilities (only those previously obtained from the session manager) and libraries to the underlying components
        \item define fidl protocols to enable the communication between the session itself and its child components
        \item instantiate components that will support specific fidl protocol middlewares between the session and the component
    \end{itemize}
    \end{comment}


\subsection{Application Layer}
This paragraph groups some entities that are the basis for the developing of applications on Fuchsia OS:
\begin{itemize}
    \item \textbf{Package}: packages are archives used to 
    \item \textbf{Flutter}:
    \item \textbf{Scenic}:
\end{itemize}
\end{comment}





==> Fuchsia OS/sections/component_runtime_execution.tex <==
\section{Component Runtime Execution}
\label{sec:component_description}

Fuchsia supports the execution of software components using various runtimes, such as running them using native processes or by relying on virtual machines. Such a choice enables the execution of heterogeneous executables ranging from elf files to web pages and even Android apps \cite{fuchsiaVirtualization}.
Thanks to the component abstraction, Fuchsia is capable of transparently executing the software using the CF and its runtime. In the following, we discuss the lifecycle of a component, focusing on its interaction with other processes and the underlying OS. 

\subsection{Component Lifecycle}

The Component Manager controls the creation of components objects and their transitions through the different states of their lifecycle.
Figure \ref{fig:component_lifecycle} shows the lifecycle of a component, which is composed of five states, as described below: %\luca{https://fuchsia.dev/fuchsia-src/concepts/components/v2/introduction qui parla anche di discovered e non cita il purged}

\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.48\textwidth]{resources/images/component_lifecycle.png}
    \caption{A simplified illustration of the Component lifecycle.}
    \label{fig:component_lifecycle}
\end{figure}

\begin{enumerate}
    \item \textbf{Created.} Upon receiving a request to start a new component, the Component Manager locates its corresponding package archive, extracts the content, and creates a \texttt{ComponentStartInfo} object containing all the necessary data to execute the component.  Such information includes the URL of the component, the type of request runner, the executable arguments, and references to kernel objects needed to start the component instance. %the requested kernel objects.

    \item \textbf{Started}. After the creation of a component, the Component Manager triggers the required Runner to execute the component. The Component Manager controls the execution of a component instance by interacting with the Runner through the \texttt{ComponentController} protocol \cite{runners}.

    \item \textbf{Stopped}. Stopping a component instance terminates the component's program. Still, the Content Manager preserves the component's state by saving all the data in the persistent storage so that it can continue where it left off when subsequently restarted.
The stop event occurs if the component terminated its task or if the system is shutting down. 

    \item \textbf{Destroyed}. Once destroyed, a component instance ceases to exist and cannot be restarted. Still, it continues to exist in persistent storage.

    \item \textbf{Purged}. The Component Manager completely removes a component from the system, including all the information saved in the persistent storage.
\end{enumerate}


\subsection{Component Topology}

In Fuchsia components can assemble together to make more complex components.
At runtime, components instances, i.e., distinct embodiment of a component running, establish a set of relationships described as a \texttt{component instance tree}. Each instance contained in the component instance tree can be referred with an unique identifier called \texttt{moniker}.

A component instance (called parent or root) can build a parent-child relationship by instantiating other components, which are known as its children. Each child component instance depends entirely on the parent, and so, it lives until the parent is alive. Children can be created either statically by declaring its existence in the component manifest or dynamically, using the Realm Framework Protocol.  

Typically, an app implements its functionaries through a composition of multiple components and, thus, it has its own component instance tree. Figure \ref{fig:component_instance_tree} shows an example of a component instance tree of a sample app composed of a parent component (A) and six child components (B-G). % with realm and collection concepts.
%\luca{va aggiornata figura rimuovendo il concetto di realm e collection evidenziando invece il parent e i children}

\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.45\textwidth]{resources/images/component_instance_tree.png}
    \caption{Example of a Component Instance Tree of a Sample App.}
    \label{fig:component_instance_tree}
\end{figure}

%The usage of component instance tree helps the Component Manager to dynamically evaluating the validity of a request sent from a component instance to another within the same component instance tree. %% questo va in security


%The component instance tree describes how component instance trees are related to each other. A moniker identifies each component instance within a component instance tree. Fuchsia uses a component instance tree to express composition relationships between component instances. Indeed, a child node is part of its parent node, forming a composition relationship between them. Each child component instance depends entirely on the parent, and so, it lives until the parent is alive. The component topology is expressed through the component instance tree. 

\subsection{Inter-Component Communication (ICC)}
%\subsubsection{FIDL}
\label{subsubsection:fidl}

The Fuchsia Interface Definition Language (FIDL) \cite{fidlOverview} is a language to describe how processes communicate with each other, using high-level interfaces based on inter-process-communication (IPC) mechanisms defined by the Zircon kernel.

The adoption of FIDL allows abstracting IPC between processes, and simplifies the implementation of components as it provides a standard and language-independent way to describe the interactions. 
The FIDL language allows exposing a set of functionalities (namely, a protocol) of a component (called a Service) to other processes. At runtime, the Service publishes the protocol by starting a server that responds to IPC calls made by other processes through a client interface.

The developer of a Service can create a FIDL definition file (in \texttt{.fidl} format), which describes the protocol. Then, the FIDL toolchain generates the client and server code in any of the supported target languages, as depicted in Figure \ref{fig:fidl_arch}. The generated code needs to be included in the Service and in the external components that would use the protocol.

\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.45\textwidth]{resources/images/fidl_architecture.png}
    \caption{FIDL architecture, taken from \cite{fidlOverview}}
    \label{fig:fidl_arch}
\end{figure}

Figure \ref{lst:example_of_fidl_file} shows a snippet of a sample FIDL file. 
The example describes a protocol called Echo and a service (EchoService) that exposes an instance of Echo called \texttt{regular\_echo}. The protocol is marked as \texttt{discoverable} (row \ref{row:disco}), indicating it is available for external clients.
The Echo protocol declares a method \texttt{EchoString} that can receive a string as input (row \ref{row:input}) and respond with the same string (row \ref{row:output}).

\begin{lstlisting}[caption={Example of a FIDL file.}, label={lst:example_of_fidl_file}]
   library fuchsia.examples;

   const MAX_STRING_LENGTH uint64 = 32;

   // [START echo]
   @discoverable |\label{row:disco}|
   protocol Echo {
       EchoString(struct {
           value string:MAX_STRING_LENGTH; |\label{row:input}|
       }) -> (struct {
           response string:MAX_STRING_LENGTH; |\label{row:output}|
       });
   };
   // [END echo]

   service EchoService {
       regular_echo client_end:Echo;
   };
\end{lstlisting}


\subsection{Interaction with the OS}

User processes can interact with the underlying kernel using system calls. 
The Zircon vDSO (virtual Dynamic Shared Object \cite{vdso}) is the sole means of access to system calls in Zircon.  
The vDSO is a shared library in the ELF format provided directly by the kernel and contains all the protocols (in FIDL language) and the user-space implementation of each syscall. 
In order to use a syscall, developers need to include in their apps the \texttt{<zircon/syscalls.h>} header from the Fuchsia SDK. 

Each time a process needs to interact with a kernel object, e.g., for a system call invocation, it needs a reference to a Handle \cite{handles}.
A Handle is a kernel construct that allows user-mode programs to reference a kernel object.
Each time the Zircon kernel creates a new kernel object (as a result of a system call invocation), it returns a handle of the new object to the calling process. It is often the case that multiple processes concurrently access the same object via different handles. However, a single handle can only be either bound to a single process or to the kernel. If another process tries to use the same reference of the handle, it would access a handle that points to another object or fail because the handle would not exist.



%%%%%%%%%%%%%%%%%%%%% OLD PARTS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\begin{comment}
Fuchsia Interface Definition Language (FIDL) is a language that allows developers to write files that describe how processes communicate with each other, using high-level interfaces based on inter-process-communication (IPC) mechanisms. The usage of FIDL to abstract IPC between processes simplifies the implementation of components and lets avoid the more prone to bugs implementation through channels. The fidlc compiler compiles fidl files to produce client and server code in the language used by the components that have to interoperate, and then these files can be included within the components code. These generated codes compose the fidl binding. The figure \ref{lst:example_of_fidl_file} shows an example of a fidl file. A protocol is a fidl construct that groups different methods to specify how different components can communicate with each other. Component expose protocols to other ones through their outgoing directory. Services are group of protocols logically linked with each other. Group protocols together allows a component to expose related protocols as a unique unit. Like protocols, also services are exposed through the outgoing directory of the component. The outgoing directory is a directory inside the namespace of a component in which are put all objects that the component wants to expose to other components. 



The example in the snippet \ref{lst:example_of_fidl_file} describes the definition of the Echo protocol, and the service EchoService. The two protocols are annotated as \textit{discoverable}, so they can be exposed from the component that declares them. The Echo protocol declares three methods:
\begin{itemize}
    \item \textbf{EchoString}: the client calls this method, passing a string as input, that is received by the server, and waits for the server response. The server has to send back a string in response to the client.
    \item \textbf{SendString}: this method applies the \textit{fire and forget} model, so a client that call this method has to send a string to the server process and it does not wait for the response
    \item \textbf{$->$OnString}: this method specifies the reception of an event, so the client has to listen for an incoming event of type \textit{OnString}, that send also a string along with the event 
\end{itemize}
The last element of this file the declaration of a service. In particular, it is composed by two Echo protocol instances that can be exposed to other processes through the outgoing directory of the component.
\begin{lstlisting}[caption={Example of fidl file}, label={lst:example_of_fidl_file}]
   library fuchsia.examples;

   const MAX_STRING_LENGTH uint64 = 32;

   // [START echo]
   @discoverable
   protocol Echo {
       EchoString(struct {
           value string:MAX_STRING_LENGTH;
       }) -> (struct {
           response string:MAX_STRING_LENGTH;
       });
       SendString(struct {
           value string:MAX_STRING_LENGTH;
       });
       -> OnString(struct {
           response string:MAX_STRING_LENGTH;
      });
   };
   // [END echo]

   service EchoService {
       regular_echo client_end:Echo;
       reversed_echo client_end:Echo;
   };
\end{lstlisting}

\end{comment}


%The following will describe the lifecycle of a component and all inter process communication mechanisms provided to components to interact with each other and with the kernel. The component manager is responsible to handle the lifecycle of the component, starting from its creation. 

%Fuchsia supports the execution of software components using a variety of runtimes, such as running them using native processes or by instancing virtual machines to execute programs that belong to different operating systems. In this paper will be analyzed only the native execution of process through components. Fuchsia OS decouples the creation of the component instance from its execution. 

\begin{comment}


Fuchsia supports the execution of software components using various runtimes, such as running them using native processes or by relying on virtual machines. Such a choice enables the execution of heterogeneous executables ranging from elf files to web pages and even Android apps \cite{virtualizationAndroidLinux}.
Thanks to the component abstraction, Fuchsia is capable of transparently execting the software using the CF and its Runtime. In the following, we discuss the lifecycle of a component, focusing on its interaction with other processes and the underlying OS.


Indeed, the starting of a component is managed from a runner component. The runner is a component that communicate with the component manager to handle the component instance starting, and it helps the component manager to manage the component instance lifecycle. The interaction between the component manager and the runner component is supervised by the ComponentRunner protocol (fidl protocols described in \ref{subsubsection:fidl}). To start a new component instance, the component manager prepares a bundle called \textit{ComponentStartInfo}, containing information about the component instance to be run:
\begin{itemize}
    \item the resolved url of the component (the one obtained from a resolver)
    \item configurations taken from the program section of the component manifest source
    \item a set of mount points 
    \item the path to an outgoing directory
    \item the path to a runtime directory, in which the runner will store all running information about the component instance
    \item a set of handles to kernel objects
\end{itemize}
The runner component will start the execution of a new component instance using the information contained inside this bundle. The component manager control the execution of a component instance by interacting with the runner component through the \textit{ComponentController} protocol. For example, through this protocol, the component manager can stop the execution of a running component, submitting the request directly to the runner component. 

\subsection{Component Lifecycle}



A component has its lifecycle, which the component manager handles. Each component could listen for incoming lifecycle events, and so, they can perform tasks based on the state changed. In the following are reported the possible states for a component:
\begin{enumerate}
    \item \textbf{Create}: the component manager can create a component as the root of its component instance tree. Most of the time, starting a component is caused by the static declaration of the component inside the manifest file of another one or by dynamically adding to an existing collection. Another important reason to start a component is a binding request from a component to another one.
    % If a component wants to bind itself to another one, the component manager will check if there is a running instance of that component. If it finds a running instance, it will bind the component to the target one. Otherwise, it will create a new instance of that component and bind it to the new instance.
    \item \textbf{Start}: after the creation of a component, the component manager interacts with the required runner to execute the code inside that component. The runner will start the component, and so, this will pass it to the started state.
    \item \textbf{Stop}: a component could be stopped from the component manager because it terminated its task or when the user turns off the device. When a component passes to a stopped state, the component manager stores its state in persistent storage to eventually further restart the component.
    \item \textbf{Destroy}: when a component instance is in a destroyed state, the component manager cannot restart it, and so, it completely removes it from its component instance tree. Still, it continues to exist in persistent storage.
    \item \textbf{Purge}: the component manager completely removes a component in this state from the system. Indeed, the OS will also delete its state from persistent storage. Figure \ref{fig:component_lifecycle} shows the lifecycle of a component and all of its possible states.
\end{enumerate}



\subsubsection{Handles}
A user process can interact with kernel objects through specific handlers called Handles. A handle is a reference to an active object. They are created when a process issues a specific system call. When a process issues a system call, the kernel eventually creates an instance of the object needed to handle the request and also all further requests regarding the task. After the execution of the system call, the kernel returns a handle to that object to the calling process. If the process executes in user mode, the handle will be an integer that indexes a table, maintained by the kernel, which contains the set of live handles and the information on the bound objects and the set of rights to access the referenced objects. The integer index is valid only within the user process context. If another process tried to use the same index to access a handle, it would access a handle that points to another object or it would failed because the handle would not exist. If the process executes in kernel mode, it will obtain a c++ object that contains a reference to the kernel object, the pid of the process bound to the object, the set of rights to access the objects. A handle bound to a kernel process is said in transit.

\subsubsection{System Call Execution}
When a process invokes a system call, the Zircon kernel starts a pipeline to handle it. In most os, a process invokes a system call passing the needed arguments to registers. Then, it invokes an interrupt to allow the os to execute the system call. In Fuchsia OS, the execution of a system call has to pass several intermediate phases to be completed:
\begin{enumerate}
    \item \textbf{vDSO}: it is a shared library that declares a function for each system call. Each declared function only has to put, in eax register, the integer that corresponds to the system call that names the function. All functions accept arguments that they have to pass to the handler procedure through the calling convention for the architecture in which the os executes. This shared object is hard-coded inside the Zircon kernel code, and it is loaded in a vmo object after the system boot.
    \item \textbf{Handler}: each system call takes its arguments from specific registers. The registers’ set is different for system calls (usually statically declared in the documentation). For all system calls, the eax register is responsible for storing the integer that identifies the system call within the system. The handler is composed of instructions that have to identify the invoked system call through the content of eax register and have to fill registers according to the specific system call invoked. The handler is different for system calls and for architecture in which the os executes. 
    \item \textbf{Wrapper}: the wrapper is a code that has to invoke the right system call implementation and handles every value returned from the system call. In most common cases, system call return handles to os objects.
    \item \textbf{Implementation}: this is the true code that execute the system call
\end{enumerate}
System call handlers and wrappers are automatically generated by a tool called kazoo \cite{kazoo}. Kazoo bases the generation of a specific pair of handler and wrapper on a fidl source file. The fidl source specifies input arguments to the system call and possible output values. In general, every kernel object has its fidl source \cite{vdso}, which declares all system calls related to that object. The fidl source is compiled with the fidlc compiler, which generates a json file as an intermediate representation. This json file is given in input to the kazoo tool, which generates the handler, a c++ source that relies on the specific architecture of the device.
% \subsection{Starnix Project}
% Recently Google started to work on a side project called Starnix \cite{starnix}, which aims to allows Fuchsia to execute native android and linux applications. Indeed, Fuchsia provides a virtualization service to run external applications, with the overhead caused by the execution on virtual machines. Hence, the idea behind Starnix is to allow Fuchsia to emulate system call invocation and api calls, similarly to the wsl 1 \cite{wsl1}, to guarantee the complete execution of programs written for other contexts. 


\end{comment}

==> Fuchsia OS/sections/discussion_new.tex <==
\section{Discussion and Conclusion} % and Conclusion}
\label{sec:discussion}

This paper describes the architecture of Fuchsia OS and its software model, and focuses on the security mechanisms implemented to guarantee a secure execution of apps inside the system. 

Despite being in an early stage of development, Fuchsia exploits a complex set of security features that include sandboxing of processes and components, the use of capabilities, and a specific focus on ICC and on the interaction with the underlying Zircon micro-kernel.
Such design enables Fuchsia to run all the software, including apps and system components, with the least privilege it needs to perform its job and gains access only to the information it needs to know. 

Still, the preliminary security analysis carried out in this work allowed us to unveil some promising research directions that could enhance the overall security of the OS or contribute to the finding of potential security weaknesses.

%%% the problem of ICC
For instance, the complexity of the layered architecture and the ICC communication mechanisms could lead to unexpected communication flows among the different layers of the Fuchsia stack. %, as the one witnessed in the Android OS \cite{armando2013breaking}.
In particular, we noticed that the Realm Framework allows for the creation of groups of components, called \texttt{collections}, that are hierarchically organized and, thus, can benefit from the capability routing mechanism. In such a case, each capability routed to a component of a collection is automatically extended to all the other members \cite{realm}. This choice could break the principle of least privilege, and lead to grant unnecessary capabilities to one or more components. 

Also, we identified several bottlenecks and critical points in the architecture whose compromise could severely affect the integrity and the availability of the system. A notable example is the Component Manager, which is in charge of handling the lifecycle of components and the capability routing of the entire system.

%% integrità dei pacchetti - in sintonia con Android

Finally, we noticed that the package verification mechanisms enable the protection against modifications that would invalidate the signature of the content. As it happens in the Android ecosystem, however, packages are not resilient to repackaging attacks that also involve the re-signing of the tampered file. % \cite{armandroid}. 
In such a scenario, Fuchsia can be targeted with malicious repackaged apps, as well. % that could harm the security and privacy of the entire system.

Thus, future extensions of this work include i) an in-depth analysis of the ICC, with a particular focus on intra-layer and inter-layer communications, and ii) the design of an integrity protection mechanisms for Fuchsia apps that could mitigate repackaging attacks.

\begin{comment}


Still, the preliminary security analysis carried out in this work allowed us to unveil some promising research directions that could enhance the security posture of the OS or find potential security weaknesses.
%%% the problem of ICC
For instance, the complexity of the layered architecture and the ICC communication mechanisms could lead to unexpected communication flows among the different layers of the Fuchsia stack, as the one witnessed in the Android OS \cite{armando2013breaking}.
In particular, we noticed that the Realm Framework allows the creation of groups of components, called collections, that are hierarchically organized and, thus, can benefit from the capability routing mechanism. In such a case, every capability routed to a component of a collection is automatically extended to all the other members \cite{realm}. This choice could break - in principle - the paradigm of least privilege, granting unnecessary capabilities to one or more components. 

Also, we identified several bottlenecks and critical points in the architecture whose compromise could severely affect the integrity and the availability of the system. A notable example is the Component Manager, which is in charge of handling the lifecycle of components and the capability routing of the entire system.

%% integrità dei pacchetti - in sintonia con Android\textbf{}

\end{comment}

==> Fuchsia OS/sections/fuchsia_os.tex <==
\section{Fuchsia OS}
\label{sec:fuchsia_os}
This section presents the stack of Fuchsia OS, describing the composing elements of the architecture stack

\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.35\textwidth]{resources/images/fuchsia_architecture.png}
    \caption{Fuchsia Architecture}
    \label{fig:fuchsia_architecture}
\end{figure}

\subsection{Zircon}
The core of this operating system is the Zircon kernel. Zircon is a micro-kernel based on the Little Kernel project \cite{lk} to guarantee high performances on all kinds of devices, from IoT devices to smartphones and pcs. Little Kernel is mainly thought to adapt itself to devices with limited computational resources. So, it is suitable for the Fuchsia project that aims to be supported from as many devices as possible. Compared to a standard kernel, Zircon has to handle fewer tasks because many elements, such as drivers and the file system, are managed by user processes. Thanks to this simplification, the number of context switches between user-mode and kernel-mode, caused by operations that the kernel code has to execute, decreases.

\subsubsection{Kernel Objects}
Zircon is an object-based kernel, which means that all its functionalities are divided among different execution units, called objects, created only when needed. These objects are interfaces between user processes and OS resources. There is an object for every kind of task that the kernel has to manage, such as inter-process-communication, execution of user code, scheduling processes, handling synchronization between threads, managing the virtual memory assigned to a process, etc.

\subsubsection{IPC}
Zircon kernel manages inter-process communication (IPC) between different processes and allows them to communicate although isolated in memory.
\begin{itemize}
    \item \textbf{Channel}: this object implements a bidirectional communication channel. A channel has two endpoints, and each of them maintains a separate fifo queue to store incoming messages. %Every channel endpoint has an owner that also marks all messages sent and received by the endpoint, and only it can access these messages. 
    They provide user code with primitives to add messages to the queue of the recipient process and to read them, and so, to dequeue them.
    \item \textbf{Socket}: this object implements a bidirectional communication channel. Processes can read and write data through their socket endpoints, using socket primitives. At the creation of the socket, the process can specify the in-bytes dimension of the socket.
    \item \textbf{FIFO}: objects thought to support shared memory between processes. They are more efficient than socket and channel objects in terms of timing to complete io operations, but they have a more limited buffer size.
\end{itemize}

\subsubsection{Scheduling \& Synchronization}
The Zircon kernel manages scheduling tasks for processes and threads that execute on the cpu of the device. This scheduler is based on the LK scheduler \cite{lk}, but it was extended to meet the needings of the Fuchsia OS. Together with scheduling tasks, Zircon also supports signal primitives to allow synchronization between different threads.
\begin{itemize}
    \item \textbf{Profile}: this object defines a set of priorities for scheduling configurations that the zircon kernel could apply to processes and threads. A single profile object could be linked with more processes and threads, and in this case, the scheduler will put them at the same level.
    \item \textbf{Event}: these objects are created to signal specific events for synchronization between processes.
    \item \textbf{Futex}: objects that manage synchronization between processes at a low level and in user-mode. They are the basis for \textit{pthread\_mutex} and \textit{pthread\_cond}, that are higher-level primitives. Futex objects do not provide rights to access to primitives that they expose because the base operations are \textit{wait} and \textit{wake} that have to be both accessible to leverage the basic functionalities of the object. Futexes does not support priority for the calling processes, but they provide some API to allow further implementations of it. 
\end{itemize}

\subsubsection{Memory Management}
Zircon kernel manages the allocation of memory to processes. Specific objects carry out all operations on the allocation and assignment of memory.
\begin{itemize}
    \item \textbf{Virtual Memory Object (VMO)}: an object that represents a region of virtual memory that can be shared among different processes. This object allows a process to perform several operations, such as reading, writing to the mapped pages. The vmo is a high-level infrastructure that allows the process to interact with the underlying memory pages, and it can also provide on-demand pages when needed.
    \item \textbf{Virtual Memory Address Region}: these objects represent a continuous set of addresses taken from a virtual address space. When a program executes, it has only a single vmar that contains all addresses of the program’s virtual address space, but it could be further divided with the creation of new vmar that do not overlap themself in their address space. Each vmar has a set of rights on the underlying memory. The starting vmar has all rights (read, write, execution) on the underlying memory. When a process makes a system call to partition an existing vmar further, it can also specify the set of permissions for the new vmar. All vmar created by a process are related to each other by a tree data structure. In detail, a parent vmar maintains a reference to its children vmar, and this does not allow the destruction of a child vmar though there are no handles to it in the processes.
    \item \textbf{Pager}: these objects are responsible for supporting data provider entities, such as filesystems, to cache data they have to pass to other processes that request them. Their main task is to create vmo objects and provide them the needed pages to store data from the data provider.
\end{itemize}

\subsection{Fuchsia Runtime}
Fuchsia provides different kinds of runtimes that can start components. These runner processes communicate with the component manager to obtain configurations for a program to be run. Their main task is to read configurations sent from the component manager to start executing new components. They do not provide libraries, but they only start their execution, so all components must have all libraries inside their package to be run correctly. A component must specify the type of runner and the needed configurations inside its manifest file. The component manager is responsible for submitting the starting of new components to the proper runner.
\begin{itemize}
    \item \textbf{ELF Runner}: this runner is responsible for executing elf files \cite{elf}, for example, the ones generated after the compilation phase of c or rust files. 
    \item \textbf{DART AOT Runner}: this runner provides dart program \cite{dart}, with a configured dart virtual machine, to execute all bytecode generated by the compilation of the program. Most Dart programs define the UI of graphical components.
    \item \textbf{Web Runner}: the runner renders web pages to the screen of the device through the Chromium web engine \cite{chromium}.
\end{itemize}

\subsection{File System}
The Fuchsia file system is not linked or loaded by the kernel, unlike most operating systems, but it entirely lives in user-mode space. So, the file system lives in a user process, and it interacts with the other processes to provide and take files through inter-process communication primitives. This structure allows Fuchsia to execute file systems of a different kind without relying on a specific one. In most OS, in which the file system is inside the kernel, changing the file system would require the recompilation of the kernel. Instead, with the Fuchsia modular approach, each file system process can execute every kind of file system. An essential aspect of the user process file system is that every operation on file systems does not require system call execution (except the ones needed for interactions between the process and the file system. A client process must invoke an RPC (Remote Procedure Code) exposed by the file system server to perform every kind of operation on file systems, such as open a file or store a file.
\begin{itemize}
    \item \textbf{Namespace}: a namespace is an isolated environment in which all resources inside it, such as files, directories, sockets, etc., are visible only to processes that live in the environment and are unknown for processes that live in different namespaces. In Fuchsia, there is no concept of a global file system because every namespace has its own.
    \item \textbf{VFS}: vfs is a library that supports different kinds of operations on file system servers inside namespaces. It provides functions that simplify the interaction between a process and a file system server.
    \item \textbf{MemFS}: this kind of file system is maintained entirely in the memory of the device. For example, the bootfs protocol uses it during the booting phase of the device.
    \item \textbf{Blobfs}: file system used to store data represented through Merkle Trees \cite{merkle_tree}, also called signed data. This kind of file system is suitable for storing data that cannot be modified because it can be written only once. Fuchsia packages are stored on this kind of file system to do not allow their further modifications.
    \item \textbf{Outgoing Directory}: the outgoing directory is a directory inside the namespace of a component in which are put all objects that the component wants to expose to other components 
\end{itemize}

\subsection{Component Framework}
Fuchsia supports the execution of components with a set of manager programs that guide their lifecycle.
\begin{itemize}
    \item \textbf{Component Manager}: this process is at the base for the execution of components. It manages the lifecycle of all components, and for this, it is one of the first started entities. It maintains the component instance tree’s topology to check the validity of certain requests sent by components. It is the core of the capability routing mechanism because it can check the validity of a certain path on the component instance tree, allowing a component to obtain a specific capability from another one.
    \item \textbf{Realm Framework}: this framework helps components to manage the creation and the handling of realms and collections. It provides a set of api to manage configurations of the environment in which a Realm executes, allows components to create a collection and attach component instances to it, enables capability routing for components inside the collection, etc.
    \item \textbf{Session Framework}: the component session manager is a component responsible for creating session components and provide them with the needed capabilities. A session supports the execution of a set of child components. It is usually used when a component needs to share resources needed from a set of components that carry out a common task. The session can
    \begin{itemize}
        \item provide capabilities (only those previously obtained from the session manager) and libraries to the underlying components
        \item define fidl protocols to enable the communication between the session itself and its child components
        \item instantiate components that will support specific fidl protocol middlewares between the session and the component
    \end{itemize}
    \item \textbf{Hub}: this directory inside a file system stores the state of component instances under a specific visibility scope. For example, it maintains the status of all components under a specific Realm (without considering the root of the realm). A process cannot modify files inside the hub directory, but only read them.
    \item \textbf{Test Framework}: this framework is used to test components. In detail, it provides a test manager that is responsible for launching component instances to test them. The test runner inside the test framework provides api, specific for the programming language used to implement the code to be run inside the component. 
    \item \textbf{Resolvers}: resolvers are specific elements of Fuchsia OS that allow a component to resolve urls. The default urls are already resolved by default, such as fuchsia-pkg, which identifies a package inside the os, fuchsia-boot, that identifies a component within the system boot image, http, that identifies a resource available through http protocol. In addition to these url schemes, a component can specify its custom url scheme through its manifest file.
\end{itemize}

\subsection{Application Layer}
This paragraph groups some entities that are the basis for the developing of applications on Fuchsia OS:
\begin{itemize}
    \item \textbf{Package}: packages are archives used to 
    \item \textbf{Flutter}:
    \item \textbf{Scenic}:
\end{itemize}

==> Fuchsia OS/sections/introduction.tex <==
\section{Introduction}
\label{sec:introduction}

Fuchsia is an open-source operating system developed by Google that prioritizes security, updatability, and performance \cite{fuchsiaOverview} with the aim to support a wide range of devices, from embedded systems to smartphones, tablets, and personal computers. 

Fuchsia tries to overcome Google's end-user-facing operating systems, e.g., Chrome OS \cite{chromeOs}, Android \cite{android}, Wear OS \cite{wearOs}, and Google Home \cite{googleHome} by providing a unique OS for a wide range of devices and application scenarios.
The new OS first appeared in August 2016 in a GitHub repository, while the first official appearance was during the Google I/O 2019 event \cite{googleIo2019}.
To demonstrate the applicability of Fuchsia in a real context, in May 2021 Google released Fuchsia OS as a part of a beta testing program on its Nest Hub devices \cite{nestHub}.

The main purpose of the Fuchsia OS is to simplify the development of applications (hereafter, apps) on different kinds of devices by supporting multiple application environments.
In Fuchsia, a \texttt{component} is the common abstraction that defines how each piece of software (regardless of source, programming language, or runtime) is described and executed on the system \cite{component}. Developers can design apps as a set of components that can run in independent runtime environments, called Runners. A \texttt{Runner} can either execute binary files, render web pages, or run compiled code inside a virtual machine.
%Components communicate with each other through FIDL, which is the language that Fuchsia uses to describe interprocess communication (IPC) protocols of components that run on Fuchsia. %%da valutare se tenere
Finally, each app is distributed through a platform-independent archive, called \texttt{Package}, that includes all the required dependencies to compile and execute the software.
%\luca{dire che gli sviluppatori quindi creano generici componenti, che vengono distrubuiti tramite package e che poi è il sistema operativo che si occupa di compilarsi il codice per l'architettura e il runtime corretti}

Such an approach aims to overcome the jeopardization of commercial OSes, like Android, where vendor-specific distributions and heterogeneous hardware configurations boost the complexity in the development of apps. %\cite{impactAndroidCustomization}.

Also, the architectural design goals of Fuchsia involve a security-oriented design that adopts the principle of least privilege and introduces security mechanisms such as \texttt{process and component isolation} (called \emph{sandboxing}), \texttt{namespaces}, and \texttt{capabilities routing} \cite{fuchsiaSecurity}.
Thus, each piece of software running on the system, including apps and system components, executes in a separated environment having the minimum set of capabilities required to perform its task. %, and it is granted access only to the minimal bunch of data.

%This article is the first research effort that tries to unmask the complexity of the security of Fuchsia OS by providing an in-depth analysis of the OS architecture and its security mechanisms. Additionally, we conclude with an overall discussion of the security posture of the OS, and we identify several research opportunities that could enhance the security of the Fuchsia environment.

This article discusses the basic of Fuschia OS and its software model, with a specif focus on the security mechanisms introduced so far to protect both the OS and the apps. 
%In detail of the security of Fuchsia OS by providing an in-depth analysis of the OS architecture and its security mechanisms. Additionally, we conclude with an overall discussion of the security posture of the OS, and we identify several research opportunities that could enhance the security of the Fuchsia environment. \luca{rifrasare un attimo}
In detail, this paper provides: 
\begin{itemize}
\item a detailed description of the Fuchsia OS architecture and its software model by analyzing both the official documentation \cite{officialDocs} and the source code repository \cite{fuchsiaRepository}, updated on August 2021 (i.e., the release $f5$).
%\footnote{Master Branch at commit f2672a246302546cb4d7283e6916f4dcfd7ab3cb}.    
\item an in-depth analysis of the core security mechanisms implemented in Fuchsia. 
\item a discussion on the security posture of the OS, identifying some research opportunities that could enhance the security of the Fuchsia ecosystem or contribute to the finding of security weaknesses.
    %\item We will release \toolname{} after the acceptance of the paper. 
\end{itemize}



\textit{\textbf{Organization}}. 
The rest of the paper is organized as follows: Section \ref{sec:fuchsia_os} presents the Fuchsia platform architecture and the software model, while Section~\ref{sec:component_description} describes the runtime behavior of apps (and components) and their interactions within the system. 
Section~\ref{sec:securty_mechanisms} provides an in-depth analysis of the security mechanisms of Fuchsia. Finally, Section~\ref{sec:discussion} provides a discussion highlighting the strengths and possible weaknesses of the OS and points out some future research directions.


\begin{comment}
Fuchsia is an operating system developed by Google. Google revealed the existence of this project in august 2016, releasing the source code of an initial version of this operating system on GitHub. Fuchsia OS was officially presented, for the first time, at Google I/O 2019. This operating system has a high potential not only for performance but also for its modularity. Indeed, a user can install this operating system into every device, such as pcs, smartphones, smartwatches, and IoT devices. Google thought this operating system focused on security, so it developed all principles and concepts to guarantee proper isolation of its sub-tasks. The primary purpose of Fuchsia OS is to simplify the development of applications on different kinds of devices, installing the same operating system on them. Indeed, Google is trying to unify its operating systems, such as Chrome OS \cite{chrome_os} and Android \cite{android}. Android is one of the most used operating systems \cite{os_perc}, and anyone can install it on every kind of device, such as smartphones, infotainment, smartwatches, etc. The main problem of the Android ecosystem is that the operating system is customized specifically for the kind of device in which it is installed. These specific customizations involve that a developer has to develop an application based on the type of the device. So, it has to develop the same application many times (developing an android app for smartphones is different from doing it for smartwatches, smart homes, etc.). From this practical problem born the idea to create an ecosystem in which all devices run the same operating system version, simplifying the development of applications. These properties make Fuchsia OS interesting and innovative compared to the existing solutions, which do not care about the modern idea of an ecosystem of devices. To demonstrate the applicability of Fuchsia in a real context, Google, in May 2021, released Fuchsia OS as part of a beta testing program on its Nest Hub \cite{nest_hub}. Fuchsia OS is an interesting project because it is modular and security-oriented, but is it secure?
Fuchsia OS is a very recent operating system. So, there are not works at the state of the art that try to address security issues of this operating system, and there are not research works that describe all of its mechanisms. This paper is the first paper that analyses Fuchsia from the security point of view, providing some deeper analysis on the security of this operating system. This paper describes the functioning of Fuchsia OS, providing a stack that may help represent the most important elements of the operating system, focusing on security mechanisms adopted by Fuchsia OS. In addition, the paper tries to discuss each security mechanism, giving some ideas on possible research topics on this operating system.
\end{comment}



==> Fuchsia OS/sections/security_mechanisms.tex <==
\section{Security Mechanisms}
\label{sec:securty_mechanisms}

%This section describes some of the most important securitymechanisms  used  by  Fuchsia  OS  to  guarantee  the  secureexecution  of  components  and  of  the  interactions  betweenprocesses and kernel objects

This section describes the main security mechanisms used by Fuchsia OS to guarantee the secure execution of components and apps, as well as the correct interaction with the kernel primitives.

\subsection{Zircon Kernel Security}

The Zircon kernel is designed to fully isolates processes by default and regulates access to its functionalities by enforcing restrictions on Objects and Handles. Also, it supports the generation of secure pseudo-random numbers and it is declared as strongly hardened against buffer overflow attacks. 
%\luca{non sono sicuro mi piacca come frase}

\subsubsection{Kernel Objects \& Handles Rights}

The usage of kernel objects and Handles enables Zircon to apply fine-grained control over the processes and their ability to interact with the kernel functionalities.

First, the concept of kernel object grants a separation of concerns that enables isolated and containerized kernel tasks. Also, the objects are created and disposed upon need, thus limiting the probability of interacting with unused or de-referenced objects. 

Then, user-space processes are able to interact with kernel objects only through Handles. Each Handle is bound only to a specific process, and the kernel generates it in response to a system call. Thus, a process is not expected to interact with a kernel object unless it has a valid Handle.
This approach aims to reduce the attack surface only to those objects owned by the process. 
For example, suppose an attacker gained access to a VMAR object through a Handle owned by a given process. 
In that case, she can only interact with the virtual address space of that process, but she is not expected to be able to propagate the attack on the virtual address space of other processes or the kernel. 

Finally, Handles can inherit a number of rights \cite{handlesRights} that describe the set of operations allowed on the kernel object (i.e., the system call that the process can invoke with the Handle). This mechanism allows the kernel to differentiate the access to the same object (e.g., a Channel object) on a per-process basis.
Also, even though a process can duplicate and maintain different Handles referring to the same object, each copy could have at most the same rights as the original one, granting the least privilege.


\begin{comment}
Objects are not secure by design, so every handle to kernel object is provided with a set of rights that enable specific operations on the referenced object. The rights are specific for the object, such as the permission to read or write to a channel, map vmo within the address space of the process, etc. The set of all possible rights is documented inside the Fuchsia documentation page \cite{handlesRights}. Handles can be duplicated so that a process can take more handles to the same object. In general, a process needs to duplicate a handle to maintain handles to the same object but with a different set of rights. This mechanism is provided because a process can share its handle with another through channel or socket objects. An object can be garbage-collected only when there are no handles that reference it. So, when all handles own by processes are destroyed, also those eventually own by kernel process, the object will be garbage-collected.

The usage of kernel objects enables the kernel to apply separation of concerns to tasks provided by zircon. Each object manages a task, also specific for a process, such as vmo and vmar. So, zircon kernel is principally an object manager and a system call handler. This separation of tasks allows the kernel to isolate its critical functions on the system. For example, if an attacker gained the control of a user process and of handles that it own, it could issue commands to objects, according to the rights provided to the handle, but the attack would be limited only to the object itself, and it would not propagate to other objects. The main idea is that a process cannot access to objects of which it has not the handle, so limiting the attack surface. Another important feature of objects, is that in most critical cases, the kernel responds to a system call issue creating a specific object instance and bound it to the process. Using this approach, critical objects, such as vmar and vmo, are only linked to a specific process, and not to a set of them. This approach protects the system in case an attacker would gain the control of a process, because the attack surface will be limited only to those objects own by the process. For example, if an attacker gained the access to a vmar object through an handle own by a process, it could do only operation on the virtual address space of that process, and it cannot propagate the attack on virtual address space of other processes. 

Providing a set of rights to a specific handle, improve the security level of the system, because a process that owns an handle can only perform a limited set of operations on that object. The security mechanism enables the secure sharing of handles between processes. Indeed, when a process wants to pass an handle to another process, it can duplicate it and eventually reduce the set of permissions assigned to the duplicated one, limiting the set of possible operations that the target process could do. A possible best practice to secure the access to kernel objects is to implement a least privilege approach on the rights of objects. Indeed, a process can change rights assigned to a handle, being able to specify only the minimum set of rights, needed to execute its task. This approach can prevent an attacker to leverage specific rights to execute non-authorized operations on objects referenced by handles own by the process.
\end{comment}

\subsubsection{Kernel Code Hardening}
%Fuchsia uses the Clang/LLVM compiler \cite{clang} to build the Zircon kernel to enforce two security features called SafeStack \cite{safeStack} and ShadowCallStack \cite{shadowCallStack}. 
The Zircon kernel is compiled using the Clang/LLVM compiler \cite{clang} with the SafeStack \cite{safeStack} and ShadowCallStack \cite{shadowCallStack} security options enabled.

SafeStack and ShadowCallStack provide the running program with two stacks: a safe stack and an unsafe one. The unsafe stack is similar to the standard stack, so it can store references to objects on the heap memory, while the safe stack is reserved for the function call stack.

Such mechanisms aim to protect the Zircon kernel against stack-smashing attacks \cite{bufferOverflow}.  In such a case, a buffer overflow attack targeting a runtime variable in the program cannot overwrite the return addresses of the function call stack since it is located in a separated memory region.
Also, Fuchsia extends such protection to all user programs developed in C by providing Clang as the default compiler.


\begin{comment}

The shadow-call-stack compiler option is similar to the safe-stack one. The shadow-call-stack options provide the program with a standard stack and a shadow call stack. The latter stack is used to store return address of each function call within the program. So, the separation between the stack that contains program variables and the one that contains function call return addresses, allows the program to be protected against buffer-overflow attacks.

such as buffer-overflows , since an overflprogram runtime data cannot overwrite the return addresses of the function call stack that is located in separate.

space. separated in two different stack, and the return address cannot be overwritten by a buffer-overflow attack from a buffer inside a unique stack.

SafeStack is a compiler option for clang compiler, that enables a more secure compilation to protect the compiled program against stack-smashing attacks, such as buffer-overflows \cite{bufferOverflow}. The safe-stack option provides the running program with two stack: a safe stack and an unsafe one. The unsafe stack is similar to the standard stack, so it can store references to objects on the heap or local variables, while the safe stack is used to store the return address of the calling function. This mechanism prevents buffer-overflows since program runtime data and the return address are separated in two different stack, and the return address cannot be overwritten by a buffer-overflow attack from a buffer inside a unique stack. The shadow-call-stack compiler option is similar to the safe-stack one. The shadow-call-stack options provide the program with a standard stack and a shadow call stack. The latter stack is used to store return address of each function call within the program. So, the separation between the stack that contains program variables and the one that contains function call return addresses, allows the program to be protected against buffer-overflow attacks.


. The usage of Clang enables Fuchsia to leverage all security mechanisms for programs compilation provided by the compiler, such as SafeStack \cite{safeStack} and ShadowCallStack \cite{shadowCallStack}. 

Both techniques enable the protection of the return addresses on the stack from being overwritten through memory vulnerabilities, such as buffer overflows \cite{bufferOverflow}.
\end{comment}

\subsubsection{Secure Pseudo-random Number Generation}

Fuchsia OS supports the secure generation of random numbers directly by the Zircon kernel exploiting the \texttt{zx\_cprng\_draw} system call \cite{draw}. 
The generation of a random number uses the Chacha20 \cite{chacha20} cryptographic algorithm.
This algorithm requires a key and an integer nonce. The nonce passed to this algorithm is incremented after each invocation of the draw system call. 
The seed, instead, is generated by an entropy function. Unlike other operating systems, in Fuchsia OS the kernel generates entropy without relying on the device driver. Such a choice depends on the fact that drivers run in user mode and, thus, they cannot be trusted in principle. The kernel ensures a frequent update of the seed value by generating a new number every 30 minutes.

\begin{comment}
Fuchsia OS supports the secure generation of random numbers through dedicated system calls. The generation of random numbers is cryptographically secure through the invocation of the draw system call. Unlike other operating systems, in Fuchsia OS, the entropy generation is trusted only from the kernel, because drivers executes in usermode, so they cannot be trusted. The generation of random number, is based on the Chacha20 \cite{chacha20} cryptographic algorithm. This algorithm requires a key and an integer nonce. The nonce passed to this algorithm is incremented every time that is invoked the draw system call. The seed of the random number is updated though the addEntropy system call. To secure the generation of random number, the seed must be updated very frequently, so the kernel creates a thread every 30 minutes to update the seed. The random number generator can be used for many purposes, such as the randomization of the program stack initial address (ASLR) to secure the execution of programs. 
\end{comment}

\subsection{Sandboxing}

Sandboxing is a security mechanism to isolate programs from each other at runtime. Fuchsia enforces sandboxing by executing all programs inside their isolated environment with the minimal set of rights needed to execute. %, thereby enforcing the least privilege.
In Fuchsia, each newly created process is isolated and does not possess any privilege, i.e., it cannot access kernel objects, allocate memory, or execute code \cite{generalSandboxing}. 
After the creation, the OS assigns the process with a minimum set of handles and resources to be allocated for the execution of a program.

Depending on the runtime environment, a program can run using different strategies, like being executed in a separated process or launched inside a separate Dart Virtual Machine hosted by a process. The component does not always correspond to a Zircon process, as documented in \cite{runners}.
Thus, Fuchsia enforces the sandboxing also at the granularity of single components.
 
\subsubsection{Namespace}
The main principle that enables component isolation is the namespace. 
Unlike other operating systems, Fuchsia does not have a "root" filesystem.
Instead, the Component Manager provides each component with one or more namespaces tailored to their specific necessities. 
The component has complete control over the assigned namespaces and runs as its own private "root" user.

The absence of users and a global root namespace makes impossible privilege escalation attacks \cite{privilegeEscalation}. 
Indeed, if an attacker takes control of a process, she would only have access to the component's resources, as Object paths (e.g., Handles and files) may not be meaningful outside the namespace boundaries.
To further enforce segregation among namespaces, Fuchsia has disabled the Dot Dot command \cite{dotdot} to prevent path traversal attacks \cite{pathTraversal}.
Components can access namespaces belonging to different components - with the granularity of a directory and its sub-directories - only through IPC mechanisms that are protected with access control mechanisms (see Sections \ref{sec:cap} and \ref{sec:cap-rout}). 


\begin{comment}

At a low level, a program is executed by a process. Fuchsia OS creates a process and gives it the minimum set of resources to start its execution. The os creates processes inside a component and provides them with the resources needed to start through the launchpad library. The launchpad library provides the process with:
\begin{itemize}
    \item a handle to a vmo that contains the executable of the program to be launched
    \item program arguments
    \item environment variables
    \item a handle to the vmo that contains the vDSO library for system call invoking
    \item handles to a local file system and a handle to the loader service
\end{itemize}
Unlike most common os, the dynamic linking of shared libraries is carried out through vmo objects. Each shared library to be used is pushed inside a vmo, so when a process wants to invoke a function provided by one of the shared objects, it has to invoke the function as an RPC \cite{rpc} through a dedicated channel object. To each process is assigned a set of resources that only it can see and access. The process cannot access or see the resources provided by another process unless they have capabilities to do it. The main principle that enable the component isolation is namespace. Component manager provides each a component with a namespace. Fuchsia OS has not a single file system, but each component has its own. The absence of a shared file system simplifies the adoption of security mechanisms to protect a component file system. Indeed, in most common operating systems, the concept of user is important to manage access to specific files or directory of the common file system. The user can access only to those files that it owns or those for which it has permissions gave from owners. This mechanism is important to manage he access of files that belong to different users and that are stored on the same physical file system. The isolation of file systems for components deletes the needing for users. Indeed, a process inside a component has all privileges to access files in its namespace, because all files belong to it. 

\subsubsection{Sandboxing of Components}
In Fuchsia OS, all programs execute inside their isolated environment or component. A process inside a component can only see resources that belong to the component, and only those own by other components of which it has the capabilities to access. So, the fact that all components are isolated between each other and that can see only their child components, improves the security level of the system compared to the most common os, in which processes are isolated between each other, but they can access to the same resources, such as the same file system. In Fuchsia OS, the set of shared resources is limited to hardware, zircon kernels, drivers. Each component has its own file system, so the attack surface is reduced respect to the common os, and most of the attacks that involve the access of a shared file system between processes, is not applicable on Fuchsia OS. In Fuchsia there is not the concept of user, because a process can access only to the limited resources provided by its component, so a process has all rights to access resources within the component, included files on the local file system. The absence of users makes impossible privilege escalation attacks. The isolation provided by components protect the system in case an attacker would take the control of a process inside a component. Indeed, if an attacker took the control of a process, it would have
access and modify only to resources inside the component, in particular only to files inside the local file system of the component and those stored in other components for which it has the capabilities to access. So, exploiting a vulnerability inside a component, compromises the execution flow only of that component, and does not propagate to others.

\end{comment}

\subsection{Capabilities}
\label{sec:cap}

Fuchsia is a \textsl{capability-based} operating system. A \texttt{capability} is a token defining how components can interact with system resources and other components. Only the possession of the appropriate capability enables a component to access the corresponding resource. 

Fuchsia capabilities are classified into seven types \cite{capList}, namely $Directory$, $Event$, $Protocol$, $Resolver$, $Runner$, $Service$, and $Storage$ capabilities.
Each type refers to a specific set of resources. For instance, the Directory and Storage capabilities manage access to specific directories and namespaces inside the local file system of components.

Capabilities can be defined, routed, and used in a component manifest to control which parts of Fuchsia have the ability to connect to and access which resources.

For example, if a component \texttt{A} wants to define a capability on its \texttt{data} directory, it can include in the component manifest the code of Listing \ref{lst:capability_definition}. The directory will be mounted in \texttt{/published-data} with read, write, and execute permissions.

\begin{lstlisting}[caption={Definition of a directory capability.}, label={lst:capability_definition}]
   {
       capabilities: [
            {
                directory: "data",
                rights: ["r*"],
                path: "/published-data",
            },
        ]
    }
\end{lstlisting}


\subsubsection{Capability Routing}
\label{sec:cap-rout}

The capability routing graph \cite{routing} describes how components gain access to capabilities exposed and offered by other components in the component instance tree, building a \emph{provider-consumer} relationship.

Components define the use and the sharing of capabilities that they provide in their manifest file. Such capability routes are determined by the \texttt{use}, \texttt{offer}, and \texttt{expose} declarations \cite{routingTerminology}.

The \texttt{use} declaration enables a component to require a capability in its namespace at runtime. 
Listing \ref{lst:example_of_use_declaration} shows how a component \texttt{A} can ask for a Directory capability regarding the \texttt{data} folder.

\begin{lstlisting}[caption={Example of use declaration.}, label={lst:example_of_use_declaration}]
   {
     use: [
         {
             directory: "data",
             rights: ["rw*"],
             path: "/data",
         },
     ],
  }
\end{lstlisting}

The \texttt{offer} declaration, instead, states how a component can route a particular capability to its child component instances. 
For instance, Listing \ref{lst:example_of_offer_declaration} states how the component \texttt{A} (i.e., the one that declares the capability on the \texttt{data} folder) offers the corresponding capability to its child \texttt{B}.
\begin{lstlisting}[caption={Example of offer declaration.}, label={lst:example_of_offer_declaration}]
   {
        offer: [
            {
                directory: "data",
                from: "self",
                to: [ "#B" ],
            },
        ],
    }
\end{lstlisting}

Finally, the \texttt{expose} declaration states that the component can route a given capability to its parent in the component instance tree. In such a case, the component \texttt{A} of the previous examples expose the declared directory capability to its parent.
\begin{lstlisting}[caption={Example of expose declaration.}, label={lst:example_of_expose_declaration}]
   {
        expose: [
            {
                directory: "data",
                from: "#A",
            },
        ]
    }
\end{lstlisting}

It is worth noticing that capabilities routing can happen only among visible components, i.e., that belong to the same component instance tree.

The Component Manager is responsible for managing the capability routing process and manage the component instance tree for all apps. %It maintains the component instance tree for all applications to manage the routing of the exposed capabilities. 
%When a component requests access to a resource provided by another component, it forwards the request to the Component Manager.
%The Component Manager is responsible for managing the capability routing process. 
%It maintains the component instance tree for all applications to manage the routing of the exposed capabilities. 
When a component requests access to a resource provided by another component, it forwards the request to the Component Manager to establish whether it can hold the appropriate capability. To do so, the manager navigates the component instance tree to check whether: i) the target component is reachable (i.e., it is included in the component instance tree), and ii) it exists a path between the caller and the target which offers-exposes the required capability (and thus the access to the resource).

Figure \ref{fig:capability_routing} shows an example of capability routing in a component instance tree of a generic app. In this example, component \texttt{E} requests access to service \texttt{S} exposed by component \texttt{F}. The request of \texttt{E} is successfully executed since 1) a path between \texttt{F} and \texttt{E} exists in the component instance tree (i.e., arrows 1 to 4), and 2) the path offers-exposes the required service capability for \texttt{S} (\texttt{S} is exposed from \texttt{F} to its parents \texttt{B} and \texttt{A}; \texttt{S} is then offered to \texttt{E} through the child \texttt{C}).

\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.5\textwidth]{resources/images/capability_routing.png}
    \caption{Example of capability routing for the service S.}
    \label{fig:capability_routing}
\end{figure}


\subsection{Package Integrity}

Fuchsia enforces an integrity verification mechanism on software packages. 
In detail, each Fuchsia package is signed using the Merkle Tree algorithm \cite{merkleTree}. The signature information is stored directly inside the package in the meta-information file (called \texttt{meta.far}), similarly to those used for Android APK files \cite{apkSign}. The metadata information includes the package name, the version, and the signature of the content.
%To verify the integrity of the package, the Component Framework recomputes the signature of the package archive. If the computed tree matches the one stored, the Component Manager can install the package.

To verify the integrity of the package, the Component Framework recomputes the Merkle tree based on the content of the package. If the computed tree matches the one stored in the contents file, i.e., within the \texttt{meta.far}, the package is correctly verified and can be used by the Component Manager to build a new component instance. 

The package signature verification enables Fuchsia to detect undesired modifications in the package archive after it has been signed and to detect corrupts file, e.g., during the download of the package from an external repository.


\begin{comment}

\begin{itemize}
    \item \textbf{meta}: metadata information are contained within the meta.far archive. This file is the result of compressing metadata files with the far archive format \cite{far}. meta.far contains the meta directory, which contains the package file, that specifies name and version for the package, and the contents file, which support checks with for merkle tree verification of the package
    \item \textbf{non-meta files}: all files and directories outside the meta.far archive, are files needed to instance a new component instances, such as the binary of the program and eventual shared libraries
\end{itemize}
Fuchsia packages support their integrity verification thanks to the application of merkle tree algorithm. A package stores all metadata information within the meta.far archive, included the ones needed to verify the integrity of the package. 


Capabilities are the main security mechanism provided by Fuchsia OS. Like other capability-based os, Fuchsia OS allows processes that live outside a specific component, to access resources, such as directories on a file system local to the component, only if they own the right capabilities. Each component can expose capabilities to access only selected resources, to enable the execution of a task shared among more components. So, all resources inside a component are isolated from processes outside the component, that cannot also see them without the right capabilities. The access model behind Fuchsia OS is based on capabilities, so if a process owns a capability for a resource, it can access that resource. This access model is opposed to those based on acl \cite{acl}, in which the process that tries to access to a specific resource, must be executed by a user can has access to the resource, and so, it must be listed inside the acl table. Capabilities can be shared, so if a capability is routed to a component, all processes inside the component can use it. This mechanism is less restrictive than the acl one, because it eliminates all checks on the identity of the process that want to access the resource, and so, every process inside the component, also malicious ones, can access the resource. 

\subsubsection{Realm \& Collection}
The component manager creates a child component instance if declared within the manifest of another one or a component calls realm framework primitives to dynamically instance new instances. In a component instance tree, a Realm is a sub-tree routed on a component instance that have only children created statically from the manifest of their parents. Each child component instance in a realm is also the root of its sub-realm. A realm manages capability routing for capabilities that belong to component instances inside the realm, deciding which capabilities can be exposed outside the realm through the root component instance of the realm. Collections are groups of dynamic component instances children that are linked to a specific parent node. A component instance can create and manage a collection through the realm framework. The capability routing for dynamic component instances inside a collection is more straightforward than that of realms. All capabilities offered to a collection are also offered to every component instance within it. 

\subsubsection{Capability Routing}
One of the most important elements of Fuchsia OS are capabilities. The interaction between components is based on capabilities exchange. Rules of Fuchsia OS rule the exchange of capabilities. Components manage the capabilities that they provide and also those that use through their manifest file. Within the manifest file, a component can specify three kinds of keywords related to the interactions with capabilities:
\begin{itemize}
    \item \textbf{use}: this keyword specifies which capability a component could use during its execution. In detail, with this keyword, a component is allowed to use a capability provided from some other component
    \item \textbf{offer}: this keyword specifies that the component can route a certain capability to its child component instances
    \item \textbf{expose}: this keyword specifies that the component can route a certain capability to its parent in the component instance tree 
\end{itemize}
The usage of these three keywords (particularly for keywords offer and expose) enables the routing of capabilities within a component instance tree. A component instance can only see its child components. So, to route a capability to some other component, there must be a sequence of routing of the capability between the intermediate component instances. In detail, each component instance must offer or expose the target capability to its children, that have to do the same until it is reached the target component instance. The capability routing has to be defined statically within the manifest of components by using the keywords explained before. When a component needs to use a  capability provided by some other component, it has to interact with the component manager. The component manager is also responsible for managing the capability routing process. It maintains the component instance tree for all applications, to manage the routing of the exposed capabilities. So, when a component tries to access to a resource provided by another component, it forwards the request to the component manager that validate it through the component instance tree of the target component instance. After receiving the request, the component manager will navigate through the component instance tree, checking the path between the component instance that issued the request and the target one, and analysing the component manifest of all intermediate component instance between them. In particular, all intermediate component instances must access the capability and expose it to children or parent. At the end of the analysis, if the component instance that issued the request, can access the capability, it will be able to perform the request to the target component through the component manager. Figure \ref{fig:capability_routing} shows an example of capability routing in a component instance tree.
\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.5\textwidth]{resources/images/capability_routing.png}
    \caption{Example of capability routing}
    \label{fig:capability_routing}
\end{figure}

\subsubsection{Security of Capability Routing}
The capability routing is a mechanism linked to component isolation. Each component exposes capabilities to allows other components to access its resources. A component can see and interact only with its child components, and so, it can expose its capabilities only to those components. When a child component acquires the capability exposed from its parent component, it can decide to share it to its child component. This mechanism allows a capability to be shared to a specific component instance, sharing it among intermediate component instances. The capability is shared to known components, because all component instances that belong to the same component instance tree, are part of the same program, and it cannot be shared to component instances that belong to different component instance trees. If all component instances define statically its child component instances, in their manifest file, a capability will be securely routed from a component to another, because all component instance would be a priori known. The mechanism presents some problems in case of collections of components. Component instances inside a collection, are created dynamically, so all capabilities routed to the collection, are also routed to all component instances. If component instance was tricked in create a malicious component instance, the latter would gain all capabilities offered by the parent component instance, and so could perform operation to destroy the logic of the application. The capability routing mechanism is a powerful mechanism in case of statically defined realm inside a component instance tree, but it lacks in case of collections.

\end{comment}

==> Fuchsia OS/sections/software_model.tex <==
\section{Software Model}
\label{sec:software_model}

In Fuchsia, \emph{component} is the term for the common abstraction that defines how all software (regardless of source, programming language, or runtime) is described and executed on a Fuchsia system \cite{component}.

A component is a program that executes on a Fuchsia device. A component provides a binary program with an isolated environment not accessible from processes that belong to a different component. 
This property allows a process to access only to resources inside its component. 
Components are aggregated to create applications. Indeed, a developer can create an application, dividing its functionalities in components that have to interact with each other to carry out the task. The division of an application in components allows a developer to create a modular service, that it could easily extend to add new functionalities. 
So, Fuchsia enables developers to develop application focusing on separation of concerns. Generally, developers think components to execute small sub-tasks of the application, to ease its modularity and its further extension. 
Components ease the work of developers on testing, because they have to test single components opposed to the entire application. 
They also ease the reuse of code, because the same component could be used as part of other applications. An other property of components is their reliability, because if a component crashed, the crash would not impacted on the entire application, but only on a limited part of it. 
All components are uniquely identified by a url, i.e., fuchsia-pkg://fuchsia.com/stash\#meta/$<component\_manifest>$.cm.
    
%\subsubsection{Component Structure}
The component source is composed from:
    \begin{itemize}
        \item \textbf{Component Manifest Source}: this file specifies the structure of the component, such as the type of runner that has to execute the program inside the component, api exposed to the other components and rights associated to resources own by component. The figure \ref{lst:example_of_component_manifest} shows an example of component manifest source.
        \begin{lstlisting}[caption={Example of component manifest source}, label={lst:example_of_component_manifest}]
       {
          include: [ "syslog/client.shard.cml" ],
          program: {
              runner: "elf",
              binary: "bin/echo_client",
              args: [
                  "arg0",
                  "arg1",
              ],
          },
          use: [
              { protocol: "fidl.examples.routing.echo.Echo" },
          ],
       }
        \end{lstlisting}
        \item \textbf{Source code of the program}: set of source files of the program
        \item \textbf{Build file}: file that specify build configurations for source files, to compile and build the program to be run. This file is used to generate an intermediate representation file that can given in input to the Ninja \cite{ninja} build system. The figure \ref{lst:example_of_build_file} shows an example of a build file for components.
        \begin{lstlisting}[caption={Example of build file}, label={lst:example_of_build_file}]
           import("//build/components.gni")
           import("//build/rust/rustc_binary.gni")
    
           rustc_binary("echo_client") {
             edition = "2018"
             deps = [
                 "//examples/components/routing/fidl:echo-rustc",
                 "//src/lib/fuchsia",
                 "//src/lib/fuchsia-async",
                 "//src/lib/fuchsia-component",
                 "//third_party/rust_crates:anyhow",
                 "//third_party/rust_crates:futures",
                 "//third_party/rust_crates:tracing",
             ]
    
             sources = [ "src/main.rs" ]
          }
    
          fuchsia_component("echo_client_component") {
            manifest = "meta/echo_client.cml"
            component_name = "echo_client"
            deps = [ ":echo_client" ]
          }
        \end{lstlisting}
    \end{itemize}

When the component manager starts the execution process for the component, it assigns resources to the new component, and in particular:
    \begin{itemize}
        \item \textbf{File System}: when the component manager creates the component, it also executes the file system server, local to the component.
        \item \textbf{References to kernel objects}: the process executed inside the component is also provided with references to kernel objects, such as vmo and vmar that manages the memory allocated to the process 
    \end{itemize}
    
    
\subsection{Packages}



==> old/conclusions.tex <==
\section{Conclusions}
\label{sec:conclusions}

This paper proposes itself as the first step in the Fuchsia world. In particular, it tries to describe the main features of this operating system. From the analysis of the features of this operating system, we highlight some points that could be analyzed deeper with dedicated researches. 

==> old/research_directions.tex <==
\section{Research Directions}
\label{sec:research_directions}
This paper presents an overview of Fuchsia OS, focusing on security mechanisms implemented to guarantee a secure execution of processes inside the system. Briefly, Fuchsia OS secures the execution of processes through sandboxing mechanisms, such as components or virtualization. Fuchsia OS provides the capability mechanism to guarantee processes interoperability, which allows components to access only specific resources that belong to other components. The verification of capabilities is done at runtime by the component manager, which leverages the component instance tree in which live the interacting component instances, to check that all components have the capabilities to perform specific actions. At a low level, Fuchsia OS provides security mechanisms to secure the interaction between a process and the kernel through the separation of concerns carried out by kernel objects and through permissions to perform operations on those objects. Thus, although Fuchsia OS is in a beta testing phase, it implements strong security mechanisms that guarantee a high-security level inside the operating system. The security analysis carried out in this paper shows that there could be promising research points that could be developed to improve the security level of Fuchsia OS. In the following, will be declared some of the most promising ones:
\begin{itemize}
    \item all component instances have to interact with each other to carry out their main task. These interactions could lead to vulnerabilities, such as information leaks and the program’s execution flow changing.
    \item a process have to interact with the kernel to execute system calls. The specific interaction between the process and kernel objects could lead to dangerous vulnerabilities.
    \item capabilities sharing could enable a component instance to abuse its permissions and execute not wanted operations.
    \item Fuchsia OS allows the developer to run its component instances inside sessions that enable sharing api and libraries between component instances. This kind of sharing could lead to vulnerabilities due to the sharing of libraries and api to component instances that have not have them.
    \item Fidl abstracts the interaction between different processes, allowing the developer to define them through a high-level language. Thus, this language and its toolchain are critical for user processes interaction and user and kernel processes interaction. A vulnerability assessment on these protocols could lead to discovering vulnerabilities exploitable on all communication between processes.
    \item the component manager creates and manages all component instances through the Realm framework. This framework is responsible for the creation and management of realm and collections, and thus, the presence of vulnerabilities in this framework could impact the entire system’s security.
    \item the realm framework provides api that allows a component instance to dynamically create a collection and attach child component instances to it. Every capability routed to a collection is also routed to every component that belongs to the collection, providing component instances with capabilities that do not need. This capability routing would allow a malicious child component inside the collection to abuse these capabilities, gaining access to resources that it must not access.
\end{itemize}

==> old/security_mechanisms_&_discussions_old/discussion.tex <==
\section{Discussion}
\label{sec:discussion}
This section tries to discuss security mechanisms of Fuchsia OS, described in this paper. 

\subsection{Security of Kernel Objects}

\subsubsection{Separation of Concerns}
The usage of kernel objects enables the kernel to apply separation of concerns to tasks provided by zircon. 
Each object manages a task, also specific for a process, such as vmo and vmar. So, zircon kernel is principally an object manager and a system call handler. This separation of tasks allows the kernel to isolate its critical functions on the system. For example, if an attacker gained the control of a user process and of handles that it own, it could issued commands to objects, according to the rights provided to the handle, but the attack would be limited only to the object itself, and it would not propagate to other objects. The main idea is that a process cannot access to objects of which it has not the handle, so limiting the attack surface. Another important feature of objects, is that in most critical cases, the kernel responds to a system call issue creating a specific object instance and bound it to the process. Using this approach, critical objects, such as vmar and vmo, are only linked to a specific process, and not to a set of them. This approach protects the system in case an attacker would gain the control of a process, because the attack surface will be limited only to those objects own by the process. For example, if an attacker gained the access to a vmar object through an handle own by a process, it could done only operation on the virtual address space of that process, and it cannot propagate the attack on virtual address space of other processes. 

\subsubsection{Handle rights}
The handle is a pointer to a specific kernel object, as described in the paper. To each handle are associated a set of permissions to carry out operation on the related object. Providing a set of permissions to a specific handle, improve the security level of the system, because a process that owns an handle can only perform a limited set of operations on that object. The security mechanism enables the secure sharing of handles between processes. Indeed, Fuchsia OS provide a process the possibility to share its handles with other processes, through the usage of channel or sockets objects. When a process wants to pass an handle to another process, it can duplicate it and eventually reduce the set of permissions assigned to the duplicated one, limiting the set of possible operations that the target process could do. 

\subsection{Security of Component Isolation}

\subsubsection{Components}
In Fuchsia OS, all programs execute inside their isolated environment or component. A process inside a component can only see resources that belong to the component, and only those own by other components of which it has the capabilities to access. So, the fact that all components are isolated between each other and that can see only their child components, improves the security level of the system compared to the most common os, in which processes are isolated between each other, but they can access to the same resources, such as the same file system. In Fuchsia OS, the set of shared resources is limited to hardware, zircon kernels, drivers. Each component has its own file system, so the attack surface is reduced respect to the common os, and most of the attacks that involve the access of a shared file system between processes, is not applicable on Fuchsia OS.

\subsubsection{Capabilities}
Capabilities are the main security mechanism provided by Fuchsia OS. Like other capability-based os, Fuchsia OS allows processes that live outside a specific component, to access resources, such as directories on a file system local to the component, only if they own the right capabilities. Each component can expose capabilities to access only selected resources, to enable the execution of a task shared among more components. So, all resources inside a component are isolated from processes outside the component, that cannot also see them without the right capabilities. The access model behind Fuchsia OS is based on capabilities, so if a process owns a capability for a resource, it can access that resource. This access model is opposed to those based on acl \cite{acl}, in which the process that tries to access to a specific resource, must be executed by a user can has access to the resource, and so, it must be listed inside the acl table. Capabilities can be shared, so if a process owns a capability, it can share it with other processes. This mechanism is less restrictive than the acl one, because it eliminates all checks on the user that want to access the resource, and so, every process that own the capability, also malicious ones, can access the resource. In contrast with the acl mechanism, the capability mechanism speeds up authentication phase, because it does not need an acl table to be checked, but it decreases the security level of the system. 

\subsection{Security of Capability Routing}
The capability routing is a mechanism linked to component isolation. Each component exposes capabilities to allows other components to access its resources. A component can see and interact only with its child components, and so, it can expose its capabilities only to those components. When a child component acquires the capability exposed from its parent component, it can decide to share it to its child component. This mechanism allows a capability to be shared to a specific component instance, sharing it among intermediate component instances. The capability is shared to known components, because all component instances that belong to the same component instance tree, are part of the same program, and it cannot be shared to component instances that belong to different component instance trees. If all component instances define statically its child component instances, in their manifest file, a capability will be securely routed from a component to another, because all component instance would be a priori known. The mechanism presents some problems in case of collections of components. Component instances inside a collection, are created dynamically, so all capabilities routed to the collection, are also routed to all component instances. If component instance was tricked in create a malicious component instance, the latter would gained all capabilities offered by the parent component instance, and so could performed operation to destroy the logic of the application. The capability routing mechanism is a powerful mechanism in case of statically defined realm inside a component instance tree, but it lacks in case of collections.

==> old/security_mechanisms_&_discussions_old/security_mechanisms.tex <==
\section{Security Mechanisms}
\label{sec:securty_mechanisms}
This section describes some of the most important security mechanisms used by Fuchsia OS to guarantee the secure execution of components and of the interactions between processes and kernel objects.

\subsection{Kernel Objects Rights}
Objects are not secure by design, so every handle to kernel object is provided with a set of rights that enable specific operations on the referenced object. The rights are specific for the object, such as the permission to read or write to a channel, map vmo within the address space of the process, etc. Handles can be duplicated so that a process can take more handles to the same object. In general, a process needs to duplicate a handle to maintain handles to the same object but with a different set of rights. This mechanism is provided because a process can share its handle with another through channel or socket objects. An object can be garbage-collected only when there are no handles that reference it. So, when all handles own by processes are destroyed, also those eventually own by kernel process, the object will be garbage-collected.

\subsection{Component Isolation}
At a low level, a program is executed by a process. Fuchsia OS creates a process and gives it the minimum set of resources to start its execution. The os creates the process and provides it with the resources needed to start through the launchpad library. The launchpad library provides the process with:
\begin{itemize}
    \item a handle to a vmo that contains the executable of the program to be launched
    \item program arguments
    \item environment variables
    \item a handle to the vmo that contains the vDSO library for system call invoking
    \item handles to a local file system and a handle to the loader service
\end{itemize}
Unlike most common os, the dynamic linking of shared libraries is carried out through vmo. Each shared library to be used is pushed inside a vmo, so when a process wants to invoke a function provided by one of the shared objects, it has to invoke the function as an RPC \cite{rpc} through a dedicated channel object. To each process is assigned a set of resources that only it can see and access. The process cannot access or see the resources provided by another process unless they have capabilities to do it.

\subsection{Capability Routing}
One of the most important elements of Fuchsia OS are capabilities. The interaction between components is based on capabilities exchange. Rules of Fuchsia OS rule the exchange of capabilities. Components handle the capabilities that they provide and also those that use through their manifest file. Within the manifest file, a component can specify three kinds of keywords related to the interactions with capabilities: 
\begin{itemize}
    \item \textbf{use}: this keyword specifies which capability a component could use during its execution. In detail, with this keyword, a component is allowed to use the capability provided from some other component
    \item \textbf{offer}: this keyword specifies that the component can route a certain capability to its children component instances
    \item \textbf{expose}: this keyword specifies that the component can route a certain capability to its parent in the component instance tree 
\end{itemize}
The usage of these three keywords (particularly for keywords offer and expose) enables the routing of capabilities within a component instance tree. A component instance can only see its child components. So, to route a capability to some other component, there must be a sequence of routing of the capability between the intermediate component instances. In detail, each component instance must offer or expose the target capability to its children, that have to do the same until it is reached the target component instance. The capability routing has to be defined statically within the manifest of components by using the keywords explained before. Figure \ref{fig:capability_routing} shows an example of capability routing in a component instance tree.
\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.5\textwidth]{resources/images/capability_routing.png}
    \caption{Example of capability routing}
    \label{fig:capability_routing}
\end{figure}



==> old/security_mechanisms_&_discussions_old/versione1.1.tex <==
\section{Security Mechanisms}
\label{sec:securty_mechanisms}
This section describes some of the most important security mechanisms used by Fuchsia OS to guarantee the secure execution of components and of the interactions between processes and kernel objects.

\subsection{Handles Rights}
Objects are not secure by design, so every handle to kernel object is provided with a set of rights that enable specific operations on the referenced object. The rights are specific for the object, such as the permission to read or write to a channel, map vmo within the address space of the process, etc. The set of all possible rights is documented inside the Fuchsia documentation page \cite{handlesRights}. Handles can be duplicated so that a process can take more handles to the same object. In general, a process needs to duplicate a handle to maintain handles to the same object but with a different set of rights. This mechanism is provided because a process can share its handle with another through channel or socket objects. An object can be garbage-collected only when there are no handles that reference it. So, when all handles own by processes are destroyed, also those eventually own by kernel process, the object will be garbage-collected.

\subsubsection{Separation of Concerns of Kernel Objects}
The usage of kernel objects enables the kernel to apply separation of concerns to tasks provided by zircon. Each object manages a task, also specific for a process, such as vmo and vmar. So, zircon kernel is principally an object manager and a system call handler. This separation of tasks allows the kernel to isolate its critical functions on the system. For example, if an attacker gained the control of a user process and of handles that it own, it could issue commands to objects, according to the rights provided to the handle, but the attack would be limited only to the object itself, and it would not propagate to other objects. The main idea is that a process cannot access to objects of which it has not the handle, so limiting the attack surface. Another important feature of objects, is that in most critical cases, the kernel responds to a system call issue creating a specific object instance and bound it to the process. Using this approach, critical objects, such as vmar and vmo, are only linked to a specific process, and not to a set of them. This approach protects the system in case an attacker would gain the control of a process, because the attack surface will be limited only to those objects own by the process. For example, if an attacker gained the access to a vmar object through an handle own by a process, it could do only operation on the virtual address space of that process, and it cannot propagate the attack on virtual address space of other processes. 

\subsubsection{Security of Handle Rights}
Providing a set of rights to a specific handle, improve the security level of the system, because a process that owns an handle can only perform a limited set of operations on that object. The security mechanism enables the secure sharing of handles between processes. Indeed, when a process wants to pass an handle to another process, it can duplicate it and eventually reduce the set of permissions assigned to the duplicated one, limiting the set of possible operations that the target process could do. A possible best practice to secure the access to kernel objects is to implement a least privilege approach on the rights of objects. Indeed, a process can change rights assigned to a handle, being able to specify only the minimum set of rights, needed to execute its task. This approach can prevent an attacker to leverage specific rights to execute non-authorized operations on objects referenced by handles own by the process. 

\subsection{Component Isolation}
At a low level, a program is executed by a process. Fuchsia OS creates a process and gives it the minimum set of resources to start its execution. The os creates processes inside a component and provides them with the resources needed to start through the launchpad library. The launchpad library provides the process with:
\begin{itemize}
    \item a handle to a vmo that contains the executable of the program to be launched
    \item program arguments
    \item environment variables
    \item a handle to the vmo that contains the vDSO library for system call invoking
    \item handles to a local file system and a handle to the loader service
\end{itemize}
Unlike most common os, the dynamic linking of shared libraries is carried out through vmo objects. Each shared library to be used is pushed inside a vmo, so when a process wants to invoke a function provided by one of the shared objects, it has to invoke the function as an RPC \cite{rpc} through a dedicated channel object. To each process is assigned a set of resources that only it can see and access. The process cannot access or see the resources provided by another process unless they have capabilities to do it. The main principle that enable the component isolation is namespace. Component manager provides each a component with a namespace. Fuchsia OS has not a single file system, but each component has its own. The absence of a shared file system simplifies the adoption of security mechanisms to protect a component file system. Indeed, in most common operating systems, the concept of user is important to manage access to specific files or directory of the common file system. The user can access only to those files that it owns or those for which it has permissions gave from owners. This mechanism is important to manage he access of files that belong to different users and that are stored on the same physical file system. The isolation of file systems for components deletes the needing for users. Indeed, a process inside a component has all privileges to access files in its namespace, because all files belong to it. 

\subsubsection{Security of Components}
In Fuchsia OS, all programs execute inside their isolated environment or component. A process inside a component can only see resources that belong to the component, and only those own by other components of which it has the capabilities to access. So, the fact that all components are isolated between each other and that can see only their child components, improves the security level of the system compared to the most common os, in which processes are isolated between each other, but they can access to the same resources, such as the same file system. In Fuchsia OS, the set of shared resources is limited to hardware, zircon kernels, drivers. Each component has its own file system, so the attack surface is reduced respect to the common os, and most of the attacks that involve the access of a shared file system between processes, is not applicable on Fuchsia OS. In Fuchsia there is not the concept of user, because a process can access only to the limited resources provided by its component, so a process has all rights to access resources within the component, included files on the local file system. The absence of users makes impossible privilege escalation attacks. The isolation provided by components protect the system in case an attacker would take the control of a process inside a component. Indeed, if an attacker took the control of a process, it would have
access and modify only to resources inside the component, in particular only to files inside the local file system of the component and those stored in other components for which it has the capabilities to access. So, exploiting a vulnerability inside a component, compromises the execution flow only of that component, and does not propagate to others.

\subsubsection{Security of Capabilities}
Capabilities are the main security mechanism provided by Fuchsia OS. Like other capability-based os, Fuchsia OS allows processes that live outside a specific component, to access resources, such as directories on a file system local to the component, only if they own the right capabilities. Each component can expose capabilities to access only selected resources, to enable the execution of a task shared among more components. So, all resources inside a component are isolated from processes outside the component, that cannot also see them without the right capabilities. The access model behind Fuchsia OS is based on capabilities, so if a process owns a capability for a resource, it can access that resource. This access model is opposed to those based on acl \cite{acl}, in which the process that tries to access to a specific resource, must be executed by a user can has access to the resource, and so, it must be listed inside the acl table. Capabilities can be shared, so if a capability is routed to a component, all processes inside the component can use it. This mechanism is less restrictive than the acl one, because it eliminates all checks on the identity of the process that want to access the resource, and so, every process inside the component, also malicious ones, can access the resource. 

\subsubsection{Packages verification}
Packages are signed through the merkle tree algorithm \cite{merkleTree}, to guarantee that its content could not be modified. Packages are uniquely identified by a url. The content of a package is separated for its typology:
\begin{itemize}
    \item \textbf{meta}: metadata information are contained within the meta.far archive. This file is the result of compressing metadata files with the far archive format \cite{far}. meta.far contains the meta directory, which contains the package file, that specifies name and version for the package, and the contents file, which support checks with for merkle tree verification of the package
    \item \textbf{non-meta files}: all files and directories outside the meta.far archive, are files needed to instance a new component instances, such as the binary of the program and eventual shared libraries
\end{itemize}
Fuchsia packages support their integrity verification thanks to the application of merkle tree algorithm. A package stores all metadata information within the meta.far archive, included the ones needed to verify the integrity of the package. To verify the integrity of the package, the package manager recomputes the merkle tree based on the content of the package. If the computed tree matches the one stored in the contents file, within the meta.far, the package is correctly verified and can be used from the component manager to instance a new component instance. Also far archives support the integrity verification through merkle tree algorithm, so the meta.far archive is previously verified before the verification of the package. The merkle root algorithm allows component manager to only verify the integrity of the package, because the package could be downloaded from external repositories through the https protocol. So, the integrity verification of the package is needed to guarantee that the package is correctly downloaded from external providers. This mechanism does not help component manager to guarantee that the package has not been maliciously modified, because an attacker could modify the package content, replacing the merkle tree stored within the contents file.

\subsection{Capability Routing}
One of the most important elements of Fuchsia OS are capabilities. The interaction between components is based on capabilities exchange. Rules of Fuchsia OS rule the exchange of capabilities. Components manage the capabilities that they provide and also those that use through their manifest file. Within the manifest file, a component can specify three kinds of keywords related to the interactions with capabilities:
\begin{itemize}
    \item \textbf{use}: this keyword specifies which capability a component could use during its execution. In detail, with this keyword, a component is allowed to use a capability provided from some other component
    \item \textbf{offer}: this keyword specifies that the component can route a certain capability to its child component instances
    \item \textbf{expose}: this keyword specifies that the component can route a certain capability to its parent in the component instance tree 
\end{itemize}
The usage of these three keywords (particularly for keywords offer and expose) enables the routing of capabilities within a component instance tree. A component instance can only see its child components. So, to route a capability to some other component, there must be a sequence of routing of the capability between the intermediate component instances. In detail, each component instance must offer or expose the target capability to its children, that have to do the same until it is reached the target component instance. The capability routing has to be defined statically within the manifest of components by using the keywords explained before. When a component needs to use a  capability provided by some other component, it has to interact with the component manager. The component manager is also responsible for managing the capability routing process. It maintains the component instance tree for all applications, to manage the routing of the exposed capabilities. So, when a component tries to access to a resource provided by another component, it forwards the request to the component manager that validate it through the component instance tree of the target component instance. After receiving the request, the component manager will navigate through the component instance tree, checking the path between the component instance that issued the request and the target one, and analysing the component manifest of all intermediate component instance between them. In particular, all intermediate component instances must access the capability and expose it to children or parent. At the end of the analysis, if the component instance that issued the request, can access the capability, it will be able to perform the request to the target component through the component manager. Figure \ref{fig:capability_routing} shows an example of capability routing in a component instance tree.
\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.5\textwidth]{resources/images/capability_routing.png}
    \caption{Example of capability routing}
    \label{fig:capability_routing}
\end{figure}

\subsubsection{Security of Capability Routing}
The capability routing is a mechanism linked to component isolation. Each component exposes capabilities to allows other components to access its resources. A component can see and interact only with its child components, and so, it can expose its capabilities only to those components. When a child component acquires the capability exposed from its parent component, it can decide to share it to its child component. This mechanism allows a capability to be shared to a specific component instance, sharing it among intermediate component instances. The capability is shared to known components, because all component instances that belong to the same component instance tree, are part of the same program, and it cannot be shared to component instances that belong to different component instance trees. If all component instances define statically its child component instances, in their manifest file, a capability will be securely routed from a component to another, because all component instance would be a priori known. The mechanism presents some problems in case of collections of components. Component instances inside a collection, are created dynamically, so all capabilities routed to the collection, are also routed to all component instances. If component instance was tricked in create a malicious component instance, the latter would gain all capabilities offered by the parent component instance, and so could perform operation to destroy the logic of the application. The capability routing mechanism is a powerful mechanism in case of statically defined realm inside a component instance tree, but it lacks in case of collections.



==> old/version_1.0/component_description.tex <==
\section{Component Description}
\label{sec:component_description}
The following will describe some concepts and functioning of Fuchsia OS with a particular effort on the component framework and on system call invoking.

\subsection{Component}
A component is a program that executes on a Fuchsia device. Every software that executes on a Fuchsia device is a component, unless the Zircon kernel, bootloader, or device drivers. A component provides a binary program with an isolated environment not accessible from processes that belong to a different component. All components are uniquely identified by a url, ie. fuchsia-pkg://fuchsia.com/stash\#meta/$<component\_manifest>$.cm. A process inside a component can access only the resources inside that component. It could use specific resources from other ones only if it has the right capabilities. It communicates with other components through inter-process-communications (IPC) primitives, such as channels, sockets, fifo, to perform specific tasks or access resources provided by other components. Components implement the separation of concerns approach, allowing a developer to modularize its programs and dividing a more complex task into sub-tasks that can be carried out separately by different components. So, this approach allows a developer to extend its main task, adding new components without altering their main structure. A component could not contain a program to execute, and so, in this case, it can deliver \textit{capabilities} to other components. Fuchsia OS provides many runner components that can execute the code of programs inside a component. The modularization of the execution of programs inside a component would allow a developer to create custom runner components to execute programs written in a code not natively supported by Fuchsia OS. Fuchsia OS allows a component to define its configurations through the component manifest file. It describes the runner that will execute the code inside the component, the capabilities \textit{exposed} or \textit{offered} by the component, the static children of the component.

\subsubsection{Capability}
Fuchsia OS is a capability-based operating system. A capability is a token that identifies the rights to access a specific resource provided by a component. A component can expose capabilities to other components to access specific resources, enabling the interaction between different components. The available capabilities are fixed, so anyone cannot define custom capabilities to access resources other than those allowed by Fuchsia OS. Fuchsia capabilities are classified into seven types:
\begin{itemize}
    \item \textbf{Directory Capability}: this capability type allows a component to expose to other components the rights to see and use a specific directory inside the file system local to the component. The set of options associated with this capability type are declared inside the component manifest. For example, within the component manifest, a component can declare the path to the local directory and the set of rights on that directory. 
    \item \textbf{Event Capability}: this capability type allows components to receive events on information originated from the component manager. All component instances in a component instance tree can use the capability. So, see the event only if they explicitly declare it in their manifest, and it could be possible to route the capability to them. 
    \item \textbf{Protocol Capability}: in Fuchsia OS, a FIDL protocol is composed of a set of methods and events, which enable the interaction between different components. This capability type allows a component to use a specific FIDL protocol, exposed from another component or by the os itself. If the component provides a protocol, it will expose it through its outgoing directory (a directory in the local file system of the component, accessible from the other components, generally the svc directory).
    \item \textbf{Resolver Capability}: resolvers are specific elements of Fuchsia OS that allow a component to resolve the url for another component. The default url is already resolved by default, such as fuchsia-pkg, which identifies a package inside the os, fuchsia-boot, that identifies a component within the system boot image, http, that identifies a resource available through http protocol. In addition to these url schemes, a component can specify its custom url scheme through its manifest file, providing the associated resolver to other components through capability routing.
    \item \textbf{Runner Capability}: a runner component is responsible for running programs. Each runner supports the execution of a program written in a specific language. A component can specify the runner capability within the environment tag of its manifest file. So it will be available to all of its descendant components (or components inside the realm).
    \item \textbf{Service Capability}: in Fuchsia OS, a service is a set of protocols that allows components to perform more complex interactions with each other. This capability enables a component to offer or expose a specific service through its outgoing directory (usually the svc directory).  
    \item \textbf{Storage Capabilities}: the storage capability is linked to the directory capability. With this capability, a component allows another one to access an isolated directory inside its file system, visible and accessible only to the other component. This capability requires that the other component also receives the capability to access the directory in which the isolated one will be created. 
\end{itemize}

\subsubsection{Component Topology}
The component manager creates components from a package, a bundle that includes manifest, build configurations, and the program’s source that the runner process has to execute. The runner process is responsible for starting a new running component, which will be called a component instance. The component instance tree describes how component instance trees are related to each other. A moniker identifies each component instance within a component instance tree. It is an identifier built from the path to the component instance within the component instance tree. If the path used to identify the component instance is a relative path, the moniker will be a relative moniker. Else it will be an absolute moniker. Fuchsia uses a component instance tree to express composition relationships between components. Indeed, a child node is part of its parent node, forming a composition relationship between them. Each child component instance depends entirely on the parent, and so, it lives until the parent is alive.

\subsubsection{Realm \& Collection}
The component manager creates a child component instance if declared within the manifest of another one or a component calls realm framework primitives to dynamically instance new instances. In a component instance tree, a Realm is a sub-tree routed on a component instance that have only children created statically from the manifest of their parents. Each child component instance in a realm is also the root of its sub-realm. A realm manages capability routing for capabilities that belong to component instances inside the realm, deciding which capabilities can be exposed outside the realm through the root component instance of the realm. Collections are groups of dynamic component instances children that are linked to a specific parent node. A component instance can create and manage a collection through the realm framework. The capability routing for dynamic component instances inside a collection is more straightforward than that of realms. All capabilities offered to a collection are also offered to every component instance within it. 
\francesco{
    \begin{itemize}
        \item inserire immagine che spieghi cosa è un realm
        \item inserire immagine che spieghi cosa è una collection
    \end{itemize}
}

\subsubsection{Component Lifecycle}
A component has its lifecycle, which the component manager handles. Each component could listen for incoming lifecycle events, and so, they can perform tasks based on the state changed. In the following are reported the possible states for a component:
\begin{enumerate}
    \item \textbf{Create}: the component manager can create a component as the root of its component instance tree. Most of the time, starting a component is caused by the static declaration of the component inside the manifest file of another component or dynamically adding to an existing collection. Another important reason to start a component is a binding request from a component to another one. If a component wants to bind itself to another one, the component manager will check if there is a running instance of that component. If it finds a running instance, it will bind the component to the target one. Otherwise, it will create a new instance of that component and bind it to the new instance.
    
    \item \textbf{Start}: after the creation of a component, the component manager interacts with the required runner to execute the code inside that component. The runner will start the component, and so, this will pass it to the started state.
    
    \item \textbf{Stop}: a component could be stopped from the component manager because it terminated its task or when the user turns off the device. When a component passes to a stopped state, the component manager stores its state in persistent storage to restart the component further.
    
    \item \textbf{Destroy}: when a component instance is in a destroyed state, the component manager cannot restart it, and so, it completely removes it from its component instance tree. Still, it continues to exist in persistent storage.
    
    \item \textbf{Purge}: the component manager completely removes a component in this state from the system. Indeed, the OS will also delete its state from persistent storage.
\end{enumerate}

\subsection{Component Framework}
The component framework provides all tools to run components on Fuchsia and to support their execution. The main approach of Fuchsia is to divide a complex task into sub-task, each carried out by a specific component. Each component implements its sub-task through a service that it exposes to the other components. The interaction between different components through the usage of the exposed services allows the components to carry out a more complex task. Indeed, Fuchsia OS was thought to be modular and extensible during its lifetime. So, all tasks to be carried out are divided into multiple sub-task, each one executed from a different component, allowing their modularization. 

\subsection{FIDL}
Fuchsia Interface Definition Language (FIDL) is a set of tools that allows processes to communicate with each other, using high-level interfaces based on inter-process-communication (IPC) mechanisms. The usage of FIDL to abstract IPC between processes simplifies the implementation of the interaction between processes and lets avoid the more prone to bugs implementation through channels. Developers can define fidl files that specify the communication structure between processes, helping to define fuchsia protocols. These files are written in fidl language, which is similar to the most common languages and allows developers to use data types like integers, strings, arrays, structs, etc.  
The fidlc compiler compiles these files to produce client and server codes in the language used by the components that have to interoperate, and then these files can be included within the components code. These generated codes compose the fidl binding. At a low level, the communication implemented by fidl protocols is based on zircon channels, so the zircon kernel has an active part in the communication of component instances. FIDL enables the communication between processes applying standard communication models, also used in standard client-server interactions: 
\begin{itemize}
    \item \textbf{Client waits}: in this model, the client sends a request to the server and waits for the reply. The request sent can be a message or a call to a function exposed by the server
    \item \textbf{Client does not wait - no reply}: The client sends a request to the server but does not wait for the reply
    \item \textbf{Client does not wait - reply}: in this model, the client sends a request to the server but does not block itself waiting for the reply, and it will eventually check for the reply asynchronously. 
    \item \textbf{Client sends one request, Server sends multiple ones}: in this model, the client sends one request and blocks itself, waiting for the response only at the end of the computation. When the server sends the response, the client will be unlocked and can continue its execution until it needs new data from the server.
    \item \textbf{Server send data without Client request}: this model is similar to the previous one, but in this case, the server sends data without an initial request from the client
\end{itemize}

\subsection{System Call Execution}
When a process invokes a system call, the Zircon kernel starts a pipeline to handle it. In most os, a process invokes a system call passing the needed arguments to registers. Then, it invokes an interrupt to allow the os to execute the system call. In Fuchsia OS, the execution of a system call has to pass several intermediate phases to be completed:
\begin{enumerate}
    \item \textbf{vDSO}: it is a shared library that declares a function for each system call. Each declared function only has to put, in eax register, the integer that corresponds to the system call that names the function. All functions accept arguments that they have to pass to the handler procedure through the calling convention for the architecture in which the os executes. After the update of the eax register, all functions will execute a context switch to kernel mode to allow the kernel to execute the handler procedure. This shared object is hard-coded inside the Zircon kernel code, and it is loaded in a vmo object after the system boot.
    \item \textbf{Handler}: each system call takes its arguments from specific registers. The registers’ set is different for system calls (usually statically declared in the documentation). For all system calls, the eax register is responsible for storing the integer that identifies the system call within the system. The handler is composed of instructions that have to identify the invoked system call through the content of eax register and have to fill registers according to the specific system call invoked. The handler is different for system calls and for architecture in which the os executes. 
    \item \textbf{Wrapper}: the wrapper is a code that has to invoke the right system call implementation and handles every value returned from the system call. In most common cases, system call return handles to os objects.
    \item \textbf{Implementation}: this is the true code that execute the system call
\end{enumerate}
System call handlers and wrappers are automatically generated by a tool called kazoo \cite{kazoo}. Kazoo bases the generation of a specific pair of handler and wrapper on a fidl source file. The fidl source specifies input arguments to the system call and possible output values. In general, every kernel object has its fidl source \cite{vdso}, which declares all system calls related to that object. The fidl source is compiled with the fidlc compiler \cite{fidlc}, which generates a json file as an intermediate representation. This json file is given in input to the kazoo tool, which generates the handler, a c++ source that relies on the specific architecture of the device.

\subsection{Starnix Project}
Recently Google started to work on a side project called Starnix \cite{starnix}, which aims to allows Fuchsia to execute native android and linux applications. Indeed, Fuchsia provides a virtualization service to run external applications, with the overhead caused by the execution on virtual machines. Hence, the idea behind Starnix is to allow Fuchsia to emulate system call invocation and api calls, similarly to the wsl 1 \cite{wsl1}, to guarantee the complete execution of programs written for other contexts. 
 

==> old/version_1.0/conclusions.tex <==
\section{Conclusions}
\label{sec:conclusions}

This paper proposes itself as the first step in the Fuchsia world. In particular, it tries to describe the main features of this operating system. From the analysis of the features of this operating system, we highlight some points that could be analyzed deeper with dedicated researches. 

==> old/version_1.0/discussion.tex <==
\section{Discussion}
\label{sec:discussion}
This section tries to discuss security mechanisms of Fuchsia OS, described in this paper. 

\subsection{Security of Kernel Objects}

\subsubsection{Separation of Concerns}
The usage of kernel objects enables the kernel to apply separation of concerns to tasks provided by zircon. 
Each object manages a task, also specific for a process, such as vmo and vmar. So, zircon kernel is principally an object manager and a system call handler. This separation of tasks allows the kernel to isolate its critical functions on the system. For example, if an attacker gained the control of a user process and of handles that it own, it could issued commands to objects, according to the rights provided to the handle, but the attack would be limited only to the object itself, and it would not propagate to other objects. The main idea is that a process cannot access to objects of which it has not the handle, so limiting the attack surface. Another important feature of objects, is that in most critical cases, the kernel responds to a system call issue creating a specific object instance and bound it to the process. Using this approach, critical objects, such as vmar and vmo, are only linked to a specific process, and not to a set of them. This approach protects the system in case an attacker would gain the control of a process, because the attack surface will be limited only to those objects own by the process. For example, if an attacker gained the access to a vmar object through an handle own by a process, it could done only operation on the virtual address space of that process, and it cannot propagate the attack on virtual address space of other processes. 

\subsubsection{Handle rights}
The handle is a pointer to a specific kernel object, as described in the paper. To each handle are associated a set of permissions to carry out operation on the related object. Providing a set of permissions to a specific handle, improve the security level of the system, because a process that owns an handle can only perform a limited set of operations on that object. The security mechanism enables the secure sharing of handles between processes. Indeed, Fuchsia OS provide a process the possibility to share its handles with other processes, through the usage of channel or sockets objects. When a process wants to pass an handle to another process, it can duplicate it and eventually reduce the set of permissions assigned to the duplicated one, limiting the set of possible operations that the target process could do. 

\subsection{Security of Component Isolation}

\subsubsection{Components}
In Fuchsia OS, all programs execute inside their isolated environment or component. A process inside a component can only see resources that belong to the component, and only those own by other components of which it has the capabilities to access. So, the fact that all components are isolated between each other and that can see only their child components, improves the security level of the system compared to the most common os, in which processes are isolated between each other, but they can access to the same resources, such as the same file system. In Fuchsia OS, the set of shared resources is limited to hardware, zircon kernels, drivers. Each component has its own file system, so the attack surface is reduced respect to the common os, and most of the attacks that involve the access of a shared file system between processes, is not applicable on Fuchsia OS.

\subsubsection{Capabilities}
Capabilities are the main security mechanism provided by Fuchsia OS. Like other capability-based os, Fuchsia OS allows processes that live outside a specific component, to access resources, such as directories on a file system local to the component, only if they own the right capabilities. Each component can expose capabilities to access only selected resources, to enable the execution of a task shared among more components. So, all resources inside a component are isolated from processes outside the component, that cannot also see them without the right capabilities. The access model behind Fuchsia OS is based on capabilities, so if a process owns a capability for a resource, it can access that resource. This access model is opposed to those based on acl \cite{acl}, in which the process that tries to access to a specific resource, must be executed by a user can has access to the resource, and so, it must be listed inside the acl table. Capabilities can be shared, so if a process owns a capability, it can share it with other processes. This mechanism is less restrictive than the acl one, because it eliminates all checks on the user that want to access the resource, and so, every process that own the capability, also malicious ones, can access the resource. In contrast with the acl mechanism, the capability mechanism speeds up authentication phase, because it does not need an acl table to be checked, but it decreases the security level of the system. 

\subsection{Security of Capability Routing}
The capability routing is a mechanism linked to component isolation. Each component exposes capabilities to allows other components to access its resources. A component can see and interact only with its child components, and so, it can expose its capabilities only to those components. When a child component acquires the capability exposed from its parent component, it can decide to share it to its child component. This mechanism allows a capability to be shared to a specific component instance, sharing it among intermediate component instances. The capability is shared to known components, because all component instances that belong to the same component instance tree, are part of the same program, and it cannot be shared to component instances that belong to different component instance trees. If all component instances define statically its child component instances, in their manifest file, a capability will be securely routed from a component to another, because all component instance would be a priori known. The mechanism presents some problems in case of collections of components. Component instances inside a collection, are created dynamically, so all capabilities routed to the collection, are also routed to all component instances. If component instance was tricked in create a malicious component instance, the latter would gained all capabilities offered by the parent component instance, and so could performed operation to destroy the logic of the application. The capability routing mechanism is a powerful mechanism in case of statically defined realm inside a component instance tree, but it lacks in case of collections.

==> old/version_1.0/fuchsia_os.tex <==
\section{Fuchsia OS}
\label{sec:fuchsia_os}
This section presents the stack of Fuchsia OS, describing the composing elements of the architecture stack

\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.5\textwidth]{resources/images/fuchsia_architecture.png}
    \caption{Fuchsia Architecture}
    \label{fig:fuchsia_architecture}
\end{figure}

\subsection{Zircon}
The core of this operating system is the Zircon kernel. Zircon is a micro-kernel based on the Little Kernel project \cite{lk} to guarantee high performances on all kinds of devices, from IoT devices to smartphones. Little Kernel is mainly thought to adapt itself to devices with limited computational resources. So, it is suitable for the Fuchsia project that aims to be supported from as many devices as possible. It provides only the basic set of functionalities needed for the OS to work correctly as a micro-kernel. It is responsible for loading userspace processes in memory, communicates with the underlying hardware to make OS and hardware communicate, handles the booting phase of the device, powers up components that will take this phase, etc. Compared to a standard kernel, Zircon has to handle fewer tasks because many elements, such as drivers and the file system, are managed by user processes. Thanks to this simplification, the number of context switches between user-mode and kernel-mode, caused by operations that the kernel code has to execute, decreases.

\subsubsection{IPC}
Zircon kernel manages inter-process communication (IPC) between different processes and allows them to communicate although isolated in memory.
\begin{itemize}
    \item \textbf{Channel}: this object implements a bidirectional communication channel. A channel has two endpoints, and each of them maintains a separate fifo queue to store incoming messages. Every channel endpoint has an owner that also marks all messages sent and received by the endpoint, and only it can access these messages. They provide user code with primitives to add messages to the queue of the recipient process and to read them, and so, to dequeue them. A channel endpoint is not duplicable, but the owner could pass its ownership to another one. When the endpoint owner passes its ownership to a new owner, the new owner cannot access all messages in the queue marked with the previous owner.
    
    \item \textbf{Socket}: this object implements a bidirectional communication channel. These objects only move data and not handles, unlike the channel object. Processes can read and write data through their socket endpoints, using socket primitives. At the creation of the socket, the process can specify the in-bytes dimension of the socket.
    
    \item \textbf{FIFO}: objects thought to support shared memory between processes. They are more efficient than socket and channel objects in terms of timing to complete io operations, but they have a more limited buffer size.
\end{itemize}

\subsubsection{Scheduling \& Synchronization}
The Zircon kernel manages scheduling tasks for processes and threads that execute on the cpu of the device. This scheduler is based on the LK scheduler \cite{lk}, but it was extended to meet the needings of the Fuchsia OS. Together with scheduling tasks, Zircon also supports signal primitives to allow synchronization between different threads.
\begin{itemize}
    \item \textbf{Profile}: this object defines a set of priorities for scheduling configurations that the zircon kernel could apply to processes and threads. A single profile object could be linked with more processes and threads, and in this case, the scheduler will put them at the same level.
    
    \item \textbf{Event}: these objects are created to signal specific events for synchronization between processes.
    
    \item \textbf{Futex}: objects that manage synchronization between processes at a low level and in user-mode. They are the basis for \textit{pthread\_mutex} and \textit{pthread\_cond}, that are higher-level primitives. Futex objects do not provide rights to access to primitives that they expose because the base operations are \textit{wait} and \textit{wake} that have to be both accessible to leverage the basic functionalities of the object. Futexes does not support priority for calling processes, but they provide some API to allow further implementations based on them that could offer priority functionalities. The basis for priority implementation is the concept of ownership of a futex. If a process owns one or more futexes, its scheduling priority will be pushed to maximum among the waiter processes on the same futex. When a process unowns all its futexes, its scheduling priority will be restored to the base one.
\end{itemize}

\subsubsection{Memory Management}
Zircon kernel manages the allocation of memory to processes. Specific objects carry out all operations on the allocation and assignment of memory.
\begin{itemize}
    \item \textbf{Virtual Memory Object (VMO)}: an object that represents a region of virtual memory that can be shared among different processes. This object allows a process to perform several operations, such as reading, writing to the mapped pages and mapping the object itself to the process that requested the object. The vmo is a high-level infrastructure that allows the process to interact with the underlying memory pages, and it can also provide on-demand pages when needed.
    
    \item \textbf{Virtual Memory Address Region}: these objects represent a continuous set of addresses taken from a virtual address space. When a program executes, it has only a single vmar that contains all addresses of the program’s virtual address space, but it could be further divided with the creation of new vmar that do not overlap themself in their address space. Each vmar has a set of rights on the underlying memory. The starting vmar has all rights (read, write, execution) on the underlying memory. When a process makes a syscall to partition an existing vmar further, it can also specify the set of permissions for the new vmar. All vmar created by a process are related to each other by a tree data structure. In detail, a parent vmar maintains a reference to its children vmar, and this does not allow the destruction of a child vmar though there are no handles to it in the processes.
    
    \item \textbf{Pager}: these objects are responsible for supporting data provider entities, such as filesystems, to cache data they have to pass to other processes that request them. Their main task is to create vmo objects and provide them the needed pages to store data from the data provider.
\end{itemize}

\subsection{Fuchsia Runtime}
Fuchsia provides different kinds of runtimes that can start components. These runner processes are components that communicate with the component manager to obtain configurations for a program to be run. Their main task is to read configurations sent from the component manager to start executing new components. They do not provide libraries, but they only start their execution, so all components must have all libraries inside their package to be run correctly. A component must specify the type of runner and the needed configurations inside its manifest file. The component manager is responsible for submitting the starting of new components to the proper runner. Before submitting the request to the runner, the component manager will build a \textit{ComponentStartInfo} bundle, which contains the url of the component to be started, the content of the component package, etc. After receiving the starting request from the component manager, the runner will start the component.
\begin{itemize}
    \item \textbf{ELF Runner}: this runner is responsible for executing elf files \cite{elf}, for example, the ones generated after the compilation phase of c or rust files. 
    \item \textbf{DART AOT Runner}: this runner provides dart program \cite{dart}, with a configured dart virtual machine, to execute all bytecode generated by the compilation of the program. Most Dart programs define the UI of graphical components.
    \item \textbf{Web Runner}: the runner renders web pages to the screen of the device through the Chromium web engine \cite{chromium}.
\end{itemize}

\subsection{File System}
The Fuchsia file system is not linked or loaded by the kernel, unlike most operating systems, but it entirely lives in user-mode space. So, the file system lives in a user process, and it interacts with the other processes to provide and take files through inter-process communication primitives. This structure allows Fuchsia to execute file systems of a different kind without relying on a specific one. In most OS, in which the file system is inside the kernel, changing the file system would require the recompilation of the kernel. Instead, with the Fuchsia modular approach, each file system process can execute every kind of file system. An essential aspect of the user process file system is that every interaction to the file system does not require system call execution. Indeed, the kernel is not aware of a file system process structure, so all operation with a file system executes only in user-mode. A client process must invoke an RPC (Remote Procedure Code) exposed by the file system server to perform every kind of operation on file systems, such as open a file or store a file. fidl protocols manage the interaction between the file system process and the other processes. All interactions between a process and the file system process are carried out through channel objects at a low level. The system calls that the process calls to perform operations on file systems are restricted to only the needed ones to communicate with channels.     
\begin{itemize}
    \item \textbf{Namespace}: a namespace is an isolated environment in which all resources inside it, such as files, directories, sockets, services, etc., are visible only to processes that live in the environment and are unknown for processes that live in different namespaces. Processes external to the namespace can access resources inside the namespace only if they have the capabilities to do it. In Fuchsia, there is no concept of a global file system because every namespace has its own.
    \item \textbf{VFS}: vfs is a library that supports different kinds of operations on file system servers inside namespaces. It provides functions that simplify the interaction between a process and a file system server. Still, the letter could not use it because the unique requirement for a file system is to rely on a fidl protocol that enables the same operations between a process and the file system.
    \item \textbf{MemFS}: this kind of file system is maintained entirely in the memory of the device. For example, the bootfs protocol uses it during the booting phase of the device.
    \item \textbf{Blobfs}: file system used to store data represented through Merkle Trees \cite{merkle_tree}, also called signed data. This kind of file system is suitable for storing data that cannot be modified because it can be written only once. Fuchsia packages are stored on this kind of file system to do not allow their further modifications.
\end{itemize}

\subsection{Component Framework}
Fuchsia supports the execution of components with a set of manager programs that guide their lifecycle.
\begin{itemize}
    \item \textbf{Component Manager}: this component is at the base for the execution of components. It manages the start of all components, and for this, it is one of the first started entities. It handles the component lifecycle, from the starting to the purge of a component. It maintains the component instance tree’s topology to check the validity of certain requests sent by components. It is the core of the capability routing mechanism because it can check the validity of a certain path on the component instance tree, allowing a component to obtain a specific capability from another component.
    \item \textbf{Realm Framework}: this framework helps components to manage the creation and the handling of Realms and Collections. It provides a set of api to manage configurations of the environment in which a Realm executes, allows components to create a collection and attach component instances to it, enables capability routing for components inside the collection, etc.
    \item \textbf{Session Framework}: the component session manager is one of the most important managers in Fuchsia OS. It is responsible for creating session components and provide them with the needed capabilities. A session is a component that supports the execution of a set of sub-components linked to it. It is usually used when a meta-component needs to share resources needed from a set of components that carry out a common task. The session can
    \begin{itemize}
        \item provides capabilities (only those previously obtained from the session manager) and libraries to the underlying components
        \item define fidl protocols to enable the communication between the session itself and its children components
        \item instantiate components that will support specific fidl protocol middleware between the session and the component
    \end{itemize}
    \item \textbf{Hub}: this component can provide the state of components instances under a specific visibility scope. For example, it can show the status of all components under a specific Realm (without considering the root of the realm). Still, it does not allow the user or other components to modify the status information it exposes.
    \item \textbf{Test Framework}: this framework is used to test components. In detail, it provides a test manager that is responsible for launching component instances to test them. The test runner inside the test framework provides api, specific for the programming language used to implement the code to be run inside the component. 
\end{itemize}


% \begin{itemize}
%     \item Cosa è un component?
%     \item Component instance tree - realms - collections
%     \item Interazione tra diversi component
%     \item Protocollo FIDL per interscambio messaggi tra diversi "oggetti" in Fuchsia (tra component diversi o tra component e kernel object per esecuzione di syscall)
%     \item Isolamento e visibilità di ciasciun component
%     \item Capability Routing
%     \item File system locale al component e tipologia ========> V
%     \item Interazione con il file system e VFS layer ========> V
%     \item Pubblicazione di un package (tramite pm tool)
%     \item Zircon kernel?  ========> V
%     \item Zircon objects? ========> V
%     \item Come vengono eseguite syscall in Fuchsia
% \end{itemize}

==> old/version_1.0/introduction.tex <==
\section{Introduction}
\label{sec:introduction}

Fuchsia is an operating system developed by Google. Google revealed the existence of this project in august 2016, releasing the source code of an initial version of this operating system on GitHub. Fuchsia OS was officially presented, for the first time, at Google I/O 2019. This operating system has a high potential not only for performance but also for its modularity. Indeed, a user can install this operating system into every device, such as pcs, smartphones, smartwatches, and IoT devices. Google thought this operating system focused on security, so it developed all principles and concepts to guarantee proper isolation of its sub-tasks. The primary purpose of Fuchsia OS is to simplify the development of applications on different kinds of devices, installing the same operating system on them. Indeed, Google is trying to unify its operating systems, such as Chrome OS \cite{chrome_os} and Android \cite{android}. Android is one of the most used operating systems \cite{os_perc}, and anyone can install it on every kind of device, such as smartphones, infotainment, smartwatches, etc. The main problem of the Android ecosystem is that the operating system is customized specifically for the kind of device in which it is installed. These specific customizations involve that a developer has to develop an application based on the type of the device. So, it has to develop the same application many times (developing an android app for smartphones is different from doing it for smartwatches, smart homes, etc.). From this practical problem born the idea to create an ecosystem in which all devices run the same operating system version, simplifying the development of applications. These properties make Fuchsia OS interesting and innovative compared to the existing solutions, which do not care about the modern idea of an ecosystem of devices. To demonstrate the applicability of Fuchsia in a real context, Google, in May 2021, released Fuchsia OS as part of a beta testing program on its Nest Hub \cite{nest_hub}. Fuchsia OS is an interesting project because it is modular and security-oriented, but is it secure?
Fuchsia OS is a very recent operating system. So, there are not works at the state of the art that try to address security issues of this operating system, and there are not research works that describe all of its mechanisms. This paper is the first paper that analyses Fuchsia from the security point of view, providing some deeper analysis on the security of this operating system. This paper describes the functioning of Fuchsia OS, providing a stack that may help represent the most important elements of the operating system, focusing on security mechanisms adopted by Fuchsia OS. In addition, the paper tries to discuss each security mechanism, giving some ideas on possible research topics on this operating system.\\
\textit{\textbf{Structure of the paper}}. The rest of the paper is organized as follows: Section \ref{sec:fuchsia_os} describes the most relevant elements of the operating system, with the help of an architectural stack and section\ref{sec:component_description} describes components structure and their interactions within the system. Section \ref{sec:securty_mechanisms} introduces security mechanisms provided by Fuchsia OS, and \ref{sec:discussion} tries to discuss these mechanisms, focusing on their strengths and weakness. Section \ref{sec:research_directions} discusses some research directions based on the analysis of security mechanisms. Section \ref{sec:conclusions} concludes the paper.



==> old/version_1.0/research_directions.tex <==
\section{Research Directions}
\label{sec:research_directions}

This section presents some research ideas based on the analysis of security mechanisms carried out in this paper. In Fuchsia OS, a task is divided into more sub-tasks, each carried out by a specific component instance. All component instances have to interact with each other to carry out the main task. These interactions could lead to vulnerabilities, such as information leaks and the program’s execution flow changing. This interaction analysis could also be extended on the interaction between a component and kernel objects. The primary security mechanism to share access to resources are capabilities. This mechanism is critical from the security point of view because capabilities can be shared among component instances. Capabilities sharing could enable a component instance to abuse its permissions and execute not wanted operations. Fuchsia allows the developer to run its component instances inside sessions that enable sharing api and libraries between component instances, linking isolated instances. This kind of sharing could lead to vulnerabilities due to unwanted interactions between component instances. Fidl is the primary communication protocol that enables a more structured communication between different processes. So, this communication protocol is critical both for user processes interaction both for user and kernel processes interaction. A vulnerability assessment on these protocols could lead to discovering vulnerabilities exploitable on all communication between processes. All component instances are created and managed through the Realm framework. This framework is responsible for the creation and managing of realm and collections, and so, the presence of vulnerabilities in this framework could impact the security of the entire system.

==> old/version_1.0/security_mechanisms.tex <==
\section{Security Mechanisms}
\label{sec:securty_mechanisms}

\subsection{Kernel Objects}
Zircon is an object-based kernel, which means that all its functionalities are divided among different execution units, called objects, created only when needed. These objects are interfaces between user processes and OS resources. There is an object for every kind of task that the kernel has to manage, such as inter-process-communication, execution of user code, scheduling processes, handling synchronization between threads, managing the virtual memory assigned to a process, etc. Objects are not secure by design. A user process can interact with an object through specific handlers called Handles. 
A handle is a reference to an active object. They are created when a process issues a specific system call. When a process issues a system call, the kernel eventually creates an instance of the object needed to handle the request and also all further requests regarding the task. After the execution of the system call, the kernel returns a handle to that object to the calling process. If the process executes in user mode, the handle will be an integer that indexes a table, maintained by the kernel, which contains the set of live handles and the information on the bound objects and the set of rights to access the referenced objects. The integer index is valid only within the user process context. If another process tried to use the same index to access a handle, it would access a handle that points to another object or failed because the handle would not exist. If the process executes in kernel mode, it will obtain a c++ object that contains a reference to the kernel object, the pid of the process bound to the object, the set of rights to access the objects. A handle bound to a kernel process is said in transit. Every handle is provided with a set of rights that enable specific operations on the referenced object. The rights are specific for the object, such as the permission to read or write to a channel, map vmo within the address space of the process, etc. Handles can be duplicated so that a process can take more handles to the same object. In general, a process needs to duplicate a handle to maintain handles to the same object but with a different set of rights. This mechanism is provided because a process can share its handle with another through channel or socket objects. An object can be garbage-collected only when there are no handles that reference it. So, when all handles own by processes are destroyed, also those eventually own by kernel process, the object will be garbage-collected.

\subsection{Component Isolation}
At a low level, a program is executed by a process. Fuchsia OS creates a process and gives it the minimum set of resources to start its execution. The os creates the process and provides it with the resources needed to start through the launchpad library. The launchpad library provides the process with:
\begin{itemize}
    \item a handle to a vmo that contains the executable of the program to be launched
    \item program arguments
    \item environment variables
    \item a handle to the vmo that contains the vDSO library for system call invoking
    \item handles to a local file system (namespace) and a handle to the loader service
\end{itemize}
Unlike most common os, the dynamic linking of shared libraries is carried out through vmo. Each shared library to be used is pushed inside a vmo, so when a process wants to invoke a function provided by one of the shared objects, it has to invoke the function as an RPC \cite{rpc} through a dedicated channel object. This approach is opposed to the one provided by most operating systems, in which the dynamic linker maps the shared object in the address space of the process. So, the latter can call functions provided by the shared object, through got \cite{got}, and plt \cite{plt} tables. So, each process is assigned a set of resources that only it can see and access. The process cannot access or see the resources provided by another process unless they have capabilities to do it.

\subsection{Capability Routing}
One of the most important elements of Fuchsia OS are capabilities. The interaction between components is based on capabilities exchange. Rules of Fuchsia OS rule the exchange of capabilities. Components handle the capabilities that they provide and also those that use through their manifest file. Within the manifest file, a component can specify three kinds of keywords related to the interactions with capabilities: 
\begin{itemize}
    \item \textbf{use}: this keyword specifies which capability a component could use during its execution. In detail, with this keyword, a component is allowed to use the capability provided from some other component
    \item \textbf{offer}: this keyword specifies that the component can route a certain capability to its children component instances
    \item \textbf{expose}: this keyword specifies that the component can route a certain capability to its parent in the component instance tree 
\end{itemize}
The usage of these three keywords (particularly for keywords offer and expose) enables the routing of capabilities within a component instance tree. A component instance can only see its child components. 
So, to route a capability to some other component, there must be a sequence of routing of the capability between the intermediate component instances. In detail, each component instance must offer or expose the target capability to its children, that have to do the same until it is reached the target component instance. The capability routing has to be defined statically within the manifest of components by using the keywords explained before.
\francesco{
    \begin{itemize}
        \item inserire un immagine che mostri un esempio di capability routing
    \end{itemize}
}



==> sections/fuchsia_os.tex <==
\section{Fuchsia OS}
\label{sec:fuchsia_os}
This section presents the stack of Fuchsia OS, describing the composing elements of the architecture stack

\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.35\textwidth]{resources/images/fuchsia_architecture.png}
    \caption{Fuchsia Architecture}
    \label{fig:fuchsia_architecture}
\end{figure}

\subsection{Zircon}
The core of this operating system is the Zircon kernel. Zircon is a micro-kernel based on the Little Kernel project \cite{lk} to guarantee high performances on all kinds of devices, from IoT devices to smartphones and pcs. Little Kernel is mainly thought to adapt itself to devices with limited computational resources. So, it is suitable for the Fuchsia project that aims to be supported from as many devices as possible. Compared to a standard kernel, Zircon has to handle fewer tasks because many elements, such as drivers and the file system, are managed by user processes. Thanks to this simplification, the number of context switches between user-mode and kernel-mode, caused by operations that the kernel code has to execute, decreases.

\subsubsection{Kernel Objects}
Zircon is an object-based kernel, which means that all its functionalities are divided among different execution units, called objects, created only when needed. These objects are interfaces between user processes and OS resources. There is an object for every kind of task that the kernel has to manage, such as inter-process-communication, execution of user code, scheduling processes, handling synchronization between threads, managing the virtual memory assigned to a process, etc.

\subsubsection{IPC}
Zircon kernel manages inter-process communication (IPC) between different processes and allows them to communicate although isolated in memory.
\begin{itemize}
    \item \textbf{Channel}: this object implements a bidirectional communication channel. A channel has two endpoints, and each of them maintains a separate fifo queue to store incoming messages. %Every channel endpoint has an owner that also marks all messages sent and received by the endpoint, and only it can access these messages. 
    They provide user code with primitives to add messages to the queue of the recipient process and to read them, and so, to dequeue them.
    \item \textbf{Socket}: this object implements a bidirectional communication channel. Processes can read and write data through their socket endpoints, using socket primitives. At the creation of the socket, the process can specify the in-bytes dimension of the socket.
    \item \textbf{FIFO}: objects thought to support shared memory between processes. They are more efficient than socket and channel objects in terms of timing to complete io operations, but they have a more limited buffer size.
\end{itemize}

\subsubsection{Scheduling \& Synchronization}
The Zircon kernel manages scheduling tasks for processes and threads that execute on the cpu of the device. This scheduler is based on the LK scheduler \cite{lk}, but it was extended to meet the needings of the Fuchsia OS. Together with scheduling tasks, Zircon also supports signal primitives to allow synchronization between different threads.
\begin{itemize}
    \item \textbf{Profile}: this object defines a set of priorities for scheduling configurations that the zircon kernel could apply to processes and threads. A single profile object could be linked with more processes and threads, and in this case, the scheduler will put them at the same level.
    \item \textbf{Event}: these objects are created to signal specific events for synchronization between processes.
    \item \textbf{Futex}: objects that manage synchronization between processes at a low level and in user-mode. They are the basis for \textit{pthread\_mutex} and \textit{pthread\_cond}, that are higher-level primitives. Futex objects do not provide rights to access to primitives that they expose because the base operations are \textit{wait} and \textit{wake} that have to be both accessible to leverage the basic functionalities of the object. Futexes does not support priority for the calling processes, but they provide some API to allow further implementations of it. 
\end{itemize}

\subsubsection{Memory Management}
Zircon kernel manages the allocation of memory to processes. Specific objects carry out all operations on the allocation and assignment of memory.
\begin{itemize}
    \item \textbf{Virtual Memory Object (VMO)}: an object that represents a region of virtual memory that can be shared among different processes. This object allows a process to perform several operations, such as reading, writing to the mapped pages. The vmo is a high-level infrastructure that allows the process to interact with the underlying memory pages, and it can also provide on-demand pages when needed.
    \item \textbf{Virtual Memory Address Region}: these objects represent a continuous set of addresses taken from a virtual address space. When a program executes, it has only a single vmar that contains all addresses of the program’s virtual address space, but it could be further divided with the creation of new vmar that do not overlap themself in their address space. Each vmar has a set of rights on the underlying memory. The starting vmar has all rights (read, write, execution) on the underlying memory. When a process makes a system call to partition an existing vmar further, it can also specify the set of permissions for the new vmar. All vmar created by a process are related to each other by a tree data structure. In detail, a parent vmar maintains a reference to its children vmar, and this does not allow the destruction of a child vmar though there are no handles to it in the processes.
    \item \textbf{Pager}: these objects are responsible for supporting data provider entities, such as filesystems, to cache data they have to pass to other processes that request them. Their main task is to create vmo objects and provide them the needed pages to store data from the data provider.
\end{itemize}

\subsection{Fuchsia Runtime}
Fuchsia provides different kinds of runtimes that can start components. These runner processes communicate with the component manager to obtain configurations for a program to be run. Their main task is to read configurations sent from the component manager to start executing new components. They do not provide libraries, but they only start their execution, so all components must have all libraries inside their package to be run correctly. A component must specify the type of runner and the needed configurations inside its manifest file. The component manager is responsible for submitting the starting of new components to the proper runner.
\begin{itemize}
    \item \textbf{ELF Runner}: this runner is responsible for executing elf files \cite{elf}, for example, the ones generated after the compilation phase of c or rust files. 
    \item \textbf{DART AOT Runner}: this runner provides dart program \cite{dart}, with a configured dart virtual machine, to execute all bytecode generated by the compilation of the program. Most Dart programs define the UI of graphical components.
    \item \textbf{Web Runner}: the runner renders web pages to the screen of the device through the Chromium web engine \cite{chromium}.
\end{itemize}

\subsection{File System}
The Fuchsia file system is not linked or loaded by the kernel, unlike most operating systems, but it entirely lives in user-mode space. So, the file system lives in a user process, and it interacts with the other processes to provide and take files through inter-process communication primitives. This structure allows Fuchsia to execute file systems of a different kind without relying on a specific one. In most OS, in which the file system is inside the kernel, changing the file system would require the recompilation of the kernel. Instead, with the Fuchsia modular approach, each file system process can execute every kind of file system. An essential aspect of the user process file system is that every operation on file systems does not require system call execution (except the ones needed for interactions between the process and the file system. A client process must invoke an RPC (Remote Procedure Code) exposed by the file system server to perform every kind of operation on file systems, such as open a file or store a file.
\begin{itemize}
    \item \textbf{Namespace}: a namespace is an isolated environment in which all resources inside it, such as files, directories, sockets, etc., are visible only to processes that live in the environment and are unknown for processes that live in different namespaces. In Fuchsia, there is no concept of a global file system because every namespace has its own.
    \item \textbf{VFS}: vfs is a library that supports different kinds of operations on file system servers inside namespaces. It provides functions that simplify the interaction between a process and a file system server.
    \item \textbf{MemFS}: this kind of file system is maintained entirely in the memory of the device. For example, the bootfs protocol uses it during the booting phase of the device.
    \item \textbf{Blobfs}: file system used to store data represented through Merkle Trees \cite{merkle_tree}, also called signed data. This kind of file system is suitable for storing data that cannot be modified because it can be written only once. Fuchsia packages are stored on this kind of file system to do not allow their further modifications.
    \item \textbf{Outgoing Directory}: the outgoing directory is a directory inside the namespace of a component in which are put all objects that the component wants to expose to other components 
\end{itemize}

\subsection{Component Framework}
Fuchsia supports the execution of components with a set of manager programs that guide their lifecycle.
\begin{itemize}
    \item \textbf{Component Manager}: this process is at the base for the execution of components. It manages the lifecycle of all components, and for this, it is one of the first started entities. It maintains the component instance tree’s topology to check the validity of certain requests sent by components. It is the core of the capability routing mechanism because it can check the validity of a certain path on the component instance tree, allowing a component to obtain a specific capability from another one.
    \item \textbf{Realm Framework}: this framework helps components to manage the creation and the handling of realms and collections. It provides a set of api to manage configurations of the environment in which a Realm executes, allows components to create a collection and attach component instances to it, enables capability routing for components inside the collection, etc.
    \item \textbf{Session Framework}: the component session manager is a component responsible for creating session components and provide them with the needed capabilities. A session supports the execution of a set of child components. It is usually used when a component needs to share resources needed from a set of components that carry out a common task. The session can
    \begin{itemize}
        \item provide capabilities (only those previously obtained from the session manager) and libraries to the underlying components
        \item define fidl protocols to enable the communication between the session itself and its child components
        \item instantiate components that will support specific fidl protocol middlewares between the session and the component
    \end{itemize}
    \item \textbf{Hub}: this directory inside a file system stores the state of component instances under a specific visibility scope. For example, it maintains the status of all components under a specific Realm (without considering the root of the realm). A process cannot modify files inside the hub directory, but only read them.
    \item \textbf{Test Framework}: this framework is used to test components. In detail, it provides a test manager that is responsible for launching component instances to test them. The test runner inside the test framework provides api, specific for the programming language used to implement the code to be run inside the component. 
    \item \textbf{Resolvers}: resolvers are specific elements of Fuchsia OS that allow a component to resolve urls. The default urls are already resolved by default, such as fuchsia-pkg, which identifies a package inside the os, fuchsia-boot, that identifies a component within the system boot image, http, that identifies a resource available through http protocol. In addition to these url schemes, a component can specify its custom url scheme through its manifest file.
\end{itemize}

\subsection{Application Layer}
This paragraph groups some entities that are the basis for the developing of applications on Fuchsia OS:
\begin{itemize}
    \item \textbf{Package}: packages are archives used to 
    \item \textbf{Flutter}:
    \item \textbf{Scenic}:
\end{itemize}

==> sections/software_model.tex <==
\section{Software Model}
\label{sec:software_model}

In Fuchsia, \emph{component} is the term for the common abstraction that defines how all software (regardless of source, programming language, or runtime) is described and executed on a Fuchsia system \cite{component}.

A component is a program that executes on a Fuchsia device. A component provides a binary program with an isolated environment not accessible from processes that belong to a different component. 
This property allows a process to access only to resources inside its component. 
Components are aggregated to create applications. Indeed, a developer can create an application, dividing its functionalities in components that have to interact with each other to carry out the task. The division of an application in components allows a developer to create a modular service, that it could easily extend to add new functionalities. 
So, Fuchsia enables developers to develop application focusing on separation of concerns. Generally, developers think components to execute small sub-tasks of the application, to ease its modularity and its further extension. 
Components ease the work of developers on testing, because they have to test single components opposed to the entire application. 
They also ease the reuse of code, because the same component could be used as part of other applications. An other property of components is their reliability, because if a component crashed, the crash would not impacted on the entire application, but only on a limited part of it. 
All components are uniquely identified by a url, i.e., fuchsia-pkg://fuchsia.com/stash\#meta/$<component\_manifest>$.cm.
    
%\subsubsection{Component Structure}
The component source is composed from:
    \begin{itemize}
        \item \textbf{Component Manifest Source}: this file specifies the structure of the component, such as the type of runner that has to execute the program inside the component, api exposed to the other components and rights associated to resources own by component. The figure \ref{lst:example_of_component_manifest} shows an example of component manifest source.
        \begin{lstlisting}[caption={Example of component manifest source}, label={lst:example_of_component_manifest}]
       {
          include: [ "syslog/client.shard.cml" ],
          program: {
              runner: "elf",
              binary: "bin/echo_client",
              args: [
                  "arg0",
                  "arg1",
              ],
          },
          use: [
              { protocol: "fidl.examples.routing.echo.Echo" },
          ],
       }
        \end{lstlisting}
        \item \textbf{Source code of the program}: set of source files of the program
        \item \textbf{Build file}: file that specify build configurations for source files, to compile and build the program to be run. This file is used to generate an intermediate representation file that can given in input to the Ninja \cite{ninja} build system. The figure \ref{lst:example_of_build_file} shows an example of a build file for components.
        \begin{lstlisting}[caption={Example of build file}, label={lst:example_of_build_file}]
           import("//build/components.gni")
           import("//build/rust/rustc_binary.gni")
    
           rustc_binary("echo_client") {
             edition = "2018"
             deps = [
                 "//examples/components/routing/fidl:echo-rustc",
                 "//src/lib/fuchsia",
                 "//src/lib/fuchsia-async",
                 "//src/lib/fuchsia-component",
                 "//third_party/rust_crates:anyhow",
                 "//third_party/rust_crates:futures",
                 "//third_party/rust_crates:tracing",
             ]
    
             sources = [ "src/main.rs" ]
          }
    
          fuchsia_component("echo_client_component") {
            manifest = "meta/echo_client.cml"
            component_name = "echo_client"
            deps = [ ":echo_client" ]
          }
        \end{lstlisting}
    \end{itemize}

When the component manager starts the execution process for the component, it assigns resources to the new component, and in particular:
    \begin{itemize}
        \item \textbf{File System}: when the component manager creates the component, it also executes the file system server, local to the component.
        \item \textbf{References to kernel objects}: the process executed inside the component is also provided with references to kernel objects, such as vmo and vmar that manages the memory allocated to the process 
    \end{itemize}
    
    
\subsection{Packages}


